Averages of $b$-hadron, $c$-hadron, and $\tau$-lepton properties as of 2021

This paper reports world averages of measurements of $b$-hadron, $c$-hadron, and $\tau$-lepton properties obtained by the Heavy Flavour Averaging Group using results available before April 2021. In rare cases, significant results obtained several months later are also used. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, CP violation parameters, parameters of semileptonic decays, and Cabibbo-Kobayashi-Maskawa matrix elements.

==> rare/Radll/rareDecays_Bs_BR_1.tex <==
\hflavrowdef{\hflavrowdefaaa}{${\cal B}(B_s^0 \to \pi^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} \multicolumn{2}{l}{CDF {\cite{Aaltonen:2011jv}\tnote{1}\hphantom{\textsuperscript{1}}}} \\ \multicolumn{2}{l}{LHCb {\cite{Aaij:2016elb}\tnote{1}\hphantom{\textsuperscript{1}}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.70\,^{+0.11}_{-0.10}$ \\ \color{gray}$0.70 \pm0.10$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaab}{${\cal B}(B_s^0 \to \pi^0 \pi^0)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {L3 \cite{Acciarri:1995bx}} & { $< 210$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 210$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaac}{${\cal B}(B_s^0 \to \eta \pi^0)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {L3 \cite{Acciarri:1995bx}} & { $< 1000$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 1000$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaad}{${\cal B}(B_s^0 \to \eta \eta)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {L3 \cite{Acciarri:1995bx}} & { $< 1500$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 1500$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaae}{${\cal B}(B_s^0 \to \rho^0(770) \rho^0(770))$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {SLD \cite{Abe:1999ze}} & { $< 320$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 320$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaaf}{${\cal B}(B_s^0 \to \eta^\prime \eta^\prime)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015qga}} & { $32.4 \pm6.2 \pm3.0$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $32 \pm7$ \\ \color{gray}$33 \pm7$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaag}{${\cal B}(B_s^0 \to \eta^\prime \phi(1020))$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016yuv}} & { $< 0.82$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 0.82$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaah}{${\cal B}(B_s^0 \to \phi(1020) f_0(980)) \times {\cal B}(f_0(980) \to \pi^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016qnm}} & { $1.12 \pm0.16 \pm0.14$ \tnote{3}\hphantom{\textsuperscript{3}}} \\ \end{tabular}}}{\begin{tabular}{l} $1.12 \pm0.21$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaai}{${\cal B}(B_s^0 \to f_2(1270) \phi(1020)) \times {\cal B}(f_2(1270) \to \pi^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016qnm}} & { $0.61 \pm0.13\,^{+0.13}_{-0.08}$ \tnote{3}\hphantom{\textsuperscript{3}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.61\,^{+0.19}_{-0.15}$ \\ \color{gray}$0.61\,^{+0.18}_{-0.15}$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaaj}{${\cal B}(B_s^0 \to \phi(1020) \rho^0(770))$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016qnm}} & { $0.27 \pm0.07 \pm0.03$ \tnote{3}\hphantom{\textsuperscript{3}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.27 \pm0.08$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaak}{${\cal B}(B_s^0 \to \phi(1020) \pi^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016qnm}} & { $3.48 \pm0.23 \pm0.39$ \tnote{4,3}\hphantom{\textsuperscript{4,3}}} \\ \end{tabular}}}{\begin{tabular}{l} $3.48 \pm0.45$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaal}{${\cal B}(B_s^0 \to \phi(1020) \phi(1020))$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015cxj}} & { $18.6 \pm0.5 \pm1.6$ \tnote{3,5}\hphantom{\textsuperscript{3,5}}} \\ {CDF \cite{Aaltonen:2011rs}} & { $19.1 \pm1.5 \pm2.5$ \tnote{6}\hphantom{\textsuperscript{6}}} \\ \end{tabular}}}{\begin{tabular}{l} $18.7 \pm1.5$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaam}{${\cal B}(B_s^0 \to K^- \pi^+)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2012as}} & { $5.9 \pm0.7 \pm0.6$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2008hg}} & { $5.7 \pm1.0 \pm0.5$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $5.8 \pm0.7$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaan}{${\cal B}(B_s^0 \to K^+ K^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2012as}} & { $25.2 \pm1.8 \pm2.4$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2011qt}} & { $27.6 \pm2.4 \pm2.6$ \tnote{}\hphantom{\textsuperscript{}}} \\ {Belle \cite{Peng:2010ze}} & { $38\,^{+10}_{-9} \pm7$ \tnote{3}\hphantom{\textsuperscript{3}}} \\ \end{tabular}}}{\begin{tabular}{l} $26.7 \pm2.2$ \\ \color{gray}$26.6 \pm2.2$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaao}{${\cal B}(B_s^0 \to K^0 \bar{K}^0)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2020qfw}} & { $16.7 \pm2.9 \pm2.1$ \tnote{3,7}\hphantom{\textsuperscript{3,7}}} \\ {Belle \cite{Pal:2015ghq}} & { $19.6\,^{+5.8}_{-5.1} \pm2.2$ \tnote{3}\hphantom{\textsuperscript{3}}} \\ \end{tabular}}}{\begin{tabular}{l} $17.4 \pm3.1$ \\ \color{gray}$17.6\,^{+3.2}_{-3.1}$\\ \end{tabular}}
\begin{table}[H]
\begin{center}
%
\begin{threeparttable}
\caption{Branching fractions of charmless $B^0_s$ decays (part 1).}
\label{tab:rareDecays_Bs_BR_1}
\begin{tabular}{| Sl l l |}
\hline
\textbf{Parameter [$10^{-6}$]} & \textbf{Measurements} & \begin{tabular}{l}\textbf{Average $^\mathrm{HFLAV}_\mathrm{\color{gray}PDG}$}\end{tabular} \\
\hline
\hline
\hflavrowdefaaa \\
\hline
\hflavrowdefaab \\
\hline
\hflavrowdefaac \\
\hline
\hflavrowdefaad \\
\hline
\hflavrowdefaae \\
\hline
\hflavrowdefaaf \\
\hline
\hflavrowdefaag \\
\hline
\hflavrowdefaah \\
\hline
\hflavrowdefaai \\
\hline
\hflavrowdefaaj \\
\hline
\hflavrowdefaak \\
\hline
\hflavrowdefaal \\
\hline
\hflavrowdefaam \\
\hline
\hflavrowdefaan \\
\hline
\hflavrowdefaao \\
\hline
\end{tabular}
\begin{tablenotes}
\item[1] Measurement of $( {\cal B}(B_s^0 \to \pi^+ \pi^-) / {\cal B}(B^0 \to K^+ \pi^-) ) \frac{f_s}{f_d}$ used in our fit.
\item[2] Using ${\cal B}(B^+ \to \eta^\prime K^+)$.
\item[3] Multiple systematic uncertainties are added in quadrature.
\item[4] $400<M(\pi^+\pi^-)<1600~\rm{MeV/c^2.}$
\item[5] Using ${\cal B}(B^0 \to \phi(1020) K^*(892)^0)$.
\item[6] Using ${\cal B}(B_s^0 \to J/\psi \phi(1020))$.
\item[7] Using ${\cal B}(B^0 \to \phi(1020) K^0)$.
\end{tablenotes}
\end{threeparttable}
%
\end{center}
\end{table}


==> rare/Radll/rareDecays_Bs_BR_2.tex <==
\hflavrowdef{\hflavrowdefaap}{${\cal B}(B_s^0 \to K^0 \pi^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017zpx}} & { $9.50 \pm1.34 \pm1.67$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $9.5 \pm2.1$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaaq}{${\cal B}(B_s^0 \to K^0 K^+ \pi^- \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017zpx}} & { $84.5 \pm3.5 \pm8.0$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $84.5 \pm8.7$ \\ \color{gray}$84.5 \pm8.8$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaar}{${\cal B}(B_s^0 \to K^*(892)^- \pi^+)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2014aaa}} & { $2.93 \pm0.98 \pm0.41$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $2.9 \pm1.1$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaas}{${\cal B}(B_s^0 \to K^*(892)^+ K^- \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019nmr}} & { $18.6 \pm1.2 \pm4.5$ \tnote{3,4}\hphantom{\textsuperscript{3,4}}} \\ \end{tabular}}}{\begin{tabular}{l} $18.6 \pm4.7$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaat}{${\cal B}(B_s^0 \to K_0^*(1430)^+ K^- \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019nmr}} & { $31.3 \pm2.3 \pm25.3$ \tnote{3,4}\hphantom{\textsuperscript{3,4}}} \\ \end{tabular}}}{\begin{tabular}{l} $31 \pm25$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaau}{${\cal B}(B_s^0 \to K_2^*(1430)^+ K^- \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019nmr}} & { $10.3 \pm2.5 \pm16.4$ \tnote{3,4}\hphantom{\textsuperscript{3,4}}} \\ \end{tabular}}}{\begin{tabular}{l} $10 \pm17$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaav}{${\cal B}(B_s^0 \to K^*(892)^0 \bar{K}^0 \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019nmr}} & { $19.8 \pm2.8 \pm5.0$ \tnote{3,4}\hphantom{\textsuperscript{3,4}}} \\ \end{tabular}}}{\begin{tabular}{l} $19.8 \pm5.7$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaaw}{${\cal B}(B_s^0 \to K_0^*(1430)^0 \bar{K}^0 \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019nmr}} & { $33.0 \pm2.5 \pm9.8$ \tnote{3,4}\hphantom{\textsuperscript{3,4}}} \\ \end{tabular}}}{\begin{tabular}{l} $33 \pm10$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaax}{${\cal B}(B_s^0 \to K_2^*(1430)^0 \bar{K}^0 \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019nmr}} & { $16.8 \pm4.5 \pm21.3$ \tnote{3,4}\hphantom{\textsuperscript{3,4}}} \\ \end{tabular}}}{\begin{tabular}{l} $17 \pm22$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaay}{${\cal B}(B_s^0 \to K^0_S K^*(892)^0)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015asa}} & { $16.7 \pm3.5 \pm2.3$ \tnote{4,5}\hphantom{\textsuperscript{4,5}}} \\ \end{tabular}}}{\begin{tabular}{l} $16.7 \pm4.2$ \\ \color{gray}$16.4 \pm4.1$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaaz}{${\cal B}(B_s^0 \to K^0 K^+ K^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017zpx}} & { $1.29 \pm0.55 \pm0.36$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $1.29 \pm0.66$ \\ \color{gray}$1.29 \pm0.65$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaba}{${\cal B}(B_s^0 \to \bar{K}^*(892)^0 \rho^0(770))$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {SLD \cite{Abe:1999ze}} & { $< 767$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 767$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabb}{${\cal B}(B_s^0 \to K^*(892)^0 \bar{K}^*(892)^0)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015kba}} & { $11.2 \pm2.2 \pm1.5$ \tnote{4,6}\hphantom{\textsuperscript{4,6}}} \\ \end{tabular}}}{\begin{tabular}{l} $11.2 \pm2.7$ \\ \color{gray}$11.1 \pm2.7$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabc}{${\cal B}(B_s^0 \to \phi(1020) \bar{K}^*(892)^0)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2013gga}} & { $1.14 \pm0.24 \pm0.17$ \tnote{4,6}\hphantom{\textsuperscript{4,6}}} \\ \end{tabular}}}{\begin{tabular}{l} $1.14 \pm0.30$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabd}{${\cal B}(B_s^0 \to p \bar{p})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017gum}} & { $< 0.015$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 0.015$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabe}{${\cal B}(B_s^0 \to p \bar{p} K^+ K^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017pgn}} & { $4.2 \pm0.3 \pm0.4$ \tnote{4}\hphantom{\textsuperscript{4}}} \\ \end{tabular}}}{\begin{tabular}{l} $4.2 \pm0.5$ \\ \color{gray}$4.5 \pm0.5$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabf}{${\cal B}(B_s^0 \to p \bar{p} K^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017pgn}} & { $1.3 \pm0.2 \pm0.2$ \tnote{4}\hphantom{\textsuperscript{4}}} \\ \end{tabular}}}{\begin{tabular}{l} $1.3 \pm0.3$ \\ \color{gray}$1.4 \pm0.3$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabg}{${\cal B}(B_s^0 \to p \bar{p} \pi^+ \pi^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017pgn}} & { $< 0.66$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 0.66$ \\ \color{gray}$0.43 \pm0.20$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabh}{${\cal B}(B_s^0 \to p \bar{\Lambda}^0 K^- \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017vnw}} & { $5.46 \pm0.61 \pm0.82$ \tnote{4}\hphantom{\textsuperscript{4}}} \\ \end{tabular}}}{\begin{tabular}{l} $5.5 \pm1.0$\\ \end{tabular}}
\begin{table}[H]
\begin{center}
%
\begin{threeparttable}
\caption{Branching fractions of charmless $B^0_s$ decays (part 2).}
\label{tab:rareDecays_Bs_BR_2}
\begin{tabular}{| Sl l l |}
\hline
\textbf{Parameter [$10^{-6}$]} & \textbf{Measurements} & \begin{tabular}{l}\textbf{Average $^\mathrm{HFLAV}_\mathrm{\color{gray}PDG}$}\end{tabular} \\
\hline
\hline
\hflavrowdefaap \\
\hline
\hflavrowdefaaq \\
\hline
\hflavrowdefaar \\
\hline
\hflavrowdefaas \\
\hline
\hflavrowdefaat \\
\hline
\hflavrowdefaau \\
\hline
\hflavrowdefaav \\
\hline
\hflavrowdefaaw \\
\hline
\hflavrowdefaax \\
\hline
\hflavrowdefaay \\
\hline
\hflavrowdefaaz \\
\hline
\hflavrowdefaba \\
\hline
\hflavrowdefabb \\
\hline
\hflavrowdefabc \\
\hline
\hflavrowdefabd \\
\hline
\hflavrowdefabe \\
\hline
\hflavrowdefabf \\
\hline
\hflavrowdefabg \\
\hline
\hflavrowdefabh \\
\hline
\end{tabular}
\begin{tablenotes}
\item[1] Using ${\cal B}(B^0 \to K^0 \pi^+ \pi^-)$.
\item[2] Using ${\cal B}(B^0 \to K^*(892)^+ \pi^-)$.
\item[3] Result extracted from Dalitz plot analysis of $B^0_s \to K_S^0 K^+ \pi^-$ decays.
\item[4] Multiple systematic uncertainties are added in quadrature.
\item[5] Using ${\cal{B}}(B^0 \to K^0 \pi^+ \pi^-)$.
\item[6] Using ${\cal B}(B^0 \to \phi(1020) K^*(892)^0)$.
\end{tablenotes}
\end{threeparttable}
%
\end{center}
\end{table}


==> rare/Radll/rareDecays_Bs_BR_3.tex <==
\hflavrowdef{\hflavrowdefabi}{${\cal B}(B_s^0 \to \gamma \gamma)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {Belle \cite{Dutta:2014sxo}} & { $< 3.1$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 3.1$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabj}{${\cal B}(B_s^0 \to \phi(1020) \gamma)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2012ita}} & { $33.9 \pm1.7 \pm3.1$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ {Belle \cite{Dutta:2014sxo}} & { $36.0 \pm5.0 \pm7.0$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $34.1 \pm3.2$ \\ \color{gray}$34.2 \pm3.6$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabk}{${\cal B}(B_s^0 \to \mu^+ \mu^-)$\tnote{2}\hphantom{\textsuperscript{2}}}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {ATLAS \cite{Aaboud:2018mst}} & { $0.0028\,^{+0.0008}_{-0.0007}$ \tnote{}\hphantom{\textsuperscript{}}} \\ {LHCb \cite{Aaij:2017vad}} & { $0.0030 \pm0.0006\,^{+0.0003}_{-0.0002}$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CMS \cite{Sirunyan:2019xdu}} & { $0.0029 \pm0.0007 \pm0.0002$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2013as}} & { $0.013\,^{+0.009}_{-0.007}$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.00295 \pm0.00041$ \\ \color{gray}$0.00294\,^{+0.00042}_{-0.00039}$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabl}{${\cal B}(B_s^0 \to e^+ e^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2020nol}} & { $< 0.0094$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2009vr}} & { $< 0.28$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 0.0094$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabm}{${\cal B}(B_s^0 \to \tau^+ \tau^-)$\tnote{3}\hphantom{\textsuperscript{3}}}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017xqt}} & { $< 5200.0$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 5200$ \\ \color{gray}$< 6800$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabn}{${\cal B}(B_s^0 \to \mu^+ \mu^- \mu^+ \mu^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016kfs}} & { $< 0.0025$ \tnote{4}\hphantom{\textsuperscript{4}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 0.0025$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabo}{${\cal B}(B_s^0 \to \phi(1020) \mu^+ \mu^-)$\tnote{5}\hphantom{\textsuperscript{5}}}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {\color{red}LHCb \cite{LHCb:2021zwz}} & { $0.859 \pm0.023 \pm0.061$ \tnote{6,7}\hphantom{\textsuperscript{6,7}}} \\ {CDF \cite{Aaltonen:2011qs}} & { $1.21 \pm0.20 \pm0.11$ \tnote{7}\hphantom{\textsuperscript{7}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.865 \pm0.065$ \\ \color{gray}$0.823\,^{+0.119}_{-0.116}$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabp}{${\cal B}(B_s^0 \to \bar{K}^*(892)^0 \mu^+ \mu^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2018jhg}} & { $0.029 \pm0.010 \pm0.004$ \tnote{6}\hphantom{\textsuperscript{6}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.029 \pm0.011$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabq}{${\cal B}(B_s^0 \to \pi^+ \pi^- \mu^+ \mu^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} \multicolumn{2}{l}{LHCb {\cite{Aaij:2014lba}\tnote{8,9}\hphantom{\textsuperscript{8,9}}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.084 \pm0.016$ \\ \color{gray}$0.084 \pm0.017$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabr}{${\cal B}(B_s^0 \to \phi(1020) \nu \bar{\nu})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {DELPHI \cite{Adam:1996ts}} & { $< 5400$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 5400$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabs}{${\cal B}(B_s^0 \to e^+ \mu^- \mathrm{+c.c.})$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017cza}} & { $< 0.0054$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2009vr}} & { $< 0.2$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 0.0054$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabt}{${\cal B}(B_s^0 \to \tau^+ \mu^- \mathrm{+c.c.})$\tnote{3}\hphantom{\textsuperscript{3}}}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2019okb}} & { $< 34.0$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 34$ \\ \color{gray}$< 42$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabu}{${\cal B}(B_s^0 \to \eta^\prime \eta)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {\color{red}Belle \cite{Belle:2021bxn}} & { $< 65$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 65$ \\ \color{gray} none\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabv}{${\cal B}(B_s^0 \to f_2^{\prime}(1525) \mu^+ \mu^-)$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {\color{red}LHCb \cite{LHCb:2021zwz}} & { $0.166 \pm0.020 \pm0.015$ \tnote{6,7}\hphantom{\textsuperscript{6,7}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.166 \pm0.025$ \\ \color{gray} none\\ \end{tabular}}
\begin{table}[H]
\begin{center}
\resizebox{1\textwidth}{!}{
\begin{threeparttable}
\caption{Branching fractions of charmless $B^0_s$ decays (part 3).}
\label{tab:rareDecays_Bs_BR_3}
\begin{tabular}{| Sl l l |}
\hline
\textbf{Parameter [$10^{-6}$]} & \textbf{Measurements} & \begin{tabular}{l}\textbf{Average $^\mathrm{HFLAV}_\mathrm{\color{gray}PDG}$}\end{tabular} \\
\hline
\hline
\hflavrowdefabi \\
\hline
\hflavrowdefabj \\
\hline
\hflavrowdefabk \\
\hline
\hflavrowdefabl \\
\hline
\hflavrowdefabm \\
\hline
\hflavrowdefabn \\
\hline
\hflavrowdefabo \\
\hline
\hflavrowdefabp \\
\hline
\hflavrowdefabq \\
\hline
\hflavrowdefabr \\
\hline
\hflavrowdefabs \\
\hline
\hflavrowdefabt \\
\hline
\hflavrowdefabu \\
\hline
\hflavrowdefabv \\
\hline
\end{tabular}
\begin{tablenotes}
\item[1] Using ${\cal B}(B^0 \to K^*(892)^0 \gamma)$.
\item[2] The ATLAS measurement is correlated with ${\cal{B}}(B^0 \to \mu^+ \mu^-)$. This correlation is not taken into account in our average. For more information see Ref.~\cite{CMS-PAS-BPH-20-003}.
\item[3] PDG shows the result obtained at 95\% CL.
\item[4] At CL=95\,\%.
\item[5] The PDG uncertainty includes a scale factor.
\item[6] Multiple systematic uncertainties are added in quadrature.
\item[7] Using ${\cal B}(B_s^0 \to J/\psi \phi(1020))$.
\item[8] Muon pairs do not originate from resonances and $0.5<m_{\pi^+\pi^-}< 1.3~\rm{GeV/}c^2$.
\item[9] Measurement of ${\cal B}(B_s^0 \to \pi^+ \pi^- \mu^+ \mu^-) / ( {\cal B}(B^0 \to J/\psi K^*(892)^0) {\cal B}(J/\psi \to \mu^+ \mu^-) {\cal B}(K^*(892)^0 \to K \pi) 2/3 )$ used in our fit.
\end{tablenotes}
\end{threeparttable}
}
\end{center}
\end{table}


==> rare/Radll/rareDecays_Bs_RBR_1.tex <==
\hflavrowdef{\hflavrowdefabw}{$\frac{f_s}{f_d}  \frac{\mathcal{B}(B^0_s\rightarrow\pi^+\pi^-)}{\mathcal{B}(B^0\rightarrow K^+\pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2016elb}} & { $0.915 \pm0.071 \pm0.083$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2011jv}} & { $0.8 \pm0.2 \pm0.1$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.893 \pm0.098$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabx}{$\frac{f_s}{f_d}  \frac{\mathcal{B}(B^0_s\rightarrow\pi^+\pi^-)}{\mathcal{B}(B^0\rightarrow \pi^+\pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2012as}} & { $5.0\,^{+1.1}_{-0.9} \pm0.4$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $5.0\,^{+1.2}_{-1.0}$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaby}{$\dfrac{{\cal B}(B_s^0 \to \phi(1020) \phi(1020))}{{\cal B}(B_s^0 \to J/\psi \phi(1020))}$\tnote{1}\hphantom{\textsuperscript{1}}}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {CDF \cite{Aaltonen:2011rs}} & { $1.78 \pm0.14 \pm0.20$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $1.78 \pm0.24$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefabz}{$\dfrac{{\cal B}(B_s^0 \to \phi(1020) \phi(1020))}{{\cal B}(B^0 \to \phi(1020) K^*(892)^0)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015cxj}} & { $184 \pm5 \pm13$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $184 \pm14$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaca}{$\frac{f_s}{f_d}  \frac{\mathcal{B}(B^0_s\rightarrow K^+\pi^-)}{\mathcal{B}(B^0_d\rightarrow K^+\pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2012as}} & { $7.4 \pm0.6 \pm0.6$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2008hg}} & { $7.1 \pm1.0 \pm0.7$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $7.30 \pm0.70$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacb}{$\frac{f_s}{f_d} \frac{\mathcal{B}(B^0_s\rightarrow K^+K^-)}{\mathcal{B}(B^0_d\rightarrow K^+\pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2012as}} & { $31.6 \pm0.9 \pm1.9$ \tnote{}\hphantom{\textsuperscript{}}} \\ {CDF \cite{Aaltonen:2011qt}} & { $34.7 \pm2.0 \pm2.1$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $32.7 \pm1.7$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacc}{$\dfrac{{\cal B}(B_s^0 \to K^0 \pi^+ \pi^-)}{{\cal B}(B^0 \to K^0 \pi^+ \pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017zpx}} & { $19.1 \pm2.7 \pm3.3$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $19.1 \pm4.3$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacd}{$\dfrac{{\cal B}(B_s^0 \to K^0 K^+ \pi^- \mathrm{+c.c.})}{{\cal B}(B^0 \to K^0 \pi^+ \pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017zpx}} & { $170 \pm7 \pm15$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $170 \pm16$\\ \end{tabular}}
\hflavrowdef{\hflavrowdeface}{$\dfrac{{\cal B}(B_s^0 \to K^0 K^+ K^-)}{{\cal B}(B^0 \to K^0 \pi^+ \pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017zpx}} & { $< 5.1$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $< 5.1$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacf}{$\dfrac{{\cal B}(B_s^0 \to K^*(892)^- \pi^+)}{{\cal B}(B^0 \to K^*(892)^+ \pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2014aaa}} & { $39 \pm13 \pm5$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $39 \pm14$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacg}{$\dfrac{{\cal B}(B_s^0 \to K^*(892)^0 \bar{K}^*(892)^0)}{{\cal B}(B^0 \to \phi(1020) K^*(892)^0)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015kba}} & { $111 \pm22 \pm13$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $111 \pm26$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefach}{$\dfrac{{\cal B}(B_s^0 \to \phi(1020) \bar{K}^*(892)^0)}{{\cal B}(B^0 \to \phi(1020) K^*(892)^0)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2013gga}} & { $11.3 \pm2.4 \pm1.6$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $11.3 \pm2.9$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaci}{$\dfrac{{\cal B}(B_s^0 \to \phi(1020) \mu^+ \mu^-)}{{\cal B}(B_s^0 \to J/\psi \phi(1020))}$\tnote{3}\hphantom{\textsuperscript{3}}}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{LHCb:2021zwz}} & { $0.0800 \pm0.0021 \pm0.0016$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ {CDF \cite{Aaltonen:2011qs}} & { $0.113 \pm0.019 \pm0.007$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.0806 \pm0.0026$\\ \end{tabular}}
\begin{table}[H]
\begin{center}
%
\begin{threeparttable}
\caption{Relative branching fractions of charmless $B^0_s$ decays (part 1).}
\label{tab:rareDecays_Bs_RBR_1}
\begin{tabular}{| Sl l l |}
\hline
\textbf{Parameter [$10^{-2}$]} & \textbf{Measurements} & \begin{tabular}{l}\textbf{Average}\end{tabular} \\
\hline
\hline
\hflavrowdefabw \\
\hline
\hflavrowdefabx \\
\hline
\hflavrowdefaby \\
\hline
\hflavrowdefabz \\
\hline
\hflavrowdefaca \\
\hline
\hflavrowdefacb \\
\hline
\hflavrowdefacc \\
\hline
\hflavrowdefacd \\
\hline
\hflavrowdeface \\
\hline
\hflavrowdefacf \\
\hline
\hflavrowdefacg \\
\hline
\hflavrowdefach \\
\hline
\hflavrowdefaci \\
\hline
\end{tabular}
\begin{tablenotes}
\item[1] The PDG average is a result of a fit including input from other measurements.
\item[2] Multiple systematic uncertainties are added in quadrature.
\item[3] The PDG uncertainty includes a scale factor.
\end{tablenotes}
\end{threeparttable}
%
\end{center}
\end{table}


==> rare/Radll/rareDecays_Bs_RBR_2.tex <==
\hflavrowdef{\hflavrowdefacj}{$\dfrac{{\cal B}(B_s^0 \to p \bar{p} K^+ \pi^-)}{{\cal B}(B^0 \to p \bar{p} K^+ \pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017pgn}} & { $22 \pm4 \pm2$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $22 \pm5$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefack}{$\dfrac{{\cal B}(B_s^0 \to p \bar{p} K^+ \pi^-)}{{\cal B}(B_s^0 \to p \bar{p} K^+ K^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017pgn}} & { $31 \pm5 \pm2$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $31 \pm5$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacl}{$\frac{ {\cal{B}}(B^0_s \to \bar{K}^*(892)^0 \mu^+\mu^-)}{ {\cal{B}}(B^0_s \to J/\psi \bar{K}^*(892)^0 ) \times {\cal{B}}(J/\psi \to \mu^+ \mu^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2018jhg}} & { $1.4 \pm0.4 \pm0.1$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $1.4 \pm0.4$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacm}{$\dfrac{{\cal B}(B_s^0 \to \bar{K}^*(892)^0 \mu^+ \mu^-)}{{\cal B}(\bar{B}^0 \to \bar{K}^*(892)^0 \mu^+ \mu^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2018jhg}} & { $3.3 \pm1.1 \pm0.4$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $3.3 \pm1.2$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacn}{$\dfrac{{\cal B}(B_s^0 \to \phi(1020) \phi(1020) \phi(1020))}{{\cal B}(B_s^0 \to \phi(1020) \phi(1020))}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2017tzn}} & { $11.7 \pm3.0 \pm1.5$ \tnote{}\hphantom{\textsuperscript{}}} \\ \end{tabular}}}{\begin{tabular}{l} $11.7 \pm3.4$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefaco}{$\dfrac{{\cal B}(B_s^0 \to K^0 \bar{K}^0)}{{\cal B}(B^0 \to \phi(1020) K^0)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2020qfw}} & { $230 \pm40 \pm22$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $230 \pm46$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacp}{$\dfrac{{\cal B}(B_s^0 \to K^0_S K^*(892)^0)}{{\cal B}(B^0 \to K^0_S \pi^+ \pi^-)}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2015asa}} & { $33 \pm7 \pm4$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $33 \pm8$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacq}{$\dfrac{{\cal B}(B_s^0 \to f_2^{\prime}(1525) \mu^+ \mu^-)}{{\cal B}(B_s^0 \to J/\psi \phi(1020))}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{LHCb:2021zwz}} & { $0.0155 \pm0.0019 \pm0.0008$ \tnote{1}\hphantom{\textsuperscript{1}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.0155 \pm0.0021$\\ \end{tabular}}
\hflavrowdef{\hflavrowdefacr}{$\frac{{\cal{B}}( B^{0}_{s} \to \pi^+ \pi^- \mu^+ \mu^-)}{{\cal{B}}( B^{0} \to J/\psi K^{*0} ) \times {\cal{B}}( J/\psi \to \mu^+ \mu^- ) \times {\cal{B}}( K^{*0} \to K^+ \pi^- )}$}{{\setlength{\tabcolsep}{0pt}\begin{tabular}{m{6em}l} {LHCb \cite{Aaij:2014lba}} & { $0.167 \pm0.029 \pm0.013$ \tnote{2}\hphantom{\textsuperscript{2}}} \\ \end{tabular}}}{\begin{tabular}{l} $0.167 \pm0.032$\\ \end{tabular}}
\begin{table}[H]
\begin{center}
%
\begin{threeparttable}
\caption{Relative branching fractions of charmless $B^0_s$ decays (part 2).}
\label{tab:rareDecays_Bs_RBR_2}
\begin{tabular}{| Sl l l |}
\hline
\textbf{Parameter [$10^{-2}$]} & \textbf{Measurements} & \begin{tabular}{l}\textbf{Average}\end{tabular} \\
\hline
\hline
\hflavrowdefacj \\
\hline
\hflavrowdefack \\
\hline
\hflavrowdefacl \\
\hline
\hflavrowdefacm \\
\hline
\hflavrowdefacn \\
\hline
\hflavrowdefaco \\
\hline
\hflavrowdefacp \\
\hline
\hflavrowdefacq \\
\hline
\hflavrowdefacr \\
\hline
\end{tabular}
\begin{tablenotes}
\item[1] Multiple systematic uncertainties are added in quadrature.
\item[2] Muon pairs do not originate from resonances and $0.5<m_{\pi^+\pi^-}< 1.3~\rm{GeV/}c^2$.
\end{tablenotes}
\end{threeparttable}
%
\end{center}
\end{table}


==> tau/hflav-2018-babar-prelim-ichep2018.tex <==
\htmeasdef{BaBar.Gamma10.prelim.ICHEP2018}{Gamma10}{\babar}{Lusiani:2019mis}{( 7.17 \pm 0.031 \pm 0.21 ) \cdot 10^{ -3 }}{7.17e-03}{\pm 0.031e-03}{0.21e-03}%
\htmeasdef{BaBar.Gamma16.prelim.ICHEP2018}{Gamma16}{\babar}{Lusiani:2019mis}{( 5.05 \pm 0.02 \pm 0.15 ) \cdot 10^{ -3 }}{5.05e-03}{\pm 0.02e-03}{0.15e-03}%
\htmeasdef{BaBar.Gamma23.prelim.ICHEP2018}{Gamma23}{\babar}{Lusiani:2019mis}{( 6.15 \pm 0.12 \pm 0.34 ) \cdot 10^{ -4 }}{6.15e-04}{\pm 0.12e-04}{0.34e-04}%
\htmeasdef{BaBar.Gamma27.prelim.ICHEP2018}{Gamma27}{\babar}{Lusiani:2019mis}{( 1.168 \pm 0.006 \pm 0.038 ) \cdot 10^{ -2 }}{1.168e-02}{\pm 0.006e-02}{0.038e-02}%
\htmeasdef{BaBar.Gamma28.prelim.ICHEP2018}{Gamma28}{\babar}{Lusiani:2019mis}{( 1.25 \pm 0.16 \pm 0.24 ) \cdot 10^{ -4 }}{1.25e-04}{\pm 0.16e-04}{0.24e-04}%
\htmeasdef{BaBar.Gamma809.prelim.ICHEP2018}{Gamma809}{\babar}{Lusiani:2019mis}{( 9.02 \pm 0.40 \pm 0.65 ) \cdot 10^{ -4 }}{9.02e-04}{\pm 0.40e-04}{0.65e-04}%
\htdef{BaBar.Gamma10.prelim.ICHEP2018,qt}{\ensuremath{(0.7170 \pm 0.0031 \pm 0.0210) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma16.prelim.ICHEP2018,qt}{\ensuremath{(0.5050 \pm 0.0020 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma23.prelim.ICHEP2018,qt}{\ensuremath{(0.0615 \pm 0.0012 \pm 0.0034) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma27.prelim.ICHEP2018,qt}{\ensuremath{(1.1680 \pm 0.0060 \pm 0.0380) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma28.prelim.ICHEP2018,qt}{\ensuremath{(1.250 \pm 0.160 \pm 0.240) \cdot 10^{-4} }}%
\htdef{BaBar.Gamma809.prelim.ICHEP2018,qt}{\ensuremath{(9.020 \pm 0.400 \pm 0.650) \cdot 10^{-4} }}%
\htdef{BaBar prelim. ICHEP2018.cite}{\cite{Lusiani:2019mis}}%
\htdef{BaBar prelim. ICHEP2018.collab}{BaBar}%
\htdef{BaBar prelim. ICHEP2018.ref}{\babar prelim. ICHEP2018 \cite{Lusiani:2019mis}}%
\htdef{BaBar prelim. ICHEP2018.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma10.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma16.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma23.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma27.gn} = \htuse{Gamma27.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma27.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma28.gn} = \htuse{Gamma28.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma28.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma809.gn} = \htuse{Gamma809.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma809.prelim.ICHEP2018}}%


==> tau/hflav-2021-elab-vadirect.tex <==
\htquantdef{B_tau_had_fit}{B_tau_had_fit}{}{64.73 \pm 0.11}{64.73}{0.11}%
\htquantdef{B_tau_had_uni}{B_tau_had_uni}{}{64.80 \pm 0.06}{64.80}{0.06}%
\htquantdef{B_tau_had_uni_SM}{B_tau_had_uni_SM}{}{64.87 \pm 0.04}{64.87}{0.04}%
\htquantdef{B_tau_s_fit}{B_tau_s_fit}{}{2.908 \pm 0.048}{2.908}{0.048}%
\htquantdef{B_tau_s_unitarity}{B_tau_s_unitarity}{}{(2.976 \pm 0.099) \cdot 10^{-2}}{2.976\cdot 10^{-2}}{0.099\cdot 10^{-2}}%
\htquantdef{B_tau_VA}{B_tau_VA}{}{0.6183 \pm 0.0010}{0.6183}{0.0010}%
\htquantdef{B_tau_VA_fit}{B_tau_VA_fit}{}{61.83 \pm 0.10}{61.83}{0.10}%
\htquantdef{B_tau_VA_unitarity}{B_tau_VA_unitarity}{}{0.61894 \pm 0.00081}{0.61894}{0.00081}%
\htquantdef{Be_by_tau_tau}{Be_by_tau_tau}{}{(6.1248 \pm 0.0021) \cdot 10^{11}}{6.1248\cdot 10^{11}}{0.0021\cdot 10^{11}}%
\htquantdef{Be_fit}{Be_fit}{}{0.17811 \pm 0.00041}{0.17811}{0.00041}%
\htquantdef{Be_from_Bmu}{Be_from_Bmu}{}{0.17878 \pm 0.00041}{0.17878}{0.00041}%
\htquantdef{Be_from_taulife}{Be_from_taulife}{}{0.17780 \pm 0.00031}{0.17780}{0.00031}%
\htquantdef{Be_lept}{Be_lept}{}{17.845 \pm 0.032}{17.845}{0.032}%
\htquantdef{Be_lept_unc_perc}{Be_lept_unc_perc}{}{0.180}{0.180}{0}%
\htquantdef{Be_unitarity}{Be_unitarity}{}{0.1788 \pm 0.0011}{0.1788}{0.0011}%
\htquantdef{Be_univ}{Be_univ}{}{17.812 \pm 0.022}{17.812}{0.022}%
\htquantdef{Bmu_by_Be_th}{Bmu_by_Be_th}{}{0.9725606 \pm 0.0000036}{0.9725606}{0.0000036}%
\htquantdef{Bmu_fit}{Bmu_fit}{}{0.17387 \pm 0.00040}{0.17387}{0.00040}%
\htquantdef{Bmu_from_taulife}{Bmu_from_taulife}{}{0.17293 \pm 0.00030}{0.17293}{0.00030}%
\htquantdef{Bmu_unitarity}{Bmu_unitarity}{}{0.1746 \pm 0.0010}{0.1746}{0.0010}%
\htquantdef{BR_a1_pigamma}{BR_a1_pigamma}{}{0.2100\cdot 10^{-2}}{0.2100\cdot 10^{-2}}{0}%
\htquantdef{BR_eta_2gam}{BR_eta_2gam}{}{0.3941}{0.3941}{0}%
\htquantdef{BR_eta_3piz}{BR_eta_3piz}{}{0.3268}{0.3268}{0}%
\htquantdef{BR_eta_charged}{BR_eta_charged}{}{0.2789}{0.2789}{0}%
\htquantdef{BR_eta_neutral}{BR_eta_neutral}{}{0.7212}{0.7212}{0}%
\htquantdef{BR_eta_pimpipgamma}{BR_eta_pimpipgamma}{}{4.220\cdot 10^{-2}}{4.220\cdot 10^{-2}}{0}%
\htquantdef{BR_eta_pimpippiz}{BR_eta_pimpippiz}{}{0.2292}{0.2292}{0}%
\htquantdef{BR_f1_2pip2pim}{BR_f1_2pip2pim}{}{0.1090}{0.1090}{0}%
\htquantdef{BR_f1_2pizpippim}{BR_f1_2pizpippim}{}{0.2180}{0.2180}{0}%
\htquantdef{BR_KS_2piz}{BR_KS_2piz}{}{0.3069}{0.3069}{0}%
\htquantdef{BR_KS_pimpip}{BR_KS_pimpip}{}{0.6920}{0.6920}{0}%
\htquantdef{BR_om_pimpip}{BR_om_pimpip}{}{1.530\cdot 10^{-2}}{1.530\cdot 10^{-2}}{0}%
\htquantdef{BR_om_pimpippiz}{BR_om_pimpippiz}{}{0.8930}{0.8930}{0}%
\htquantdef{BR_om_pizgamma}{BR_om_pizgamma}{}{8.400\cdot 10^{-2}}{8.400\cdot 10^{-2}}{0}%
\htquantdef{BR_phi_KmKp}{BR_phi_KmKp}{}{0.4920}{0.4920}{0}%
\htquantdef{BR_phi_KSKL}{BR_phi_KSKL}{}{0.3400}{0.3400}{0}%
\htquantdef{BRA_Kz_KL_KET}{BRA_Kz_KL_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{BRA_Kz_KS_KET}{BRA_Kz_KS_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{BRA_Kzbar_KL_KET}{BRA_Kzbar_KL_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{BRA_Kzbar_KS_KET}{BRA_Kzbar_KS_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{c0}{c0}{CODATA 2018 speed of light in vacuum}{2.998\cdot 10^{8}}{2.998\cdot 10^{8}}{0}%
\htquantdef{corr_dRrad_pi_munu_K_munu}{corr_dRrad_pi_munu_K_munu}{}{0.67}{0.67}{0}%
\htquantdef{corr_dRrad_pi_munu_K_munu_dicarlo2019}{corr_dRrad_pi_munu_K_munu_dicarlo2019}{}{0.63}{0.63}{0}%
\htquantdef{deltaR_su3break}{deltaR_su3break}{}{0.238 \pm 0.033}{0.238}{0.033}%
\htquantdef{deltaR_su3break_d2pert}{deltaR_su3break_d2pert}{}{9.300 \pm 3.400}{9.300}{3.400}%
\htquantdef{deltaR_su3break_pheno}{deltaR_su3break_pheno}{}{0.1544 \pm 0.0037}{0.1544}{0.0037}%
\htquantdef{deltaR_su3break_remain}{deltaR_su3break_remain}{}{(0.3400 \pm 0.2800) \cdot 10^{-2}}{0.3400\cdot 10^{-2}}{0.2800\cdot 10^{-2}}%
\htquantdef{dRrad_K_munu}{dRrad_K_munu}{}{1.07 \pm 0.21}{1.07}{0.21}%
\htquantdef{dRrad_K_munu_dicarlo2019}{dRrad_K_munu_dicarlo2019}{}{0.24 \pm 0.10}{0.24}{0.10}%
\htquantdef{dRrad_kmunu_by_pimunu}{dRrad_kmunu_by_pimunu}{}{-0.69 \pm 0.17}{-0.69}{0.17}%
\htquantdef{dRrad_kmunu_by_pimunu_dicarlo2019}{dRrad_kmunu_by_pimunu_dicarlo2019}{}{-1.26 \pm 0.14}{-1.26}{0.14}%
\htquantdef{dRrad_pi_munu}{dRrad_pi_munu}{}{1.76 \pm 0.21}{1.76}{0.21}%
\htquantdef{dRrad_pi_munu_dicarlo2019}{dRrad_pi_munu_dicarlo2019}{}{1.53 \pm 0.19}{1.53}{0.19}%
\htquantdef{dRrad_tauK}{dRrad_tauK}{}{-0.15 \pm 0.57}{-0.15}{0.57}%
\htquantdef{dRrad_tauK_by_Kmu}{dRrad_tauK_by_Kmu}{}{0.97 \pm 0.58}{0.97}{0.58}%
\htquantdef{dRrad_tauK_by_taupi}{dRrad_tauK_by_taupi}{}{0.10 \pm 0.80}{0.10}{0.80}%
\htquantdef{dRrad_taupi}{dRrad_taupi}{}{-0.24 \pm 0.56}{-0.24}{0.56}%
\htquantdef{dRrad_taupi_by_pimu}{dRrad_taupi_by_pimu}{}{0.18 \pm 0.57}{0.18}{0.57}%
\htquantdef{EmNuNumb}{EmNuNumb}{}{0.1782}{0.1782}{0}%
\htquantdef{f_K_by_f_pi_dicarlo2019}{f_K_by_f_pi_dicarlo2019}{}{1.1966 \pm 0.0018}{1.1966}{0.0018}%
\htquantdef{f_K_dicarlo2019}{f_K_dicarlo2019}{}{156.1 \pm 0.2}{156.1}{0.2}%
\htquantdef{f_Kpm}{f_Kpm}{}{155.7 \pm 0.3}{155.7}{0.3}%
\htquantdef{f_Kpm_by_f_pipm}{f_Kpm_by_f_pipm}{}{1.1932 \pm 0.0021}{1.1932}{0.0021}%
\htquantdef{f_pipm}{f_pipm}{}{130.2 \pm 0.8}{130.2}{0.8}%
\htquantdef{Gamma1}{\BR_{1}}{\BRF{\tau^-}{particle^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K^0\, \nu_\tau}}{0.8518 \pm 0.0011}{0.8518}{0.0011}%
\htquantdef{Gamma10}{\BR_{10}}{\BRF{\tau^-}{K^- \nu_\tau}}{(0.6957 \pm 0.0096) \cdot 10^{-2}}{0.6957\cdot 10^{-2}}{0.0096\cdot 10^{-2}}%
\htquantdef{Gamma102}{\BR_{102}}{\BRF{\tau^-}{3h^- 2h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0)}}{(9.925 \pm 0.368) \cdot 10^{-4}}{9.925\cdot 10^{-4}}{0.368\cdot 10^{-4}}%
\htquantdef{Gamma103}{\BR_{103}}{\BRF{\tau^-}{3h^- 2h^+ \nu_\tau\;(\text{ex.}K^0)}}{(8.281 \pm 0.314) \cdot 10^{-4}}{8.281\cdot 10^{-4}}{0.314\cdot 10^{-4}}%
\htquantdef{Gamma104}{\BR_{104}}{\BRF{\tau^-}{3h^- 2h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(1.645 \pm 0.114) \cdot 10^{-4}}{1.645\cdot 10^{-4}}{0.114\cdot 10^{-4}}%
\htquantdef{Gamma106}{\BR_{106}}{\BRF{\tau^-}{(5\pi)^- \nu_\tau}}{(0.7793 \pm 0.0534) \cdot 10^{-2}}{0.7793\cdot 10^{-2}}{0.0534\cdot 10^{-2}}%
\htquantdef{Gamma10by5}{\frac{\BR_{10}}{\BR_{5}}}{\frac{\BRF{\tau^-}{K^- \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{(3.906 \pm 0.054) \cdot 10^{-2}}{3.906\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma10by9}{\frac{\BR_{10}}{\BR_{9}}}{\frac{\BRF{\tau^-}{K^- \nu_\tau}}{\BRF{\tau^-}{\pi^- \nu_\tau}}}{(6.437 \pm 0.092) \cdot 10^{-2}}{6.437\cdot 10^{-2}}{0.092\cdot 10^{-2}}%
\htquantdef{Gamma11}{\BR_{11}}{\BRF{\tau^-}{h^- \ge{} 1\,  \text{neutrals}\, \nu_\tau}}{0.36977 \pm 0.00098}{0.36977}{0.00098}%
\htquantdef{Gamma110}{\BR_{110}}{\BRF{\tau^-}{X_s^- \nu_\tau}}{(2.908 \pm 0.048) \cdot 10^{-2}}{2.908\cdot 10^{-2}}{0.048\cdot 10^{-2}}%
\htquantdef{Gamma110_pdg09}{\BR_{110}_pdg09}{}{(2.840 \pm 0.037) \cdot 10^{-2}}{2.840\cdot 10^{-2}}{0.037\cdot 10^{-2}}%
\htquantdef{Gamma12}{\BR_{12}}{\BRF{\tau^-}{h^- \ge{} 1\, \pi^0\, \nu_\tau\;(\text{ex.}K^0)}}{0.36477 \pm 0.00098}{0.36477}{0.00098}%
\htquantdef{Gamma126}{\BR_{126}}{\BRF{\tau^-}{\pi^- \pi^0 \eta \nu_\tau}}{(0.1386 \pm 0.0072) \cdot 10^{-2}}{0.1386\cdot 10^{-2}}{0.0072\cdot 10^{-2}}%
\htquantdef{Gamma128}{\BR_{128}}{\BRF{\tau^-}{K^- \eta \nu_\tau}}{(1.547 \pm 0.080) \cdot 10^{-4}}{1.547\cdot 10^{-4}}{0.080\cdot 10^{-4}}%
\htquantdef{Gamma13}{\BR_{13}}{\BRF{\tau^-}{h^- \pi^0 \nu_\tau}}{0.25918 \pm 0.00090}{0.25918}{0.00090}%
\htquantdef{Gamma130}{\BR_{130}}{\BRF{\tau^-}{K^- \pi^0 \eta \nu_\tau}}{(4.827 \pm 1.161) \cdot 10^{-5}}{4.827\cdot 10^{-5}}{1.161\cdot 10^{-5}}%
\htquantdef{Gamma132}{\BR_{132}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \eta \nu_\tau}}{(9.371 \pm 1.491) \cdot 10^{-5}}{9.371\cdot 10^{-5}}{1.491\cdot 10^{-5}}%
\htquantdef{Gamma136}{\BR_{136}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \eta \nu_\tau\;(\text{ex.}K^0)}}{(2.202 \pm 0.129) \cdot 10^{-4}}{2.202\cdot 10^{-4}}{0.129\cdot 10^{-4}}%
\htquantdef{Gamma14}{\BR_{14}}{\BRF{\tau^-}{\pi^- \pi^0 \nu_\tau}}{0.25486 \pm 0.00090}{0.25486}{0.00090}%
\htquantdef{Gamma149}{\BR_{149}}{\BRF{\tau^-}{h^- \omega \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(2.395 \pm 0.075) \cdot 10^{-2}}{2.395\cdot 10^{-2}}{0.075\cdot 10^{-2}}%
\htquantdef{Gamma150}{\BR_{150}}{\BRF{\tau^-}{h^- \omega \nu_\tau}}{(1.988 \pm 0.064) \cdot 10^{-2}}{1.988\cdot 10^{-2}}{0.064\cdot 10^{-2}}%
\htquantdef{Gamma150by66}{\frac{\BR_{150}}{\BR_{66}}}{\frac{\BRF{\tau^-}{h^- \omega \nu_\tau}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}}{0.4348 \pm 0.0140}{0.4348}{0.0140}%
\htquantdef{Gamma151}{\BR_{151}}{\BRF{\tau^-}{K^- \omega \nu_\tau}}{(4.101 \pm 0.922) \cdot 10^{-4}}{4.101\cdot 10^{-4}}{0.922\cdot 10^{-4}}%
\htquantdef{Gamma152}{\BR_{152}}{\BRF{\tau^-}{h^- \pi^0 \omega \nu_\tau}}{(0.4069 \pm 0.0419) \cdot 10^{-2}}{0.4069\cdot 10^{-2}}{0.0419\cdot 10^{-2}}%
\htquantdef{Gamma152by54}{\frac{\BR_{152}}{\BR_{54}}}{\frac{\BRF{\tau^-}{h^- \omega \pi^0 \nu_\tau}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}}{(2.678 \pm 0.275) \cdot 10^{-2}}{2.678\cdot 10^{-2}}{0.275\cdot 10^{-2}}%
\htquantdef{Gamma152by76}{\frac{\BR_{152}}{\BR_{76}}}{\frac{\BRF{\tau^-}{h^- \omega \pi^0 \nu_\tau}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}}{0.8235 \pm 0.0757}{0.8235}{0.0757}%
\htquantdef{Gamma16}{\BR_{16}}{\BRF{\tau^-}{K^- \pi^0 \nu_\tau}}{(0.4322 \pm 0.0148) \cdot 10^{-2}}{0.4322\cdot 10^{-2}}{0.0148\cdot 10^{-2}}%
\htquantdef{Gamma167}{\BR_{167}}{\BRF{\tau^-}{K^- \phi \nu_\tau}}{(4.408 \pm 1.626) \cdot 10^{-5}}{4.408\cdot 10^{-5}}{1.626\cdot 10^{-5}}%
\htquantdef{Gamma168}{\BR_{168}}{\BRF{\tau^-}{K^- \phi(K^+ K^-) \nu_\tau}}{(2.169 \pm 0.800) \cdot 10^{-5}}{2.169\cdot 10^{-5}}{0.800\cdot 10^{-5}}%
\htquantdef{Gamma169}{\BR_{169}}{\BRF{\tau^-}{K^- \phi(K_S^0 K_L^0) \nu_\tau}}{(1.499 \pm 0.553) \cdot 10^{-5}}{1.499\cdot 10^{-5}}{0.553\cdot 10^{-5}}%
\htquantdef{Gamma17}{\BR_{17}}{\BRF{\tau^-}{h^- \ge{} 2\,  \pi^0\, \nu_\tau}}{0.10794 \pm 0.00097}{0.10794}{0.00097}%
\htquantdef{Gamma18}{\BR_{18}}{\BRF{\tau^-}{h^- 2\pi^0 \nu_\tau}}{(9.460 \pm 0.100) \cdot 10^{-2}}{9.460\cdot 10^{-2}}{0.100\cdot 10^{-2}}%
\htquantdef{Gamma19}{\BR_{19}}{\BRF{\tau^-}{h^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(9.309 \pm 0.100) \cdot 10^{-2}}{9.309\cdot 10^{-2}}{0.100\cdot 10^{-2}}%
\htquantdef{Gamma19by13}{\frac{\BR_{19}}{\BR_{13}}}{\frac{\BRF{\tau^-}{h^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{\BRF{\tau^-}{h^- \pi^0 \nu_\tau}}}{0.3592 \pm 0.0045}{0.3592}{0.0045}%
\htquantdef{Gamma2}{\BR_{2}}{\BRF{\tau^-}{particle^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}{0.8452 \pm 0.0010}{0.8452}{0.0010}%
\htquantdef{Gamma20}{\BR_{20}}{\BRF{\tau^-}{\pi^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(9.245 \pm 0.099) \cdot 10^{-2}}{9.245\cdot 10^{-2}}{0.099\cdot 10^{-2}}%
\htquantdef{Gamma23}{\BR_{23}}{\BRF{\tau^-}{K^- 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(6.339 \pm 2.189) \cdot 10^{-4}}{6.339\cdot 10^{-4}}{2.189\cdot 10^{-4}}%
\htquantdef{Gamma24}{\BR_{24}}{\BRF{\tau^-}{h^- \ge{} 3\, \pi^0\, \nu_\tau}}{(1.335 \pm 0.066) \cdot 10^{-2}}{1.335\cdot 10^{-2}}{0.066\cdot 10^{-2}}%
\htquantdef{Gamma25}{\BR_{25}}{\BRF{\tau^-}{h^- \ge{} 3\, \pi^0\, \nu_\tau\;(\text{ex.}K^0)}}{(1.250 \pm 0.066) \cdot 10^{-2}}{1.250\cdot 10^{-2}}{0.066\cdot 10^{-2}}%
\htquantdef{Gamma26}{\BR_{26}}{\BRF{\tau^-}{h^- 3\pi^0 \nu_\tau}}{(1.173 \pm 0.072) \cdot 10^{-2}}{1.173\cdot 10^{-2}}{0.072\cdot 10^{-2}}%
\htquantdef{Gamma26by13}{\frac{\BR_{26}}{\BR_{13}}}{\frac{\BRF{\tau^-}{h^- 3\pi^0 \nu_\tau}}{\BRF{\tau^-}{h^- \pi^0 \nu_\tau}}}{(4.526 \pm 0.278) \cdot 10^{-2}}{4.526\cdot 10^{-2}}{0.278\cdot 10^{-2}}%
\htquantdef{Gamma27}{\BR_{27}}{\BRF{\tau^-}{\pi^- 3\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(1.040 \pm 0.071) \cdot 10^{-2}}{1.040\cdot 10^{-2}}{0.071\cdot 10^{-2}}%
\htquantdef{Gamma28}{\BR_{28}}{\BRF{\tau^-}{K^- 3\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta)}}{(4.648 \pm 2.131) \cdot 10^{-4}}{4.648\cdot 10^{-4}}{2.131\cdot 10^{-4}}%
\htquantdef{Gamma29}{\BR_{29}}{\BRF{\tau^-}{h^- 4\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(0.1587 \pm 0.0391) \cdot 10^{-2}}{0.1587\cdot 10^{-2}}{0.0391\cdot 10^{-2}}%
\htquantdef{Gamma3}{\BR_{3}}{\BRF{\tau^-}{\mu^- \bar{\nu}_\mu \nu_\tau}}{0.17387 \pm 0.00040}{0.17387}{0.00040}%
\htquantdef{Gamma30}{\BR_{30}}{\BRF{\tau^-}{h^- 4\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta)}}{(0.1118 \pm 0.0391) \cdot 10^{-2}}{0.1118\cdot 10^{-2}}{0.0391\cdot 10^{-2}}%
\htquantdef{Gamma31}{\BR_{31}}{\BRF{\tau^-}{K^- \ge{} 0\, \pi^0 \ge{} 0\, K^0 \ge{} 0\, \gamma \nu_\tau}}{(1.548 \pm 0.029) \cdot 10^{-2}}{1.548\cdot 10^{-2}}{0.029\cdot 10^{-2}}%
\htquantdef{Gamma32}{\BR_{32}}{\BRF{\tau^-}{K^- \ge{} 1\, (\pi^0\,\text{or}\,K^0\,\text{or}\,\gamma) \nu_\tau}}{(0.8556 \pm 0.0282) \cdot 10^{-2}}{0.8556\cdot 10^{-2}}{0.0282\cdot 10^{-2}}%
\htquantdef{Gamma33}{\BR_{33}}{\BRF{\tau^-}{K_S^0 (\text{particles})^- \nu_\tau}}{(0.9370 \pm 0.0292) \cdot 10^{-2}}{0.9370\cdot 10^{-2}}{0.0292\cdot 10^{-2}}%
\htquantdef{Gamma34}{\BR_{34}}{\BRF{\tau^-}{h^- \bar{K}^0 \nu_\tau}}{(0.9861 \pm 0.0138) \cdot 10^{-2}}{0.9861\cdot 10^{-2}}{0.0138\cdot 10^{-2}}%
\htquantdef{Gamma35}{\BR_{35}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \nu_\tau}}{(0.8375 \pm 0.0139) \cdot 10^{-2}}{0.8375\cdot 10^{-2}}{0.0139\cdot 10^{-2}}%
\htquantdef{Gamma37}{\BR_{37}}{\BRF{\tau^-}{K^- K^0 \nu_\tau}}{(0.1486 \pm 0.0034) \cdot 10^{-2}}{0.1486\cdot 10^{-2}}{0.0034\cdot 10^{-2}}%
\htquantdef{Gamma38}{\BR_{38}}{\BRF{\tau^-}{K^- K^0 \ge{} 0\,  \pi^0\, \nu_\tau}}{(0.2985 \pm 0.0073) \cdot 10^{-2}}{0.2985\cdot 10^{-2}}{0.0073\cdot 10^{-2}}%
\htquantdef{Gamma39}{\BR_{39}}{\BRF{\tau^-}{h^- \bar{K}^0 \pi^0 \nu_\tau}}{(0.5310 \pm 0.0134) \cdot 10^{-2}}{0.5310\cdot 10^{-2}}{0.0134\cdot 10^{-2}}%
\htquantdef{Gamma3by5}{\frac{\BR_{3}}{\BR_{5}}}{\frac{\BRF{\tau^-}{\mu^- \bar{\nu}_\mu \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{0.9762 \pm 0.0028}{0.9762}{0.0028}%
\htquantdef{Gamma40}{\BR_{40}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \pi^0 \nu_\tau}}{(0.3810 \pm 0.0129) \cdot 10^{-2}}{0.3810\cdot 10^{-2}}{0.0129\cdot 10^{-2}}%
\htquantdef{Gamma42}{\BR_{42}}{\BRF{\tau^-}{K^- K^0 \pi^0 \nu_\tau}}{(0.1499 \pm 0.0070) \cdot 10^{-2}}{0.1499\cdot 10^{-2}}{0.0070\cdot 10^{-2}}%
\htquantdef{Gamma43}{\BR_{43}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \ge{} 1\,  \pi^0\, \nu_\tau}}{(0.4045 \pm 0.0260) \cdot 10^{-2}}{0.4045\cdot 10^{-2}}{0.0260\cdot 10^{-2}}%
\htquantdef{Gamma44}{\BR_{44}}{\BRF{\tau^-}{\pi^- \bar{K}^0 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(2.342 \pm 2.306) \cdot 10^{-4}}{2.342\cdot 10^{-4}}{2.306\cdot 10^{-4}}%
\htquantdef{Gamma46}{\BR_{46}}{\BRF{\tau^-}{\pi^- K^0 \bar{K}^0 \nu_\tau}}{(0.1517 \pm 0.0247) \cdot 10^{-2}}{0.1517\cdot 10^{-2}}{0.0247\cdot 10^{-2}}%
\htquantdef{Gamma47}{\BR_{47}}{\BRF{\tau^-}{\pi^- K_S^0 K_S^0 \nu_\tau}}{(2.349 \pm 0.065) \cdot 10^{-4}}{2.349\cdot 10^{-4}}{0.065\cdot 10^{-4}}%
\htquantdef{Gamma48}{\BR_{48}}{\BRF{\tau^-}{\pi^- K_S^0 K_L^0 \nu_\tau}}{(0.1048 \pm 0.0247) \cdot 10^{-2}}{0.1048\cdot 10^{-2}}{0.0247\cdot 10^{-2}}%
\htquantdef{Gamma49}{\BR_{49}}{\BRF{\tau^-}{\pi^- \pi^0 K^0 \bar{K}^0 \nu_\tau}}{(3.543 \pm 1.193) \cdot 10^{-4}}{3.543\cdot 10^{-4}}{1.193\cdot 10^{-4}}%
\htquantdef{Gamma5}{\BR_{5}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}{0.17811 \pm 0.00041}{0.17811}{0.00041}%
\htquantdef{Gamma50}{\BR_{50}}{\BRF{\tau^-}{\pi^- K_S^0 K_S^0 \pi^0 \nu_\tau}}{(1.820 \pm 0.207) \cdot 10^{-5}}{1.820\cdot 10^{-5}}{0.207\cdot 10^{-5}}%
\htquantdef{Gamma51}{\BR_{51}}{\BRF{\tau^-}{\pi^- K_S^0 K_L^0 \pi^0 \nu_\tau}}{(3.179 \pm 1.192) \cdot 10^{-4}}{3.179\cdot 10^{-4}}{1.192\cdot 10^{-4}}%
\htquantdef{Gamma53}{\BR_{53}}{\BRF{\tau^-}{\bar{K}^0 h^- h^- h^+ \nu_\tau}}{(2.223 \pm 2.024) \cdot 10^{-4}}{2.223\cdot 10^{-4}}{2.024\cdot 10^{-4}}%
\htquantdef{Gamma54}{\BR_{54}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}{0.15193 \pm 0.00063}{0.15193}{0.00063}%
\htquantdef{Gamma55}{\BR_{55}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0)}}{0.14545 \pm 0.00058}{0.14545}{0.00058}%
\htquantdef{Gamma56}{\BR_{56}}{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau}}{(9.790 \pm 0.055) \cdot 10^{-2}}{9.790\cdot 10^{-2}}{0.055\cdot 10^{-2}}%
\htquantdef{Gamma57}{\BR_{57}}{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0)}}{(9.449 \pm 0.054) \cdot 10^{-2}}{9.449\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma57by55}{\frac{\BR_{57}}{\BR_{55}}}{\frac{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0)}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.}K^0)}}}{0.6496 \pm 0.0031}{0.6496}{0.0031}%
\htquantdef{Gamma58}{\BR_{58}}{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau\;(\text{ex.}K^0,\omega)}}{(9.419 \pm 0.054) \cdot 10^{-2}}{9.419\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma59}{\BR_{59}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau}}{(9.300 \pm 0.052) \cdot 10^{-2}}{9.300\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma60}{\BR_{60}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0)}}{(9.010 \pm 0.052) \cdot 10^{-2}}{9.010\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma62}{\BR_{62}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0,\omega)}}{(8.981 \pm 0.052) \cdot 10^{-2}}{8.981\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma63}{\BR_{63}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 1\,  \text{neutrals}\, \nu_\tau}}{(5.293 \pm 0.052) \cdot 10^{-2}}{5.293\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma64}{\BR_{64}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 1\,  \pi^0\, \nu_\tau\;(\text{ex.}K^0)}}{(5.088 \pm 0.052) \cdot 10^{-2}}{5.088\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma65}{\BR_{65}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau}}{(4.757 \pm 0.054) \cdot 10^{-2}}{4.757\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma66}{\BR_{66}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(4.573 \pm 0.054) \cdot 10^{-2}}{4.573\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma67}{\BR_{67}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega)}}{(2.791 \pm 0.071) \cdot 10^{-2}}{2.791\cdot 10^{-2}}{0.071\cdot 10^{-2}}%
\htquantdef{Gamma68}{\BR_{68}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau}}{(4.620 \pm 0.054) \cdot 10^{-2}}{4.620\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma69}{\BR_{69}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(4.488 \pm 0.054) \cdot 10^{-2}}{4.488\cdot 10^{-2}}{0.054\cdot 10^{-2}}%
\htquantdef{Gamma7}{\BR_{7}}{\BRF{\tau^-}{h^- \ge{} 0\,  K_L^0\, \nu_\tau}}{0.12020 \pm 0.00055}{0.12020}{0.00055}%
\htquantdef{Gamma70}{\BR_{70}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega)}}{(2.743 \pm 0.071) \cdot 10^{-2}}{2.743\cdot 10^{-2}}{0.071\cdot 10^{-2}}%
\htquantdef{Gamma74}{\BR_{74}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 2\, \pi^0\, \nu_\tau\;(\text{ex.}K^0)}}{(0.5154 \pm 0.0312) \cdot 10^{-2}}{0.5154\cdot 10^{-2}}{0.0312\cdot 10^{-2}}%
\htquantdef{Gamma75}{\BR_{75}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau}}{(0.5041 \pm 0.0311) \cdot 10^{-2}}{0.5041\cdot 10^{-2}}{0.0311\cdot 10^{-2}}%
\htquantdef{Gamma76}{\BR_{76}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(0.4942 \pm 0.0311) \cdot 10^{-2}}{0.4942\cdot 10^{-2}}{0.0311\cdot 10^{-2}}%
\htquantdef{Gamma76by54}{\frac{\BR_{76}}{\BR_{54}}}{\frac{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}}{(3.252 \pm 0.203) \cdot 10^{-2}}{3.252\cdot 10^{-2}}{0.203\cdot 10^{-2}}%
\htquantdef{Gamma77}{\BR_{77}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.}K^0,\omega,\eta)}}{(9.790 \pm 3.562) \cdot 10^{-4}}{9.790\cdot 10^{-4}}{3.562\cdot 10^{-4}}%
\htquantdef{Gamma78}{\BR_{78}}{\BRF{\tau^-}{h^- h^- h^+ 3\pi^0 \nu_\tau}}{(2.124 \pm 0.299) \cdot 10^{-4}}{2.124\cdot 10^{-4}}{0.299\cdot 10^{-4}}%
\htquantdef{Gamma79}{\BR_{79}}{\BRF{\tau^-}{K^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(0.6276 \pm 0.0140) \cdot 10^{-2}}{0.6276\cdot 10^{-2}}{0.0140\cdot 10^{-2}}%
\htquantdef{Gamma8}{\BR_{8}}{\BRF{\tau^-}{h^- \nu_\tau}}{0.11504 \pm 0.00054}{0.11504}{0.00054}%
\htquantdef{Gamma80}{\BR_{80}}{\BRF{\tau^-}{K^- \pi^- h^+ \nu_\tau\;(\text{ex.}K^0)}}{(0.4364 \pm 0.0073) \cdot 10^{-2}}{0.4364\cdot 10^{-2}}{0.0073\cdot 10^{-2}}%
\htquantdef{Gamma800}{\BR_{800}}{\BRF{\tau^-}{\pi^- \omega \nu_\tau}}{(1.947 \pm 0.065) \cdot 10^{-2}}{1.947\cdot 10^{-2}}{0.065\cdot 10^{-2}}%
\htquantdef{Gamma802}{\BR_{802}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \nu_\tau\;(\text{ex.}K^0,\omega)}}{(0.2924 \pm 0.0068) \cdot 10^{-2}}{0.2924\cdot 10^{-2}}{0.0068\cdot 10^{-2}}%
\htquantdef{Gamma803}{\BR_{803}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\omega,\eta)}}{(3.874 \pm 1.423) \cdot 10^{-4}}{3.874\cdot 10^{-4}}{1.423\cdot 10^{-4}}%
\htquantdef{Gamma804}{\BR_{804}}{\BRF{\tau^-}{\pi^- K_L^0 K_L^0 \nu_\tau}}{(2.349 \pm 0.065) \cdot 10^{-4}}{2.349\cdot 10^{-4}}{0.065\cdot 10^{-4}}%
\htquantdef{Gamma805}{\BR_{805}}{\BRF{\tau^-}{a_1^-(\pi^- \gamma) \nu_\tau}}{(4.000 \pm 2.000) \cdot 10^{-4}}{4.000\cdot 10^{-4}}{2.000\cdot 10^{-4}}%
\htquantdef{Gamma806}{\BR_{806}}{\BRF{\tau^-}{\pi^- K_L^0 K_L^0 \pi^0 \nu_\tau}}{(1.820 \pm 0.207) \cdot 10^{-5}}{1.820\cdot 10^{-5}}{0.207\cdot 10^{-5}}%
\htquantdef{Gamma80by60}{\frac{\BR_{80}}{\BR_{60}}}{\frac{\BRF{\tau^-}{K^- \pi^- h^+ \nu_\tau\;(\text{ex.}K^0)}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0)}}}{(4.843 \pm 0.079) \cdot 10^{-2}}{4.843\cdot 10^{-2}}{0.079\cdot 10^{-2}}%
\htquantdef{Gamma81}{\BR_{81}}{\BRF{\tau^-}{K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(8.498 \pm 1.169) \cdot 10^{-4}}{8.498\cdot 10^{-4}}{1.169\cdot 10^{-4}}%
\htquantdef{Gamma810}{\BR_{810}}{\BRF{\tau^-}{2\pi^- \pi^+ 3\pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(1.940 \pm 0.298) \cdot 10^{-4}}{1.940\cdot 10^{-4}}{0.298\cdot 10^{-4}}%
\htquantdef{Gamma811}{\BR_{811}}{\BRF{\tau^-}{\pi^- 2\pi^0 \omega \nu_\tau}}{(7.164 \pm 1.586) \cdot 10^{-5}}{7.164\cdot 10^{-5}}{1.586\cdot 10^{-5}}%
\htquantdef{Gamma812}{\BR_{812}}{\BRF{\tau^-}{2\pi^- \pi^+ 3\pi^0 \nu_\tau\;(\text{ex.}K^0,\eta,\omega,f_1)}}{(1.353 \pm 2.683) \cdot 10^{-5}}{1.353\cdot 10^{-5}}{2.683\cdot 10^{-5}}%
\htquantdef{Gamma81by69}{\frac{\BR_{81}}{\BR_{69}}}{\frac{\BRF{\tau^-}{K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0)}}}{(1.893 \pm 0.264) \cdot 10^{-2}}{1.893\cdot 10^{-2}}{0.264\cdot 10^{-2}}%
\htquantdef{Gamma82}{\BR_{82}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(0.4759 \pm 0.0136) \cdot 10^{-2}}{0.4759\cdot 10^{-2}}{0.0136\cdot 10^{-2}}%
\htquantdef{Gamma820}{\BR_{820}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0,\omega)}}{(8.262 \pm 0.313) \cdot 10^{-4}}{8.262\cdot 10^{-4}}{0.313\cdot 10^{-4}}%
\htquantdef{Gamma821}{\BR_{821}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0,\omega,f_1)}}{(7.738 \pm 0.295) \cdot 10^{-4}}{7.738\cdot 10^{-4}}{0.295\cdot 10^{-4}}%
\htquantdef{Gamma822}{\BR_{822}}{\BRF{\tau^-}{K^- 2\pi^- 2\pi^+ \nu_\tau\;(\text{ex.}K^0)}}{(0.593 \pm 1.208) \cdot 10^{-6}}{0.593\cdot 10^{-6}}{1.208\cdot 10^{-6}}%
\htquantdef{Gamma83}{\BR_{83}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \ge{} 0\,  \pi^0\, \nu_\tau\;(\text{ex.}K^0)}}{(0.3719 \pm 0.0134) \cdot 10^{-2}}{0.3719\cdot 10^{-2}}{0.0134\cdot 10^{-2}}%
\htquantdef{Gamma830}{\BR_{830}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(1.633 \pm 0.113) \cdot 10^{-4}}{1.633\cdot 10^{-4}}{0.113\cdot 10^{-4}}%
\htquantdef{Gamma831}{\BR_{831}}{\BRF{\tau^-}{2\pi^- \pi^+ \omega \nu_\tau\;(\text{ex.}K^0)}}{(8.417 \pm 0.624) \cdot 10^{-5}}{8.417\cdot 10^{-5}}{0.624\cdot 10^{-5}}%
\htquantdef{Gamma832}{\BR_{832}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\eta,\omega,f_1)}}{(3.772 \pm 0.874) \cdot 10^{-5}}{3.772\cdot 10^{-5}}{0.874\cdot 10^{-5}}%
\htquantdef{Gamma833}{\BR_{833}}{\BRF{\tau^-}{K^- 2\pi^- 2\pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(1.107 \pm 0.566) \cdot 10^{-6}}{1.107\cdot 10^{-6}}{0.566\cdot 10^{-6}}%
\htquantdef{Gamma84}{\BR_{84}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \nu_\tau}}{(0.3444 \pm 0.0069) \cdot 10^{-2}}{0.3444\cdot 10^{-2}}{0.0069\cdot 10^{-2}}%
\htquantdef{Gamma85}{\BR_{85}}{\BRF{\tau^-}{K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0)}}{(0.2930 \pm 0.0068) \cdot 10^{-2}}{0.2930\cdot 10^{-2}}{0.0068\cdot 10^{-2}}%
\htquantdef{Gamma85by60}{\frac{\BR_{85}}{\BR_{60}}}{\frac{\BRF{\tau^-}{K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0)}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0)}}}{(3.252 \pm 0.074) \cdot 10^{-2}}{3.252\cdot 10^{-2}}{0.074\cdot 10^{-2}}%
\htquantdef{Gamma87}{\BR_{87}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau}}{(0.1308 \pm 0.0119) \cdot 10^{-2}}{0.1308\cdot 10^{-2}}{0.0119\cdot 10^{-2}}%
\htquantdef{Gamma88}{\BR_{88}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0)}}{(7.891 \pm 1.161) \cdot 10^{-4}}{7.891\cdot 10^{-4}}{1.161\cdot 10^{-4}}%
\htquantdef{Gamma89}{\BR_{89}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.}K^0,\eta)}}{(7.536 \pm 1.161) \cdot 10^{-4}}{7.536\cdot 10^{-4}}{1.161\cdot 10^{-4}}%
\htquantdef{Gamma8by5}{\frac{\BR_{8}}{\BR_{5}}}{\frac{\BRF{\tau^-}{h^- \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{0.6459 \pm 0.0033}{0.6459}{0.0033}%
\htquantdef{Gamma9}{\BR_{9}}{\BRF{\tau^-}{\pi^- \nu_\tau}}{0.10808 \pm 0.00053}{0.10808}{0.00053}%
\htquantdef{Gamma910}{\BR_{910}}{\BRF{\tau^-}{2\pi^- \pi^+ \eta(3\pi^0) \nu_\tau\;(\text{ex.}K^0)}}{(7.195 \pm 0.422) \cdot 10^{-5}}{7.195\cdot 10^{-5}}{0.422\cdot 10^{-5}}%
\htquantdef{Gamma911}{\BR_{911}}{\BRF{\tau^-}{\pi^- 2\pi^0 \eta(\pi^+ \pi^- \pi^0) \nu_\tau\;(\text{ex.}K^0)}}{(4.457 \pm 0.867) \cdot 10^{-5}}{4.457\cdot 10^{-5}}{0.867\cdot 10^{-5}}%
\htquantdef{Gamma92}{\BR_{92}}{\BRF{\tau^-}{\pi^- K^- K^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(0.1495 \pm 0.0033) \cdot 10^{-2}}{0.1495\cdot 10^{-2}}{0.0033\cdot 10^{-2}}%
\htquantdef{Gamma920}{\BR_{920}}{\BRF{\tau^-}{\pi^- f_1(2\pi^- 2\pi^+) \nu_\tau}}{(5.237 \pm 0.444) \cdot 10^{-5}}{5.237\cdot 10^{-5}}{0.444\cdot 10^{-5}}%
\htquantdef{Gamma93}{\BR_{93}}{\BRF{\tau^-}{\pi^- K^- K^+ \nu_\tau}}{(0.1434 \pm 0.0027) \cdot 10^{-2}}{0.1434\cdot 10^{-2}}{0.0027\cdot 10^{-2}}%
\htquantdef{Gamma930}{\BR_{930}}{\BRF{\tau^-}{2\pi^- \pi^+ \eta(\pi^+ \pi^- \pi^0) \nu_\tau\;(\text{ex.}K^0)}}{(5.046 \pm 0.296) \cdot 10^{-5}}{5.046\cdot 10^{-5}}{0.296\cdot 10^{-5}}%
\htquantdef{Gamma93by60}{\frac{\BR_{93}}{\BR_{60}}}{\frac{\BRF{\tau^-}{\pi^- K^- K^+ \nu_\tau}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.}K^0)}}}{(1.592 \pm 0.030) \cdot 10^{-2}}{1.592\cdot 10^{-2}}{0.030\cdot 10^{-2}}%
\htquantdef{Gamma94}{\BR_{94}}{\BRF{\tau^-}{\pi^- K^- K^+ \pi^0 \nu_\tau}}{(6.069 \pm 1.829) \cdot 10^{-5}}{6.069\cdot 10^{-5}}{1.829\cdot 10^{-5}}%
\htquantdef{Gamma944}{\BR_{944}}{\BRF{\tau^-}{2\pi^- \pi^+ \eta(\gamma \gamma) \nu_\tau\;(\text{ex.}K^0)}}{(8.676 \pm 0.509) \cdot 10^{-5}}{8.676\cdot 10^{-5}}{0.509\cdot 10^{-5}}%
\htquantdef{Gamma945}{\BR_{945}}{\BRF{\tau^-}{\pi^- 2\pi^0 \eta \nu_\tau\;(\text{ex.}K^0)}}{(1.945 \pm 0.378) \cdot 10^{-4}}{1.945\cdot 10^{-4}}{0.378\cdot 10^{-4}}%
\htquantdef{Gamma94by69}{\frac{\BR_{94}}{\BR_{69}}}{\frac{\BRF{\tau^-}{\pi^- K^- K^+ \pi^0 \nu_\tau}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.}K^0)}}}{(0.1352 \pm 0.0408) \cdot 10^{-2}}{0.1352\cdot 10^{-2}}{0.0408\cdot 10^{-2}}%
\htquantdef{Gamma96}{\BR_{96}}{\BRF{\tau^-}{K^- K^- K^+ \nu_\tau}}{(2.169 \pm 0.800) \cdot 10^{-5}}{2.169\cdot 10^{-5}}{0.800\cdot 10^{-5}}%
\htquantdef{Gamma998}{\BR_{998}}{1 - \BR_{\text{All}}}{(0.0684 \pm 0.1068) \cdot 10^{-2}}{0.0684\cdot 10^{-2}}{0.1068\cdot 10^{-2}}%
\htquantdef{Gamma9by5}{\frac{\BR_{9}}{\BR_{5}}}{\frac{\BRF{\tau^-}{\pi^- \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{0.6068 \pm 0.0032}{0.6068}{0.0032}%
\htquantdef{GammaAll}{\BR_{\text{all}}}{\BRF{\tau^-}{\text{all}}}{0.9993 \pm 0.0011}{0.9993}{0.0011}%
\htquantdef{gf}{gf}{CODATA 2018 Fermi coupling constant}{(1.16637870 \pm 0.00000060) \cdot 10^{-5}}{1.16637870\cdot 10^{-5}}{0.00000060\cdot 10^{-5}}%
\htquantdef{gmubyge_tau}{gmubyge_tau}{}{1.0019 \pm 0.0014}{1.0019}{0.0014}%
\htquantdef{gtaubyge_tau}{gtaubyge_tau}{}{1.0027 \pm 0.0014}{1.0027}{0.0014}%
\htquantdef{gtaubygemu_tau}{gtaubygemu_tau}{}{1.0018 \pm 0.0013}{1.0018}{0.0013}%
\htquantdef{gtaubygemu_tau_syst_Be_lept_perc}{gtaubygemu_tau_syst_Be_lept_perc}{}{0.090}{0.090}{0}%
\htquantdef{gtaubygemu_tau_syst_m_tau_perc}{gtaubygemu_tau_syst_m_tau_perc}{}{0.017}{0.017}{0}%
\htquantdef{gtaubygemu_tau_syst_tau_tau_perc}{gtaubygemu_tau_syst_tau_tau_perc}{}{0.086}{0.086}{0}%
\htquantdef{gtaubygemu_tau_unc_perc}{gtaubygemu_tau_unc_perc}{}{0.126}{0.126}{0}%
\htquantdef{gtaubygmu_fit}{gtaubygmu_fit}{}{1.0003 \pm 0.0014}{1.0003}{0.0014}%
\htquantdef{gtaubygmu_K}{gtaubygmu_K}{}{0.9855 \pm 0.0075}{0.9855}{0.0075}%
\htquantdef{gtaubygmu_pi}{gtaubygmu_pi}{}{0.9959 \pm 0.0038}{0.9959}{0.0038}%
\htquantdef{gtaubygmu_piK_fit}{gtaubygmu_piK_fit}{}{0.9939 \pm 0.0035}{0.9939}{0.0035}%
\htquantdef{gtaubygmu_tau}{gtaubygmu_tau}{}{1.0009 \pm 0.0014}{1.0009}{0.0014}%
\htquantdef{hbarev}{hbarev}{CODATA 2018 reduced Planck constant in eV s}{6.582\cdot 10^{-16}}{6.582\cdot 10^{-16}}{0}%
\htquantdef{KmKzsNu}{KmKzsNu}{}{7.430\cdot 10^{-4}}{7.430\cdot 10^{-4}}{0}%
\htquantdef{KmPizKzsNu}{KmPizKzsNu}{}{7.500\cdot 10^{-4}}{7.500\cdot 10^{-4}}{0}%
\htquantdef{KtoENu}{KtoENu}{}{(1.5820 \pm 0.0070) \cdot 10^{-5}}{1.5820\cdot 10^{-5}}{0.0070\cdot 10^{-5}}%
\htquantdef{KtoMuNu}{KtoMuNu}{}{0.6356 \pm 0.0011}{0.6356}{0.0011}%
\htquantdef{m_e}{m_e}{}{0.5109989461 \pm 0.0000000031}{0.5109989461}{0.0000000031}%
\htquantdef{m_K}{m_K}{}{493.677 \pm 0.016}{493.677}{0.016}%
\htquantdef{m_mu}{m_mu}{}{105.6583745 \pm 0.0000024}{105.6583745}{0.0000024}%
\htquantdef{m_pi}{m_pi}{}{139.57039 \pm 0.00018}{139.57039}{0.00018}%
\htquantdef{m_s}{m_s}{}{93.00 \pm 8.54}{93.00}{8.54}%
\htquantdef{m_tau}{m_tau}{}{(1.77686 \pm 0.00012) \cdot 10^{3}}{1.77686\cdot 10^{3}}{0.00012\cdot 10^{3}}%
\htquantdef{m_tau_unc_perc}{m_tau_unc_perc}{}{0.007}{0.007}{0}%
\htquantdef{m_W}{m_W}{}{(8.0379 \pm 0.0012) \cdot 10^{4}}{8.0379\cdot 10^{4}}{0.0012\cdot 10^{4}}%
\htquantdef{MumNuNumb}{MumNuNumb}{}{0.1739}{0.1739}{0}%
\htquantdef{phspf_mebymmu}{phspf_mebymmu}{}{0.9998129491711 \pm 0.0000000000088}{0.9998129491711}{0.0000000000088}%
\htquantdef{phspf_mebymtau}{phspf_mebymtau}{}{0.999999338359 \pm 0.000000000089}{0.999999338359}{0.000000000089}%
\htquantdef{phspf_mmubymtau}{phspf_mmubymtau}{}{0.9725600 \pm 0.0000036}{0.9725600}{0.0000036}%
\htquantdef{PimKmKpNu}{PimKmKpNu}{}{0.1435\cdot 10^{-2}}{0.1435\cdot 10^{-2}}{0}%
\htquantdef{PimKmPipNu}{PimKmPipNu}{}{0.2930\cdot 10^{-2}}{0.2930\cdot 10^{-2}}{0}%
\htquantdef{PimKzsKzlNu}{PimKzsKzlNu}{}{0.1080\cdot 10^{-2}}{0.1080\cdot 10^{-2}}{0}%
\htquantdef{PimKzsKzsNu}{PimKzsKzsNu}{}{2.330\cdot 10^{-4}}{2.330\cdot 10^{-4}}{0}%
\htquantdef{PimPimPipNu}{PimPimPipNu}{}{8.990\cdot 10^{-2}}{8.990\cdot 10^{-2}}{0}%
\htquantdef{PimPimPipPizNu}{PimPimPipPizNu}{}{4.620\cdot 10^{-2}}{4.620\cdot 10^{-2}}{0}%
\htquantdef{PimPizKzsNu}{PimPizKzsNu}{}{0.1910\cdot 10^{-2}}{0.1910\cdot 10^{-2}}{0}%
\htquantdef{PimPizNu}{PimPizNu}{}{0.2549}{0.2549}{0}%
\htquantdef{pitoENu}{pitoENu}{}{(1.2300 \pm 0.0040) \cdot 10^{-4}}{1.2300\cdot 10^{-4}}{0.0040\cdot 10^{-4}}%
\htquantdef{pitoMuNu}{pitoMuNu}{}{0.99987700 \pm 0.00000040}{0.99987700}{0.00000040}%
\htquantdef{R_tau}{R_tau}{}{3.6343 \pm 0.0082}{3.6343}{0.0082}%
\htquantdef{R_tau_leptonly}{R_tau_leptonly}{}{3.6381 \pm 0.0075}{3.6381}{0.0075}%
\htquantdef{R_tau_leptuniv}{R_tau_leptuniv}{}{3.6417 \pm 0.0070}{3.6417}{0.0070}%
\htquantdef{R_tau_s}{R_tau_s}{}{0.1632 \pm 0.0027}{0.1632}{0.0027}%
\htquantdef{R_tau_uni}{R_tau_uni}{}{3.6381 \pm 0.0075}{3.6381}{0.0075}%
\htquantdef{R_tau_uni_SM}{R_tau_uni_SM}{}{3.6417 \pm 0.0070}{3.6417}{0.0070}%
\htquantdef{R_tau_VA}{R_tau_VA}{}{3.4710 \pm 0.0079}{3.4710}{0.0079}%
\htquantdef{Rrad_mu_gamma}{Rrad_mu_gamma}{}{0.9958}{0.9958}{0}%
\htquantdef{Rrad_mu_W}{Rrad_mu_W}{}{1.00000103682 \pm 0.00000000031}{1.00000103682}{0.00000000031}%
\htquantdef{Rrad_tau_gamma}{Rrad_tau_gamma}{}{0.9957}{0.9957}{0}%
\htquantdef{Rrad_tau_W}{Rrad_tau_W}{}{1.000296316 \pm 0.000000097}{1.000296316}{0.000000097}%
\htquantdef{S_EW}{S_EW}{}{1.02320 \pm 0.00030}{1.02320}{0.00030}%
\htquantdef{sigmataupmy4s}{sigmataupmy4s}{}{0.9190}{0.9190}{0}%
\htquantdef{tau_K}{tau_K}{}{(1.2380 \pm 0.0020) \cdot 10^{-8}}{1.2380\cdot 10^{-8}}{0.0020\cdot 10^{-8}}%
\htquantdef{tau_mu}{tau_mu}{}{(2.196981 \pm 0.000022) \cdot 10^{-6}}{2.196981\cdot 10^{-6}}{0.000022\cdot 10^{-6}}%
\htquantdef{tau_pi}{tau_pi}{}{(2.60330 \pm 0.00050) \cdot 10^{-8}}{2.60330\cdot 10^{-8}}{0.00050\cdot 10^{-8}}%
\htquantdef{tau_tau}{tau_tau}{}{290.3 \pm 0.5}{290.3}{0.5}%
\htquantdef{tau_tau_unc_perc}{tau_tau_unc_perc}{}{0.172}{0.172}{0}%
\htquantdef{Vub}{Vub}{}{(0.3820 \pm 0.0240) \cdot 10^{-2}}{0.3820\cdot 10^{-2}}{0.0240\cdot 10^{-2}}%
\htquantdef{Vud}{Vud}{}{0.97373 \pm 0.00031}{0.97373}{0.00031}%
\htquantdef{Vus}{Vus}{}{0.2184 \pm 0.0021}{0.2184}{0.0021}%
\htquantdef{Vus_by_Vud_tauKpi}{Vus_by_Vud_tauKpi}{}{0.2289 \pm 0.0019}{0.2289}{0.0019}%
\htquantdef{Vus_by_Vud_tauXs}{Vus_by_Vud_tauXs}{}{0.2243 \pm 0.0022}{0.2243}{0.0022}%
\htquantdef{Vus_err_exp}{Vus_err_exp}{}{0.1827\cdot 10^{-2}}{0.1827\cdot 10^{-2}}{0}%
\htquantdef{Vus_err_exp_perc}{Vus_err_exp_perc}{}{0.8367}{0.8367}{0}%
\htquantdef{Vus_err_perc}{Vus_err_perc}{}{0.9673}{0.9673}{0}%
\htquantdef{Vus_err_th}{Vus_err_th}{}{0.0011}{0.0011}{0}%
\htquantdef{Vus_err_th_perc}{Vus_err_th_perc}{}{0.49}{0.49}{0}%
\htquantdef{Vus_Kl2}{Vus_Kl2}{}{0.22520 \pm 0.00050}{0.22520}{0.00050}%
\htquantdef{Vus_Kl3}{Vus_Kl3}{}{0.22309 \pm 0.00056}{0.22309}{0.00056}%
\htquantdef{Vus_mism}{Vus_mism}{}{(-0.9283 \pm 0.2533) \cdot 10^{-2}}{-0.9283\cdot 10^{-2}}{0.2533\cdot 10^{-2}}%
\htquantdef{Vus_mism_sigma}{Vus_mism_sigma}{}{-3.7}{-3.7}{0}%
\htquantdef{Vus_mism_sigma_abs}{Vus_mism_sigma_abs}{}{3.7}{3.7}{0}%
\htquantdef{Vus_tau}{Vus_tau}{}{0.2207 \pm 0.0014}{0.2207}{0.0014}%
\htquantdef{Vus_tau_excl}{Vus_tau_excl}{}{0.2222 \pm 0.0017}{0.2222}{0.0017}%
\htquantdef{Vus_tau_excl_mism}{Vus_tau_excl_mism}{}{(-0.5495 \pm 0.2173) \cdot 10^{-2}}{-0.5495\cdot 10^{-2}}{0.2173\cdot 10^{-2}}%
\htquantdef{Vus_tau_excl_mism_sigma}{Vus_tau_excl_mism_sigma}{}{-2.5}{-2.5}{0}%
\htquantdef{Vus_tau_excl_mism_sigma_abs}{Vus_tau_excl_mism_sigma_abs}{}{2.5}{2.5}{0}%
\htquantdef{Vus_tau_mism}{Vus_tau_mism}{}{(-0.6926 \pm 0.1968) \cdot 10^{-2}}{-0.6926\cdot 10^{-2}}{0.1968\cdot 10^{-2}}%
\htquantdef{Vus_tau_mism_sigma}{Vus_tau_mism_sigma}{}{-3.5}{-3.5}{0}%
\htquantdef{Vus_tau_mism_sigma_abs}{Vus_tau_mism_sigma_abs}{}{3.5}{3.5}{0}%
\htquantdef{Vus_tau2}{Vus_tau2}{}{0.2209 \pm 0.0015}{0.2209}{0.0015}%
\htquantdef{Vus_tau2_mism}{Vus_tau2_mism}{}{(-0.6926 \pm 0.1968) \cdot 10^{-2}}{-0.6926\cdot 10^{-2}}{0.1968\cdot 10^{-2}}%
\htquantdef{Vus_tau2_mism_sigma}{Vus_tau2_mism_sigma}{}{-3.5}{-3.5}{0}%
\htquantdef{Vus_tau2_mism_sigma_abs}{Vus_tau2_mism_sigma_abs}{}{3.5}{3.5}{0}%
\htquantdef{Vus_tauKnu}{Vus_tauKnu}{}{0.2219 \pm 0.0017}{0.2219}{0.0017}%
\htquantdef{Vus_tauKnu_err_th_perc}{Vus_tauKnu_err_th_perc}{}{0.1927}{0.1927}{0}%
\htquantdef{Vus_tauKnu_mism}{Vus_tauKnu_mism}{}{(-0.5730 \pm 0.2178) \cdot 10^{-2}}{-0.5730\cdot 10^{-2}}{0.2178\cdot 10^{-2}}%
\htquantdef{Vus_tauKnu_mism_sigma}{Vus_tauKnu_mism_sigma}{}{-2.6}{-2.6}{0}%
\htquantdef{Vus_tauKnu_mism_sigma_abs}{Vus_tauKnu_mism_sigma_abs}{}{2.6}{2.6}{0}%
\htquantdef{Vus_tauKpi}{Vus_tauKpi}{}{0.2229 \pm 0.0019}{0.2229}{0.0019}%
\htquantdef{Vus_tauKpi_err_th_perc}{Vus_tauKpi_err_th_perc}{}{0.1760}{0.1760}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_dRrad_kmunu_by_pimunu}{Vus_tauKpi_err_th_perc_dRrad_kmunu_by_pimunu}{}{0.000}{0.000}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_dRrad_tauK_by_Kmu}{Vus_tauKpi_err_th_perc_dRrad_tauK_by_Kmu}{}{0.000}{0.000}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_dRrad_taupi_by_pimu}{Vus_tauKpi_err_th_perc_dRrad_taupi_by_pimu}{}{0.000}{0.000}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_f_Kpm_by_f_pipm}{Vus_tauKpi_err_th_perc_f_Kpm_by_f_pipm}{}{0.1760}{0.1760}{0}%
\htquantdef{Vus_tauKpi_mism}{Vus_tauKpi_mism}{}{(-0.4803 \pm 0.2336) \cdot 10^{-2}}{-0.4803\cdot 10^{-2}}{0.2336\cdot 10^{-2}}%
\htquantdef{Vus_tauKpi_mism_sigma}{Vus_tauKpi_mism_sigma}{}{-2.1}{-2.1}{0}%
\htquantdef{Vus_tauKpi_mism_sigma_abs}{Vus_tauKpi_mism_sigma_abs}{}{2.1}{2.1}{0}%
\htquantdef{Vus_uni}{Vus_uni}{}{0.2277 \pm 0.0013}{0.2277}{0.0013}%
\htdef{couplingsCorr}{%
$\displaystyle\left( \frac{g_\tau}{g_e} \right)_\tau$ &   51\\
$\displaystyle\left( \frac{g_\mu}{g_e} \right)_\tau$ &  -50 &   49\\
$\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_\pi$ &   16 &   18 &    1\\
$\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_K$ &   12 &   11 &   -1 &    7\\
 & $\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_\tau$ & $\displaystyle\left( \frac{g_\tau}{g_e} \right)_\tau$ & $\displaystyle\left( \frac{g_\mu}{g_e} \right)_\tau$ & $\displaystyle\left( \frac{g_\tau}{g_\mu} \right)_\pi$}%


==> tau/hflav-2021.tex <==
\htdef{UnitarityResid}{(0.07 \pm 0.11)\%}%
\htdef{MeasNum}{171}%
\htdef{QuantNum}{135}%
\htdef{QuantNumNonRatio}{118}%
\htdef{QuantNumRatio}{17}%
\htdef{QuantNumWithMeas}{88}%
\htdef{QuantNumNonRatioWithMeas}{75}%
\htdef{QuantNumRatioWithMeas}{13}%
\htdef{QuantNumPdg}{129}%
\htdef{QuantNumNonRatioPdg}{112}%
\htdef{QuantNumRatioPdg}{17}%
\htdef{QuantNumWithMeasPdg}{86}%
\htdef{QuantNumNonRatioWithMeasPdg}{73}%
\htdef{QuantNumRatioWithMeasPdg}{13}%
\htdef{IndepQuantNum}{47}%
\htdef{BaseQuantNum}{47}%
\htdef{UnitarityQuantNum}{48}%
\htdef{ConstrNum}{88}%
\htdef{ConstrNumPdg}{82}%
\htdef{Chisq}{134}%
\htdef{Dof}{124}%
\htdef{ChisqProb}{24.56\%}%
\htdef{ChisqProbRound}{25\%}%
\htmeasdef{ALEPH.Gamma10.pub.BARATE.99K}{Gamma10}{ALEPH}{Barate:1999hi}{0.00696 \pm 0.00025 \pm 0.00014}{0.00696}{\pm 0.00025}{0.00014}%
\htmeasdef{ALEPH.Gamma103.pub.SCHAEL.05C}{Gamma103}{ALEPH}{Schael:2005am}{0.00072 \pm 0.00009 \pm 0.00012}{0.00072}{\pm 0.00009}{0.00012}%
\htmeasdef{ALEPH.Gamma104.pub.SCHAEL.05C}{Gamma104}{ALEPH}{Schael:2005am}{( 0.021 \pm 0.007 \pm 0.009 ) \cdot 10^{ -2 }}{0.021e-2}{\pm 0.007e-2}{0.009e-2}%
\htmeasdef{ALEPH.Gamma126.pub.BUSKULIC.97C}{Gamma126}{ALEPH}{Buskulic:1996qs}{0.0018 \pm 0.0004 \pm 0.0002}{0.0018}{\pm 0.0004}{0.0002}%
\htmeasdef{ALEPH.Gamma128.pub.BUSKULIC.97C}{Gamma128}{ALEPH}{Buskulic:1996qs}{( 2.9 {}^{+1.3\cdot 10^{-4}}_{-1.2} \pm 0.7 ) \cdot 10^{ -4 }}{2.9e-4}{{}^{+1.3e-4}_{-1.2e-4}}{0.7e-4}%
\htmeasdef{ALEPH.Gamma14.pub.SCHAEL.05C}{Gamma14}{ALEPH}{Schael:2005am}{0.25471 \pm 0.00097 \pm 0.00085}{0.25471}{\pm 0.00097}{0.00085}%
\htmeasdef{ALEPH.Gamma150.pub.BUSKULIC.97C}{Gamma150}{ALEPH}{Buskulic:1996qs}{0.0191 \pm 0.0007 \pm 0.0006}{0.0191}{\pm 0.0007}{0.0006}%
\htmeasdef{ALEPH.Gamma150by66.pub.BUSKULIC.96}{Gamma150by66}{ALEPH}{Buskulic:1995ty}{0.431 \pm 0.033}{0.431}{\pm 0.033}{0}%
\htmeasdef{ALEPH.Gamma152.pub.BUSKULIC.97C}{Gamma152}{ALEPH}{Buskulic:1996qs}{0.0043 \pm 0.0006 \pm 0.0005}{0.0043}{\pm 0.0006}{0.0005}%
\htmeasdef{ALEPH.Gamma16.pub.BARATE.99K}{Gamma16}{ALEPH}{Barate:1999hi}{0.00444 \pm 0.00026 \pm 0.00024}{0.00444}{\pm 0.00026}{0.00024}%
\htmeasdef{ALEPH.Gamma20.pub.SCHAEL.05C}{Gamma20}{ALEPH}{Schael:2005am}{0.09239 \pm 0.00086 \pm 0.0009}{0.09239}{\pm 0.00086}{0.0009}%
\htmeasdef{ALEPH.Gamma23.pub.BARATE.99K}{Gamma23}{ALEPH}{Barate:1999hi}{0.00056 \pm 0.0002 \pm 0.00015}{0.00056}{\pm 0.0002}{0.00015}%
\htmeasdef{ALEPH.Gamma27.pub.SCHAEL.05C}{Gamma27}{ALEPH}{Schael:2005am}{0.00977 \pm 0.00069 \pm 0.00058}{0.00977}{\pm 0.00069}{0.00058}%
\htmeasdef{ALEPH.Gamma28.pub.BARATE.99K}{Gamma28}{ALEPH}{Barate:1999hi}{0.00037 \pm 0.00021 \pm 0.00011}{0.00037}{\pm 0.00021}{0.00011}%
\htmeasdef{ALEPH.Gamma3.pub.SCHAEL.05C}{Gamma3}{ALEPH}{Schael:2005am}{0.17319 \pm 0.0007 \pm 0.00032}{0.17319}{\pm 0.0007}{0.00032}%
\htmeasdef{ALEPH.Gamma30.pub.SCHAEL.05C}{Gamma30}{ALEPH}{Schael:2005am}{0.00112 \pm 0.00037 \pm 0.00035}{0.00112}{\pm 0.00037}{0.00035}%
\htmeasdef{ALEPH.Gamma33.pub.BARATE.98E}{Gamma33}{ALEPH}{Barate:1997tt}{0.0097 \pm 0.00058 \pm 0.00062}{0.0097}{\pm 0.00058}{0.00062}%
\htmeasdef{ALEPH.Gamma35.pub.BARATE.99K}{Gamma35}{ALEPH}{Barate:1999hi}{0.00928 \pm 0.00045 \pm 0.00034}{0.00928}{\pm 0.00045}{0.00034}%
\htmeasdef{ALEPH.Gamma37.pub.BARATE.98E}{Gamma37}{ALEPH}{Barate:1997tt}{0.00158 \pm 0.00042 \pm 0.00017}{0.00158}{\pm 0.00042}{0.00017}%
\htmeasdef{ALEPH.Gamma37.pub.BARATE.99K}{Gamma37}{ALEPH}{Barate:1999hi}{0.00162 \pm 0.00021 \pm 0.00011}{0.00162}{\pm 0.00021}{0.00011}%
\htmeasdef{ALEPH.Gamma40.pub.BARATE.98E}{Gamma40}{ALEPH}{Barate:1997tt}{0.00294 \pm 0.00073 \pm 0.00037}{0.00294}{\pm 0.00073}{0.00037}%
\htmeasdef{ALEPH.Gamma40.pub.BARATE.99K}{Gamma40}{ALEPH}{Barate:1999hi}{0.00347 \pm 0.00053 \pm 0.00037}{0.00347}{\pm 0.00053}{0.00037}%
\htmeasdef{ALEPH.Gamma42.pub.BARATE.98E}{Gamma42}{ALEPH}{Barate:1997tt}{0.00152 \pm 0.00076 \pm 0.00021}{0.00152}{\pm 0.00076}{0.00021}%
\htmeasdef{ALEPH.Gamma42.pub.BARATE.99K}{Gamma42}{ALEPH}{Barate:1999hi}{0.00143 \pm 0.00025 \pm 0.00015}{0.00143}{\pm 0.00025}{0.00015}%
\htmeasdef{ALEPH.Gamma44.pub.BARATE.99R}{Gamma44}{ALEPH}{Barate:1999hj}{0.00026 \pm 0.00024}{0.00026}{\pm 0.00024}{0}%
\htmeasdef{ALEPH.Gamma47.pub.BARATE.98E}{Gamma47}{ALEPH}{Barate:1997tt}{0.00026 \pm 0.0001 \pm 5\cdot 10^{-5}}{0.00026}{\pm 0.0001}{5e-05}%
\htmeasdef{ALEPH.Gamma48.pub.BARATE.98E}{Gamma48}{ALEPH}{Barate:1997tt}{0.00101 \pm 0.00023 \pm 0.00013}{0.00101}{\pm 0.00023}{0.00013}%
\htmeasdef{ALEPH.Gamma5.pub.SCHAEL.05C}{Gamma5}{ALEPH}{Schael:2005am}{0.17837 \pm 0.00072 \pm 0.00036}{0.17837}{\pm 0.00072}{0.00036}%
\htmeasdef{ALEPH.Gamma51.pub.BARATE.98E}{Gamma51}{ALEPH}{Barate:1997tt}{( 3.1 \pm 1.1 \pm 0.5 ) \cdot 10^{ -4 }}{3.1e-4}{\pm 1.1e-4}{0.5e-4}%
\htmeasdef{ALEPH.Gamma53.pub.BARATE.98E}{Gamma53}{ALEPH}{Barate:1997tt}{0.00023 \pm 0.00019 \pm 0.00007}{0.00023}{\pm 0.00019}{0.00007}%
\htmeasdef{ALEPH.Gamma62.pub.SCHAEL.05C}{Gamma62}{ALEPH}{Schael:2005am}{0.09041 \pm 0.0006 \pm 0.00076}{0.09041}{\pm 0.0006}{0.00076}%
\htmeasdef{ALEPH.Gamma69.pub.SCHAEL.05C}{Gamma69}{ALEPH}{Schael:2005am}{0.04598 \pm 0.00057 \pm 0.00064}{0.04598}{\pm 0.00057}{0.00064}%
\htmeasdef{ALEPH.Gamma76.pub.SCHAEL.05C}{Gamma76}{ALEPH}{Schael:2005am}{0.00435 \pm 0.00030 \pm 0.00035}{0.00435}{\pm 0.00030}{0.00035}%
\htmeasdef{ALEPH.Gamma805.pub.SCHAEL.05C}{Gamma805}{ALEPH}{Schael:2005am}{( 4 \pm 2 ) \cdot 10^{ -4 }}{4e-04}{\pm 2e-04}{0}%
\htmeasdef{ALEPH.Gamma85.pub.BARATE.98}{Gamma85}{ALEPH}{Barate:1997ma}{0.00214 \pm 0.00037 \pm 0.00029}{0.00214}{\pm 0.00037}{0.00029}%
\htmeasdef{ALEPH.Gamma88.pub.BARATE.98}{Gamma88}{ALEPH}{Barate:1997ma}{0.00061 \pm 0.00039 \pm 0.00018}{0.00061}{\pm 0.00039}{0.00018}%
\htmeasdef{ALEPH.Gamma9.pub.SCHAEL.05C}{Gamma9}{ALEPH}{Schael:2005am}{0.10828 \pm 0.0007 \pm 0.00078}{0.10828}{\pm 0.0007}{0.00078}%
\htmeasdef{ALEPH.Gamma93.pub.BARATE.98}{Gamma93}{ALEPH}{Barate:1997ma}{0.00163 \pm 0.00021 \pm 0.00017}{0.00163}{\pm 0.00021}{0.00017}%
\htmeasdef{ALEPH.Gamma94.pub.BARATE.98}{Gamma94}{ALEPH}{Barate:1997ma}{0.00075 \pm 0.00029 \pm 0.00015}{0.00075}{\pm 0.00029}{0.00015}%
\htmeasdef{ARGUS.Gamma103.pub.ALBRECHT.88B}{Gamma103}{ARGUS}{Albrecht:1987zf}{0.00064 \pm 0.00023 \pm 0.0001}{0.00064}{\pm 0.00023}{0.0001}%
\htmeasdef{ARGUS.Gamma3by5.pub.ALBRECHT.92D}{Gamma3by5}{ARGUS}{Albrecht:1991rh}{0.997 \pm 0.035 \pm 0.04}{0.997}{\pm 0.035}{0.04}%
\htmeasdef{BaBar.Gamma10by5.pub.AUBERT.10F}{Gamma10by5}{\babar}{Aubert:2009qj}{0.03882 \pm 0.00032 \pm 0.00057}{0.03882}{\pm 0.00032}{0.00057}%
\htmeasdef{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E}{Gamma128}{\babar}{delAmoSanchez:2010pc}{0.000142 \pm 1.1\cdot 10^{-5} \pm 7\cdot 10^{-6}}{0.000142}{\pm 1.1e-05}{7e-06}%
\htmeasdef{BaBar.Gamma16.pub.AUBERT.07AP}{Gamma16}{\babar}{Aubert:2007jh}{0.00416 \pm 3\cdot 10^{-5} \pm 0.00018}{0.00416}{\pm 3e-05}{0.00018}%
\htmeasdef{BaBar.Gamma37.pub.LEES.18B}{Gamma37}{\babar}{BaBar:2018qry}{( 14.78 \pm 0.22 \pm 0.40 ) \cdot 10^{ -4 }}{14.78e-4}{\pm 0.22e-4}{0.40e-4}%
\htmeasdef{BaBar.Gamma3by5.pub.AUBERT.10F}{Gamma3by5}{\babar}{Aubert:2009qj}{0.9796 \pm 0.0016 \pm 0.0036}{0.9796}{\pm 0.0016}{0.0036}%
\htmeasdef{BaBar.Gamma47.pub.LEES.12Y}{Gamma47}{\babar}{Lees:2012de}{( 2.31 \pm 0.04 \pm 0.08 ) \cdot 10^{ -4 }}{2.31e-4}{\pm 0.04e-4}{0.08e-4}%
\htmeasdef{BaBar.Gamma50.pub.LEES.12Y}{Gamma50}{\babar}{Lees:2012de}{( 1.60 \pm 0.20 \pm 0.22 ) \cdot 10^{ -5 }}{1.60e-5}{\pm 0.20e-5}{0.22e-5}%
\htmeasdef{BaBar.Gamma60.pub.AUBERT.08}{Gamma60}{\babar}{Aubert:2007mh}{0.0883 \pm 0.0001 \pm 0.0013}{0.0883}{\pm 0.0001}{0.0013}%
\htmeasdef{BaBar.Gamma811.pub.LEES.12X}{Gamma811}{\babar}{Lees:2012ks}{( 7.3 \pm 1.2 \pm 1.2 ) \cdot 10^{ -5 }}{7.3e-5}{\pm 1.2e-5}{1.2e-5}%
\htmeasdef{BaBar.Gamma812.pub.LEES.12X}{Gamma812}{\babar}{Lees:2012ks}{( 0.1 \pm 0.08 \pm 0.30 ) \cdot 10^{ -4 }}{0.1e-4}{\pm 0.08e-4}{0.30e-4}%
\htmeasdef{BaBar.Gamma821.pub.LEES.12X}{Gamma821}{\babar}{Lees:2012ks}{( 7.68 \pm 0.04 \pm 0.40 ) \cdot 10^{ -4 }}{7.68e-4}{\pm 0.04e-4}{0.40e-4}%
\htmeasdef{BaBar.Gamma822.pub.LEES.12X}{Gamma822}{\babar}{Lees:2012ks}{( 0.6 \pm 0.5 \pm 1.1 ) \cdot 10^{ -6 }}{0.6e-06}{\pm 0.5e-06}{1.1e-06}%
\htmeasdef{BaBar.Gamma831.pub.LEES.12X}{Gamma831}{\babar}{Lees:2012ks}{( 8.4 \pm 0.4 \pm 0.6 ) \cdot 10^{ -5 }}{8.4e-5}{\pm 0.4e-5}{0.6e-5}%
\htmeasdef{BaBar.Gamma832.pub.LEES.12X}{Gamma832}{\babar}{Lees:2012ks}{( 0.36 \pm 0.03 \pm 0.09 ) \cdot 10^{ -4 }}{0.36e-4}{\pm 0.03e-4}{0.09e-4}%
\htmeasdef{BaBar.Gamma833.pub.LEES.12X}{Gamma833}{\babar}{Lees:2012ks}{( 1.1 \pm 0.4 \pm 0.4 ) \cdot 10^{ -6 }}{1.1e-6}{\pm 0.4e-6}{0.4e-6}%
\htmeasdef{BaBar.Gamma85.pub.AUBERT.08}{Gamma85}{\babar}{Aubert:2007mh}{0.00273 \pm 2\cdot 10^{-5} \pm 9\cdot 10^{-5}}{0.00273}{\pm 2e-05}{9e-05}%
\htmeasdef{BaBar.Gamma910.pub.LEES.12X}{Gamma910}{\babar}{Lees:2012ks}{( 8.27 \pm 0.88 \pm 0.81 ) \cdot 10^{ -5 }}{8.27e-5}{\pm 0.88e-5}{0.81e-5}%
\htmeasdef{BaBar.Gamma911.pub.LEES.12X}{Gamma911}{\babar}{Lees:2012ks}{( 4.57 \pm 0.77 \pm 0.50 ) \cdot 10^{ -5 }}{4.57e-5}{\pm 0.77e-5}{0.50e-5}%
\htmeasdef{BaBar.Gamma920.pub.LEES.12X}{Gamma920}{\babar}{Lees:2012ks}{( 5.20 \pm 0.31 \pm 0.37 ) \cdot 10^{ -5 }}{5.20e-5}{\pm 0.31e-5}{0.37e-5}%
\htmeasdef{BaBar.Gamma93.pub.AUBERT.08}{Gamma93}{\babar}{Aubert:2007mh}{0.001346 \pm 1\cdot 10^{-5} \pm 3.6\cdot 10^{-5}}{0.001346}{\pm 1e-05}{3.6e-05}%
\htmeasdef{BaBar.Gamma930.pub.LEES.12X}{Gamma930}{\babar}{Lees:2012ks}{( 5.39 \pm 0.27 \pm 0.41 ) \cdot 10^{ -5 }}{5.39e-5}{\pm 0.27e-5}{0.41e-5}%
\htmeasdef{BaBar.Gamma944.pub.LEES.12X}{Gamma944}{\babar}{Lees:2012ks}{( 8.26 \pm 0.35 \pm 0.51 ) \cdot 10^{ -5 }}{8.26e-5}{\pm 0.35e-5}{0.51e-5}%
\htmeasdef{BaBar.Gamma96.pub.AUBERT.08}{Gamma96}{\babar}{Aubert:2007mh}{1.5777\cdot 10^{-5} \pm 1.3\cdot 10^{-6} \pm 1.2308\cdot 10^{-6}}{1.5777e-05}{\pm 1.3e-06}{1.2308e-06}%
\htmeasdef{BaBar.Gamma9by5.pub.AUBERT.10F}{Gamma9by5}{\babar}{Aubert:2009qj}{0.5945 \pm 0.0014 \pm 0.0061}{0.5945}{\pm 0.0014}{0.0061}%
\htmeasdef{Belle.Gamma126.pub.INAMI.09}{Gamma126}{Belle}{Inami:2008ar}{0.00135 \pm 3\cdot 10^{-5} \pm 7\cdot 10^{-5}}{0.00135}{\pm 3e-05}{7e-05}%
\htmeasdef{Belle.Gamma128.pub.INAMI.09}{Gamma128}{Belle}{Inami:2008ar}{0.000158 \pm 5\cdot 10^{-6} \pm 9\cdot 10^{-6}}{0.000158}{\pm 5e-06}{9e-06}%
\htmeasdef{Belle.Gamma13.pub.FUJIKAWA.08}{Gamma13}{Belle}{Fujikawa:2008ma}{0.2567 \pm 1\cdot 10^{-4} \pm 0.0039}{0.2567}{\pm 1e-04}{0.0039}%
\htmeasdef{Belle.Gamma130.pub.INAMI.09}{Gamma130}{Belle}{Inami:2008ar}{4.6\cdot 10^{-5} \pm 1.1\cdot 10^{-5} \pm 4\cdot 10^{-6}}{4.6e-05}{\pm 1.1e-05}{4e-06}%
\htmeasdef{Belle.Gamma132.pub.INAMI.09}{Gamma132}{Belle}{Inami:2008ar}{8.8\cdot 10^{-5} \pm 1.4\cdot 10^{-5} \pm 6\cdot 10^{-6}}{8.8e-05}{\pm 1.4e-05}{6e-06}%
\htmeasdef{Belle.Gamma35.pub.RYU.14vpc}{Gamma35}{Belle}{Ryu:2014vpc}{8.32\cdot 10^{-3} \pm 0.3\% \pm 1.8\%}{8.32e-03}{\pm 0.3\%}{1.8\%}%
\htmeasdef{Belle.Gamma37.pub.RYU.14vpc}{Gamma37}{Belle}{Ryu:2014vpc}{14.8\cdot 10^{-4} \pm 0.9\% \pm 3.7\%}{14.8e-04}{\pm 0.9\%}{3.7\%}%
\htmeasdef{Belle.Gamma40.pub.RYU.14vpc}{Gamma40}{Belle}{Ryu:2014vpc}{3.86\cdot 10^{-3} \pm 0.8\% \pm 3.5\%}{3.86e-03}{\pm 0.8\%}{3.5\%}%
\htmeasdef{Belle.Gamma42.pub.RYU.14vpc}{Gamma42}{Belle}{Ryu:2014vpc}{14.96\cdot 10^{-4} \pm 1.3\% \pm 4.9\%}{14.96e-04}{\pm 1.3\%}{4.9\%}%
\htmeasdef{Belle.Gamma47.pub.RYU.14vpc}{Gamma47}{Belle}{Ryu:2014vpc}{2.33\cdot 10^{-4} \pm 1.4\% \pm 4.0\%}{2.33e-04}{\pm 1.4\%}{4.0\%}%
\htmeasdef{Belle.Gamma50.pub.RYU.14vpc}{Gamma50}{Belle}{Ryu:2014vpc}{2.00\cdot 10^{-5} \pm 10.8\% \pm 10.1\%}{2.00e-05}{\pm 10.8\%}{10.1\%}%
\htmeasdef{Belle.Gamma60.pub.LEE.10}{Gamma60}{Belle}{Lee:2010tc}{0.0842 \pm 0 {}^{+0.0026}_{-0.0025}}{0.0842}{\pm 0}{{}^{+0.0026}_{-0.0025}}%
\htmeasdef{Belle.Gamma85.pub.LEE.10}{Gamma85}{Belle}{Lee:2010tc}{0.0033 \pm 1\cdot 10^{-5} {}^{+0.00016}_{-0.00017}}{0.0033}{\pm 1e-05}{{}^{+0.00016}_{-0.00017}}%
\htmeasdef{Belle.Gamma93.pub.LEE.10}{Gamma93}{Belle}{Lee:2010tc}{0.00155 \pm 1\cdot 10^{-5} {}^{+6\cdot 10^{-5}}_{-5\cdot 10^{-5}}}{0.00155}{\pm 1e-05}{{}^{+6e-05}_{-5e-05}}%
\htmeasdef{Belle.Gamma96.pub.LEE.10}{Gamma96}{Belle}{Lee:2010tc}{3.29\cdot 10^{-5} \pm 1.7\cdot 10^{-6} {}^{+1.9\cdot 10^{-6}}_{-2.0\cdot 10^{-6}}}{3.29e-05}{\pm 1.7e-06}{{}^{+1.9e-06}_{-2.0e-06}}%
\htmeasdef{CELLO.Gamma54.pub.BEHREND.89B}{Gamma54}{CELLO}{Behrend:1989wc}{0.15 \pm 0.004 \pm 0.003}{0.15}{\pm 0.004}{0.003}%
\htmeasdef{CLEO.Gamma10.pub.BATTLE.94}{Gamma10}{CLEO}{Battle:1994by}{0.0066 \pm 0.0007 \pm 0.0009}{0.0066}{\pm 0.0007}{0.0009}%
\htmeasdef{CLEO.Gamma102.pub.GIBAUT.94B}{Gamma102}{CLEO}{Gibaut:1994ik}{0.00097 \pm 5\cdot 10^{-5} \pm 0.00011}{0.00097}{\pm 5e-05}{0.00011}%
\htmeasdef{CLEO.Gamma103.pub.GIBAUT.94B}{Gamma103}{CLEO}{Gibaut:1994ik}{0.00077 \pm 5\cdot 10^{-5} \pm 9\cdot 10^{-5}}{0.00077}{\pm 5e-05}{9e-05}%
\htmeasdef{CLEO.Gamma104.pub.ANASTASSOV.01}{Gamma104}{CLEO}{Anastassov:2000xu}{0.00017 \pm 2\cdot 10^{-5} \pm 2\cdot 10^{-5}}{0.00017}{\pm 2e-05}{2e-05}%
\htmeasdef{CLEO.Gamma126.pub.ARTUSO.92}{Gamma126}{CLEO}{Artuso:1992qu}{0.0017 \pm 0.0002 \pm 0.0002}{0.0017}{\pm 0.0002}{0.0002}%
\htmeasdef{CLEO.Gamma128.pub.BARTELT.96}{Gamma128}{CLEO}{Bartelt:1996iv}{( 2.6 \pm 0.5 \pm 0.5 ) \cdot 10^{ -4 }}{2.6e-4}{\pm 0.5e-4}{0.5e-4}%
\htmeasdef{CLEO.Gamma13.pub.ARTUSO.94}{Gamma13}{CLEO}{Artuso:1994ii}{0.2587 \pm 0.0012 \pm 0.0042}{0.2587}{\pm 0.0012}{0.0042}%
\htmeasdef{CLEO.Gamma130.pub.BISHAI.99}{Gamma130}{CLEO}{Bishai:1998gf}{( 1.77 \pm 0.56 \pm 0.71 ) \cdot 10^{ -4 }}{1.77e-4}{\pm 0.56e-4}{0.71e-4}%
\htmeasdef{CLEO.Gamma132.pub.BISHAI.99}{Gamma132}{CLEO}{Bishai:1998gf}{( 2.2 \pm 0.70 \pm 0.22 ) \cdot 10^{ -4 }}{2.2e-4}{\pm 0.70e-4}{0.22e-4}%
\htmeasdef{CLEO.Gamma150.pub.BARINGER.87}{Gamma150}{CLEO}{Baringer:1987tr}{0.016 \pm 0.0027 \pm 0.0041}{0.016}{\pm 0.0027}{0.0041}%
\htmeasdef{CLEO.Gamma150by66.pub.BALEST.95C}{Gamma150by66}{CLEO}{Balest:1995kq}{0.464 \pm 0.016 \pm 0.017}{0.464}{\pm 0.016}{0.017}%
\htmeasdef{CLEO.Gamma152by76.pub.BORTOLETTO.93}{Gamma152by76}{CLEO}{Bortoletto:1993px}{0.81 \pm 0.06 \pm 0.06}{0.81}{\pm 0.06}{0.06}%
\htmeasdef{CLEO.Gamma16.pub.BATTLE.94}{Gamma16}{CLEO}{Battle:1994by}{0.0051 \pm 0.001 \pm 0.0007}{0.0051}{\pm 0.001}{0.0007}%
\htmeasdef{CLEO.Gamma19by13.pub.PROCARIO.93}{Gamma19by13}{CLEO}{Procario:1992hd}{0.342 \pm 0.006 \pm 0.016}{0.342}{\pm 0.006}{0.016}%
\htmeasdef{CLEO.Gamma23.pub.BATTLE.94}{Gamma23}{CLEO}{Battle:1994by}{0.0009 \pm 0.001 \pm 0.0003}{0.0009}{\pm 0.001}{0.0003}%
\htmeasdef{CLEO.Gamma26by13.pub.PROCARIO.93}{Gamma26by13}{CLEO}{Procario:1992hd}{0.044 \pm 0.003 \pm 0.005}{0.044}{\pm 0.003}{0.005}%
\htmeasdef{CLEO.Gamma29.pub.PROCARIO.93}{Gamma29}{CLEO}{Procario:1992hd}{0.0016 \pm 0.0005 \pm 0.0005}{0.0016}{\pm 0.0005}{0.0005}%
\htmeasdef{CLEO.Gamma31.pub.BATTLE.94}{Gamma31}{CLEO}{Battle:1994by}{0.017 \pm 0.0012 \pm 0.0019}{0.017}{\pm 0.0012}{0.0019}%
\htmeasdef{CLEO.Gamma34.pub.COAN.96}{Gamma34}{CLEO}{Coan:1996iu}{0.00855 \pm 0.00036 \pm 0.00073}{0.00855}{\pm 0.00036}{0.00073}%
\htmeasdef{CLEO.Gamma37.pub.COAN.96}{Gamma37}{CLEO}{Coan:1996iu}{0.00151 \pm 0.00021 \pm 0.00022}{0.00151}{\pm 0.00021}{0.00022}%
\htmeasdef{CLEO.Gamma39.pub.COAN.96}{Gamma39}{CLEO}{Coan:1996iu}{0.00562 \pm 0.0005 \pm 0.00048}{0.00562}{\pm 0.0005}{0.00048}%
\htmeasdef{CLEO.Gamma3by5.pub.ANASTASSOV.97}{Gamma3by5}{CLEO}{Anastassov:1996tc}{0.9777 \pm 0.0063 \pm 0.0087}{0.9777}{\pm 0.0063}{0.0087}%
\htmeasdef{CLEO.Gamma42.pub.COAN.96}{Gamma42}{CLEO}{Coan:1996iu}{0.00145 \pm 0.00036 \pm 0.0002}{0.00145}{\pm 0.00036}{0.0002}%
\htmeasdef{CLEO.Gamma47.pub.COAN.96}{Gamma47}{CLEO}{Coan:1996iu}{0.00023 \pm 5\cdot 10^{-5} \pm 3\cdot 10^{-5}}{0.00023}{\pm 5e-05}{3e-05}%
\htmeasdef{CLEO.Gamma5.pub.ANASTASSOV.97}{Gamma5}{CLEO}{Anastassov:1996tc}{0.1776 \pm 0.0006 \pm 0.0017}{0.1776}{\pm 0.0006}{0.0017}%
\htmeasdef{CLEO.Gamma57.pub.BALEST.95C}{Gamma57}{CLEO}{Balest:1995kq}{0.0951 \pm 0.0007 \pm 0.002}{0.0951}{\pm 0.0007}{0.002}%
\htmeasdef{CLEO.Gamma66.pub.BALEST.95C}{Gamma66}{CLEO}{Balest:1995kq}{0.0423 \pm 0.0006 \pm 0.0022}{0.0423}{\pm 0.0006}{0.0022}%
\htmeasdef{CLEO.Gamma69.pub.EDWARDS.00A}{Gamma69}{CLEO}{Edwards:1999fj}{0.0419 \pm 0.001 \pm 0.0021}{0.0419}{\pm 0.001}{0.0021}%
\htmeasdef{CLEO.Gamma76by54.pub.BORTOLETTO.93}{Gamma76by54}{CLEO}{Bortoletto:1993px}{0.034 \pm 0.002 \pm 0.003}{0.034}{\pm 0.002}{0.003}%
\htmeasdef{CLEO.Gamma78.pub.ANASTASSOV.01}{Gamma78}{CLEO}{Anastassov:2000xu}{0.00022 \pm 3\cdot 10^{-5} \pm 4\cdot 10^{-5}}{0.00022}{\pm 3e-05}{4e-05}%
\htmeasdef{CLEO.Gamma8.pub.ANASTASSOV.97}{Gamma8}{CLEO}{Anastassov:1996tc}{0.1152 \pm 0.0005 \pm 0.0012}{0.1152}{\pm 0.0005}{0.0012}%
\htmeasdef{CLEO.Gamma80by60.pub.RICHICHI.99}{Gamma80by60}{CLEO}{Richichi:1998bc}{0.0544 \pm 0.0021 \pm 0.0053}{0.0544}{\pm 0.0021}{0.0053}%
\htmeasdef{CLEO.Gamma81by69.pub.RICHICHI.99}{Gamma81by69}{CLEO}{Richichi:1998bc}{0.0261 \pm 0.0045 \pm 0.0042}{0.0261}{\pm 0.0045}{0.0042}%
\htmeasdef{CLEO.Gamma93by60.pub.RICHICHI.99}{Gamma93by60}{CLEO}{Richichi:1998bc}{0.016 \pm 0.0015 \pm 0.003}{0.016}{\pm 0.0015}{0.003}%
\htmeasdef{CLEO.Gamma94by69.pub.RICHICHI.99}{Gamma94by69}{CLEO}{Richichi:1998bc}{0.0079 \pm 0.0044 \pm 0.0016}{0.0079}{\pm 0.0044}{0.0016}%
\htmeasdef{CLEO3.Gamma151.pub.ARMS.05}{Gamma151}{CLEO3}{Arms:2005qg}{( 4.1 \pm 0.6 \pm 0.7 ) \cdot 10^{ -4 }}{4.1e-4}{\pm 0.6e-4}{0.7e-4}%
\htmeasdef{CLEO3.Gamma60.pub.BRIERE.03}{Gamma60}{CLEO3}{Briere:2003fr}{0.0913 \pm 0.0005 \pm 0.0046}{0.0913}{\pm 0.0005}{0.0046}%
\htmeasdef{CLEO3.Gamma85.pub.BRIERE.03}{Gamma85}{CLEO3}{Briere:2003fr}{0.00384 \pm 0.00014 \pm 0.00038}{0.00384}{\pm 0.00014}{0.00038}%
\htmeasdef{CLEO3.Gamma88.pub.ARMS.05}{Gamma88}{CLEO3}{Arms:2005qg}{0.00074 \pm 8\cdot 10^{-5} \pm 0.00011}{0.00074}{\pm 8e-05}{0.00011}%
\htmeasdef{CLEO3.Gamma93.pub.BRIERE.03}{Gamma93}{CLEO3}{Briere:2003fr}{0.00155 \pm 6\cdot 10^{-5} \pm 9\cdot 10^{-5}}{0.00155}{\pm 6e-05}{9e-05}%
\htmeasdef{CLEO3.Gamma94.pub.ARMS.05}{Gamma94}{CLEO3}{Arms:2005qg}{( 5.5 \pm 1.4 \pm 1.2 ) \cdot 10^{ -5 }}{5.5e-05}{\pm 1.4e-05}{1.2e-05}%
\htmeasdef{DELPHI.Gamma10.pub.ABREU.94K}{Gamma10}{DELPHI}{Abreu:1994fi}{0.0085 \pm 0.0018}{0.0085}{\pm 0.0018}{0}%
\htmeasdef{DELPHI.Gamma103.pub.ABDALLAH.06A}{Gamma103}{DELPHI}{Abdallah:2003cw}{0.00097 \pm 0.00015 \pm 5\cdot 10^{-5}}{0.00097}{\pm 0.00015}{5e-05}%
\htmeasdef{DELPHI.Gamma104.pub.ABDALLAH.06A}{Gamma104}{DELPHI}{Abdallah:2003cw}{0.00016 \pm 0.00012 \pm 6\cdot 10^{-5}}{0.00016}{\pm 0.00012}{6e-05}%
\htmeasdef{DELPHI.Gamma13.pub.ABDALLAH.06A}{Gamma13}{DELPHI}{Abdallah:2003cw}{0.2574 \pm 0.00201 \pm 0.00138}{0.2574}{\pm 0.00201}{0.00138}%
\htmeasdef{DELPHI.Gamma19.pub.ABDALLAH.06A}{Gamma19}{DELPHI}{Abdallah:2003cw}{0.09498 \pm 0.0032 \pm 0.00275}{0.09498}{\pm 0.0032}{0.00275}%
\htmeasdef{DELPHI.Gamma25.pub.ABDALLAH.06A}{Gamma25}{DELPHI}{Abdallah:2003cw}{0.01403 \pm 0.00214 \pm 0.00224}{0.01403}{\pm 0.00214}{0.00224}%
\htmeasdef{DELPHI.Gamma3.pub.ABREU.99X}{Gamma3}{DELPHI}{Abreu:1999rb}{0.17325 \pm 0.00095 \pm 0.00077}{0.17325}{\pm 0.00095}{0.00077}%
\htmeasdef{DELPHI.Gamma31.pub.ABREU.94K}{Gamma31}{DELPHI}{Abreu:1994fi}{0.0154 \pm 0.0024}{0.0154}{\pm 0.0024}{0}%
\htmeasdef{DELPHI.Gamma5.pub.ABREU.99X}{Gamma5}{DELPHI}{Abreu:1999rb}{0.17877 \pm 0.00109 \pm 0.0011}{0.17877}{\pm 0.00109}{0.0011}%
\htmeasdef{DELPHI.Gamma57.pub.ABDALLAH.06A}{Gamma57}{DELPHI}{Abdallah:2003cw}{0.09317 \pm 0.0009 \pm 0.00082}{0.09317}{\pm 0.0009}{0.00082}%
\htmeasdef{DELPHI.Gamma66.pub.ABDALLAH.06A}{Gamma66}{DELPHI}{Abdallah:2003cw}{0.04545 \pm 0.00106 \pm 0.00103}{0.04545}{\pm 0.00106}{0.00103}%
\htmeasdef{DELPHI.Gamma7.pub.ABREU.92N}{Gamma7}{DELPHI}{Abreu:1992gn}{0.124 \pm 0.007 \pm 0.007}{0.124}{\pm 0.007}{0.007}%
\htmeasdef{DELPHI.Gamma74.pub.ABDALLAH.06A}{Gamma74}{DELPHI}{Abdallah:2003cw}{0.00561 \pm 0.00068 \pm 0.00095}{0.00561}{\pm 0.00068}{0.00095}%
\htmeasdef{DELPHI.Gamma8.pub.ABDALLAH.06A}{Gamma8}{DELPHI}{Abdallah:2003cw}{0.11571 \pm 0.0012 \pm 0.00114}{0.11571}{\pm 0.0012}{0.00114}%
\htmeasdef{HRS.Gamma102.pub.BYLSMA.87}{Gamma102}{HRS}{Bylsma:1986zy}{0.00102 \pm 0.00029}{0.00102}{\pm 0.00029}{0}%
\htmeasdef{HRS.Gamma103.pub.BYLSMA.87}{Gamma103}{HRS}{Bylsma:1986zy}{0.00051 \pm 0.0002}{0.00051}{\pm 0.0002}{0}%
\htmeasdef{L3.Gamma102.pub.ACHARD.01D}{Gamma102}{L3}{Achard:2001pk}{0.0017 \pm 0.00022 \pm 0.00026}{0.0017}{\pm 0.00022}{0.00026}%
\htmeasdef{L3.Gamma13.pub.ACCIARRI.95}{Gamma13}{L3}{Acciarri:1994vr}{0.2505 \pm 0.0035 \pm 0.005}{0.2505}{\pm 0.0035}{0.005}%
\htmeasdef{L3.Gamma19.pub.ACCIARRI.95}{Gamma19}{L3}{Acciarri:1994vr}{0.0888 \pm 0.0037 \pm 0.0042}{0.0888}{\pm 0.0037}{0.0042}%
\htmeasdef{L3.Gamma26.pub.ACCIARRI.95}{Gamma26}{L3}{Acciarri:1994vr}{0.017 \pm 0.0024 \pm 0.0038}{0.017}{\pm 0.0024}{0.0038}%
\htmeasdef{L3.Gamma3.pub.ACCIARRI.01F}{Gamma3}{L3}{Acciarri:2001sg}{0.17342 \pm 0.0011 \pm 0.00067}{0.17342}{\pm 0.0011}{0.00067}%
\htmeasdef{L3.Gamma35.pub.ACCIARRI.95F}{Gamma35}{L3}{Acciarri:1995kx}{0.0095 \pm 0.0015 \pm 0.0006}{0.0095}{\pm 0.0015}{0.0006}%
\htmeasdef{L3.Gamma40.pub.ACCIARRI.95F}{Gamma40}{L3}{Acciarri:1995kx}{0.0041 \pm 0.0012 \pm 0.0003}{0.0041}{\pm 0.0012}{0.0003}%
\htmeasdef{L3.Gamma5.pub.ACCIARRI.01F}{Gamma5}{L3}{Acciarri:2001sg}{0.17806 \pm 0.00104 \pm 0.00076}{0.17806}{\pm 0.00104}{0.00076}%
\htmeasdef{L3.Gamma54.pub.ADEVA.91F}{Gamma54}{L3}{Adeva:1991qq}{0.144 \pm 0.006 \pm 0.003}{0.144}{\pm 0.006}{0.003}%
\htmeasdef{L3.Gamma55.pub.ACHARD.01D}{Gamma55}{L3}{Achard:2001pk}{0.14556 \pm 0.00105 \pm 0.00076}{0.14556}{\pm 0.00105}{0.00076}%
\htmeasdef{L3.Gamma7.pub.ACCIARRI.95}{Gamma7}{L3}{Acciarri:1994vr}{0.1247 \pm 0.0026 \pm 0.0043}{0.1247}{\pm 0.0026}{0.0043}%
\htmeasdef{OPAL.Gamma10.pub.ABBIENDI.01J}{Gamma10}{OPAL}{Abbiendi:2000ee}{0.00658 \pm 0.00027 \pm 0.00029}{0.00658}{\pm 0.00027}{0.00029}%
\htmeasdef{OPAL.Gamma103.pub.ACKERSTAFF.99E}{Gamma103}{OPAL}{Ackerstaff:1998ia}{0.00091 \pm 0.00014 \pm 6\cdot 10^{-5}}{0.00091}{\pm 0.00014}{6e-05}%
\htmeasdef{OPAL.Gamma104.pub.ACKERSTAFF.99E}{Gamma104}{OPAL}{Ackerstaff:1998ia}{0.00027 \pm 0.00018 \pm 9\cdot 10^{-5}}{0.00027}{\pm 0.00018}{9e-05}%
\htmeasdef{OPAL.Gamma13.pub.ACKERSTAFF.98M}{Gamma13}{OPAL}{Ackerstaff:1997tx}{0.2589 \pm 0.0017 \pm 0.0029}{0.2589}{\pm 0.0017}{0.0029}%
\htmeasdef{OPAL.Gamma16.pub.ABBIENDI.04J}{Gamma16}{OPAL}{Abbiendi:2004xa}{0.00471 \pm 0.00059 \pm 0.00023}{0.00471}{\pm 0.00059}{0.00023}%
\htmeasdef{OPAL.Gamma17.pub.ACKERSTAFF.98M}{Gamma17}{OPAL}{Ackerstaff:1997tx}{0.0991 \pm 0.0031 \pm 0.0027}{0.0991}{\pm 0.0031}{0.0027}%
\htmeasdef{OPAL.Gamma3.pub.ABBIENDI.03}{Gamma3}{OPAL}{Abbiendi:2002jw}{0.1734 \pm 0.0009 \pm 0.0006}{0.1734}{\pm 0.0009}{0.0006}%
\htmeasdef{OPAL.Gamma31.pub.ABBIENDI.01J}{Gamma31}{OPAL}{Abbiendi:2000ee}{0.01528 \pm 0.00039 \pm 0.0004}{0.01528}{\pm 0.00039}{0.0004}%
\htmeasdef{OPAL.Gamma33.pub.AKERS.94G}{Gamma33}{OPAL}{Akers:1994td}{0.0097 \pm 0.0009 \pm 0.0006}{0.0097}{\pm 0.0009}{0.0006}%
\htmeasdef{OPAL.Gamma35.pub.ABBIENDI.00C}{Gamma35}{OPAL}{Abbiendi:1999pm}{0.00933 \pm 0.00068 \pm 0.00049}{0.00933}{\pm 0.00068}{0.00049}%
\htmeasdef{OPAL.Gamma38.pub.ABBIENDI.00C}{Gamma38}{OPAL}{Abbiendi:1999pm}{0.0033 \pm 0.00055 \pm 0.00039}{0.0033}{\pm 0.00055}{0.00039}%
\htmeasdef{OPAL.Gamma43.pub.ABBIENDI.00C}{Gamma43}{OPAL}{Abbiendi:1999pm}{0.00324 \pm 0.00074 \pm 0.00066}{0.00324}{\pm 0.00074}{0.00066}%
\htmeasdef{OPAL.Gamma5.pub.ABBIENDI.99H}{Gamma5}{OPAL}{Abbiendi:1998cx}{0.1781 \pm 0.0009 \pm 0.0006}{0.1781}{\pm 0.0009}{0.0006}%
\htmeasdef{OPAL.Gamma55.pub.AKERS.95Y}{Gamma55}{OPAL}{Akers:1995ry}{0.1496 \pm 0.0009 \pm 0.0022}{0.1496}{\pm 0.0009}{0.0022}%
\htmeasdef{OPAL.Gamma57by55.pub.AKERS.95Y}{Gamma57by55}{OPAL}{Akers:1995ry}{0.66 \pm 0.004 \pm 0.014}{0.66}{\pm 0.004}{0.014}%
\htmeasdef{OPAL.Gamma7.pub.ALEXANDER.91D}{Gamma7}{OPAL}{Alexander:1991am}{0.121 \pm 0.007 \pm 0.005}{0.121}{\pm 0.007}{0.005}%
\htmeasdef{OPAL.Gamma8.pub.ACKERSTAFF.98M}{Gamma8}{OPAL}{Ackerstaff:1997tx}{0.1198 \pm 0.0013 \pm 0.0016}{0.1198}{\pm 0.0013}{0.0016}%
\htmeasdef{OPAL.Gamma85.pub.ABBIENDI.04J}{Gamma85}{OPAL}{Abbiendi:2004xa}{0.00415 \pm 0.00053 \pm 0.0004}{0.00415}{\pm 0.00053}{0.0004}%
\htmeasdef{OPAL.Gamma92.pub.ABBIENDI.00D}{Gamma92}{OPAL}{Abbiendi:1999cq}{0.00159 \pm 0.00053 \pm 0.0002}{0.00159}{\pm 0.00053}{0.0002}%
\htmeasdef{TPC.Gamma54.pub.AIHARA.87B}{Gamma54}{TPC}{Aihara:1986mw}{0.151 \pm 0.008 \pm 0.006}{0.151}{\pm 0.008}{0.006}%
\htmeasdef{TPC.Gamma82.pub.BAUER.94}{Gamma82}{TPC}{Bauer:1993wn}{0.0058 {}^{+0.0015}_{-0.0013} \pm 0.0012}{0.0058}{{}^{+0.0015}_{-0.0013}}{0.0012}%
\htmeasdef{TPC.Gamma92.pub.BAUER.94}{Gamma92}{TPC}{Bauer:1993wn}{0.0015 {}^{+0.0009}_{-0.0007} \pm 0.0003}{0.0015}{{}^{+0.0009}_{-0.0007}}{0.0003}%
\htdef{Gamma1.qt}{\ensuremath{0.8518 \pm 0.0011}}%
\htdef{Gamma2.qt}{\ensuremath{0.8452 \pm 0.0010}}%
\htdef{Gamma3.qt}{\ensuremath{0.17387 \pm 0.00040}}%
\htdef{ALEPH.Gamma3.pub.SCHAEL.05C,qt}{\ensuremath{0.17319 \pm 0.00070 \pm 0.00032}}%
\htdef{DELPHI.Gamma3.pub.ABREU.99X,qt}{\ensuremath{0.17325 \pm 0.00095 \pm 0.00077}}%
\htdef{L3.Gamma3.pub.ACCIARRI.01F,qt}{\ensuremath{0.17342 \pm 0.00110 \pm 0.00067}}%
\htdef{OPAL.Gamma3.pub.ABBIENDI.03,qt}{\ensuremath{0.17340 \pm 0.00090 \pm 0.00060}}%
\htdef{Gamma3by5.qt}{\ensuremath{0.9762 \pm 0.0028}}%
\htdef{ARGUS.Gamma3by5.pub.ALBRECHT.92D,qt}{\ensuremath{0.9970 \pm 0.0350 \pm 0.0400}}%
\htdef{BaBar.Gamma3by5.pub.AUBERT.10F,qt}{\ensuremath{0.9796 \pm 0.0016 \pm 0.0036}}%
\htdef{CLEO.Gamma3by5.pub.ANASTASSOV.97,qt}{\ensuremath{0.9777 \pm 0.0063 \pm 0.0087}}%
\htdef{Gamma5.qt}{\ensuremath{0.17811 \pm 0.00041}}%
\htdef{ALEPH.Gamma5.pub.SCHAEL.05C,qt}{\ensuremath{0.17837 \pm 0.00072 \pm 0.00036}}%
\htdef{CLEO.Gamma5.pub.ANASTASSOV.97,qt}{\ensuremath{0.17760 \pm 0.00060 \pm 0.00170}}%
\htdef{DELPHI.Gamma5.pub.ABREU.99X,qt}{\ensuremath{0.17877 \pm 0.00109 \pm 0.00110}}%
\htdef{L3.Gamma5.pub.ACCIARRI.01F,qt}{\ensuremath{0.17806 \pm 0.00104 \pm 0.00076}}%
\htdef{OPAL.Gamma5.pub.ABBIENDI.99H,qt}{\ensuremath{0.17810 \pm 0.00090 \pm 0.00060}}%
\htdef{Gamma7.qt}{\ensuremath{0.12020 \pm 0.00055}}%
\htdef{DELPHI.Gamma7.pub.ABREU.92N,qt}{\ensuremath{0.12400 \pm 0.00700 \pm 0.00700}}%
\htdef{L3.Gamma7.pub.ACCIARRI.95,qt}{\ensuremath{0.12470 \pm 0.00260 \pm 0.00430}}%
\htdef{OPAL.Gamma7.pub.ALEXANDER.91D,qt}{\ensuremath{0.12100 \pm 0.00700 \pm 0.00500}}%
\htdef{Gamma8.qt}{\ensuremath{0.11504 \pm 0.00054}}%
\htdef{CLEO.Gamma8.pub.ANASTASSOV.97,qt}{\ensuremath{0.11520 \pm 0.00050 \pm 0.00120}}%
\htdef{DELPHI.Gamma8.pub.ABDALLAH.06A,qt}{\ensuremath{0.11571 \pm 0.00120 \pm 0.00114}}%
\htdef{OPAL.Gamma8.pub.ACKERSTAFF.98M,qt}{\ensuremath{0.11980 \pm 0.00130 \pm 0.00160}}%
\htdef{Gamma8by5.qt}{\ensuremath{0.6459 \pm 0.0033}}%
\htdef{Gamma9.qt}{\ensuremath{0.10808 \pm 0.00053}}%
\htdef{ALEPH.Gamma9.pub.SCHAEL.05C,qt}{\ensuremath{0.10828 \pm 0.00070 \pm 0.00078}}%
\htdef{Gamma9by5.qt}{\ensuremath{0.6068 \pm 0.0032}}%
\htdef{BaBar.Gamma9by5.pub.AUBERT.10F,qt}{\ensuremath{0.5945 \pm 0.0014 \pm 0.0061}}%
\htdef{Gamma10.qt}{\ensuremath{(0.6957 \pm 0.0096) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma10.pub.BARATE.99K,qt}{\ensuremath{(0.6960 \pm 0.0250 \pm 0.0140) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma10.pub.BATTLE.94,qt}{\ensuremath{(0.6600 \pm 0.0700 \pm 0.0900) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma10.pub.ABREU.94K,qt}{\ensuremath{(0.8500 \pm 0.1800 \pm 0.0000) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma10.pub.ABBIENDI.01J,qt}{\ensuremath{(0.6580 \pm 0.0270 \pm 0.0290) \cdot 10^{-2} }}%
\htdef{Gamma10by5.qt}{\ensuremath{(3.906 \pm 0.054) \cdot 10^{-2}}}%
\htdef{BaBar.Gamma10by5.pub.AUBERT.10F,qt}{\ensuremath{(3.882 \pm 0.032 \pm 0.057) \cdot 10^{-2} }}%
\htdef{Gamma10by9.qt}{\ensuremath{(6.437 \pm 0.092) \cdot 10^{-2}}}%
\htdef{Gamma11.qt}{\ensuremath{0.36977 \pm 0.00098}}%
\htdef{Gamma12.qt}{\ensuremath{0.36477 \pm 0.00098}}%
\htdef{Gamma13.qt}{\ensuremath{0.25918 \pm 0.00090}}%
\htdef{Belle.Gamma13.pub.FUJIKAWA.08,qt}{\ensuremath{0.25670 \pm 0.00010 \pm 0.00390}}%
\htdef{CLEO.Gamma13.pub.ARTUSO.94,qt}{\ensuremath{0.25870 \pm 0.00120 \pm 0.00420}}%
\htdef{DELPHI.Gamma13.pub.ABDALLAH.06A,qt}{\ensuremath{0.25740 \pm 0.00201 \pm 0.00138}}%
\htdef{L3.Gamma13.pub.ACCIARRI.95,qt}{\ensuremath{0.25050 \pm 0.00350 \pm 0.00500}}%
\htdef{OPAL.Gamma13.pub.ACKERSTAFF.98M,qt}{\ensuremath{0.25890 \pm 0.00170 \pm 0.00290}}%
\htdef{Gamma14.qt}{\ensuremath{0.25486 \pm 0.00090}}%
\htdef{ALEPH.Gamma14.pub.SCHAEL.05C,qt}{\ensuremath{0.25471 \pm 0.00097 \pm 0.00085}}%
\htdef{Gamma16.qt}{\ensuremath{(0.4322 \pm 0.0148) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma16.pub.BARATE.99K,qt}{\ensuremath{(0.4440 \pm 0.0260 \pm 0.0240) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma16.pub.AUBERT.07AP,qt}{\ensuremath{(0.4160 \pm 0.0030 \pm 0.0180) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma16.pub.BATTLE.94,qt}{\ensuremath{(0.5100 \pm 0.1000 \pm 0.0700) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma16.pub.ABBIENDI.04J,qt}{\ensuremath{(0.4710 \pm 0.0590 \pm 0.0230) \cdot 10^{-2} }}%
\htdef{Gamma17.qt}{\ensuremath{0.10794 \pm 0.00097}}%
\htdef{OPAL.Gamma17.pub.ACKERSTAFF.98M,qt}{\ensuremath{0.09910 \pm 0.00310 \pm 0.00270}}%
\htdef{Gamma18.qt}{\ensuremath{(9.460 \pm 0.100) \cdot 10^{-2}}}%
\htdef{Gamma19.qt}{\ensuremath{(9.309 \pm 0.100) \cdot 10^{-2}}}%
\htdef{DELPHI.Gamma19.pub.ABDALLAH.06A,qt}{\ensuremath{(9.498 \pm 0.320 \pm 0.275) \cdot 10^{-2} }}%
\htdef{L3.Gamma19.pub.ACCIARRI.95,qt}{\ensuremath{(8.880 \pm 0.370 \pm 0.420) \cdot 10^{-2} }}%
\htdef{Gamma19by13.qt}{\ensuremath{0.3592 \pm 0.0045}}%
\htdef{CLEO.Gamma19by13.pub.PROCARIO.93,qt}{\ensuremath{0.3420 \pm 0.0060 \pm 0.0160}}%
\htdef{Gamma20.qt}{\ensuremath{(9.245 \pm 0.099) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma20.pub.SCHAEL.05C,qt}{\ensuremath{(9.239 \pm 0.086 \pm 0.090) \cdot 10^{-2} }}%
\htdef{Gamma23.qt}{\ensuremath{(0.0634 \pm 0.0219) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma23.pub.BARATE.99K,qt}{\ensuremath{(0.0560 \pm 0.0200 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma23.pub.BATTLE.94,qt}{\ensuremath{(0.0900 \pm 0.1000 \pm 0.0300) \cdot 10^{-2} }}%
\htdef{Gamma24.qt}{\ensuremath{(1.335 \pm 0.066) \cdot 10^{-2}}}%
\htdef{Gamma25.qt}{\ensuremath{(1.250 \pm 0.066) \cdot 10^{-2}}}%
\htdef{DELPHI.Gamma25.pub.ABDALLAH.06A,qt}{\ensuremath{(1.403 \pm 0.214 \pm 0.224) \cdot 10^{-2} }}%
\htdef{Gamma26.qt}{\ensuremath{(1.173 \pm 0.072) \cdot 10^{-2}}}%
\htdef{L3.Gamma26.pub.ACCIARRI.95,qt}{\ensuremath{(1.700 \pm 0.240 \pm 0.380) \cdot 10^{-2} }}%
\htdef{Gamma26by13.qt}{\ensuremath{(4.526 \pm 0.278) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma26by13.pub.PROCARIO.93,qt}{\ensuremath{(4.400 \pm 0.300 \pm 0.500) \cdot 10^{-2} }}%
\htdef{Gamma27.qt}{\ensuremath{(1.040 \pm 0.071) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma27.pub.SCHAEL.05C,qt}{\ensuremath{(0.977 \pm 0.069 \pm 0.058) \cdot 10^{-2} }}%
\htdef{Gamma28.qt}{\ensuremath{(4.648 \pm 2.131) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma28.pub.BARATE.99K,qt}{\ensuremath{(3.700 \pm 2.100 \pm 1.100) \cdot 10^{-4} }}%
\htdef{Gamma29.qt}{\ensuremath{(0.1587 \pm 0.0391) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma29.pub.PROCARIO.93,qt}{\ensuremath{(0.1600 \pm 0.0500 \pm 0.0500) \cdot 10^{-2} }}%
\htdef{Gamma30.qt}{\ensuremath{(0.1118 \pm 0.0391) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma30.pub.SCHAEL.05C,qt}{\ensuremath{(0.1120 \pm 0.0370 \pm 0.0350) \cdot 10^{-2} }}%
\htdef{Gamma31.qt}{\ensuremath{(1.548 \pm 0.029) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma31.pub.BATTLE.94,qt}{\ensuremath{(1.700 \pm 0.120 \pm 0.190) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma31.pub.ABREU.94K,qt}{\ensuremath{(1.540 \pm 0.240 \pm 0.000) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma31.pub.ABBIENDI.01J,qt}{\ensuremath{(1.528 \pm 0.039 \pm 0.040) \cdot 10^{-2} }}%
\htdef{Gamma32.qt}{\ensuremath{(0.8556 \pm 0.0282) \cdot 10^{-2}}}%
\htdef{Gamma33.qt}{\ensuremath{(0.9370 \pm 0.0292) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma33.pub.BARATE.98E,qt}{\ensuremath{(0.9700 \pm 0.0580 \pm 0.0620) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma33.pub.AKERS.94G,qt}{\ensuremath{(0.9700 \pm 0.0900 \pm 0.0600) \cdot 10^{-2} }}%
\htdef{Gamma34.qt}{\ensuremath{(0.9861 \pm 0.0138) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma34.pub.COAN.96,qt}{\ensuremath{(0.8550 \pm 0.0360 \pm 0.0730) \cdot 10^{-2} }}%
\htdef{Gamma35.qt}{\ensuremath{(0.8375 \pm 0.0139) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma35.pub.BARATE.99K,qt}{\ensuremath{(0.9280 \pm 0.0450 \pm 0.0340) \cdot 10^{-2} }}%
\htdef{Belle.Gamma35.pub.RYU.14vpc,qt}{\ensuremath{(0.8320 \pm 0.0025 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{L3.Gamma35.pub.ACCIARRI.95F,qt}{\ensuremath{(0.9500 \pm 0.1500 \pm 0.0600) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma35.pub.ABBIENDI.00C,qt}{\ensuremath{(0.9330 \pm 0.0680 \pm 0.0490) \cdot 10^{-2} }}%
\htdef{Gamma37.qt}{\ensuremath{(0.1486 \pm 0.0034) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma37.pub.BARATE.98E,qt}{\ensuremath{(0.1580 \pm 0.0420 \pm 0.0170) \cdot 10^{-2} }}%
\htdef{ALEPH.Gamma37.pub.BARATE.99K,qt}{\ensuremath{(0.1620 \pm 0.0210 \pm 0.0110) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma37.pub.LEES.18B,qt}{\ensuremath{(0.1478 \pm 0.0022 \pm 0.0040) \cdot 10^{-2} }}%
\htdef{Belle.Gamma37.pub.RYU.14vpc,qt}{\ensuremath{(0.1480 \pm 0.0013 \pm 0.0055) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma37.pub.COAN.96,qt}{\ensuremath{(0.1510 \pm 0.0210 \pm 0.0220) \cdot 10^{-2} }}%
\htdef{Gamma38.qt}{\ensuremath{(0.2985 \pm 0.0073) \cdot 10^{-2}}}%
\htdef{OPAL.Gamma38.pub.ABBIENDI.00C,qt}{\ensuremath{(0.3300 \pm 0.0550 \pm 0.0390) \cdot 10^{-2} }}%
\htdef{Gamma39.qt}{\ensuremath{(0.5310 \pm 0.0134) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma39.pub.COAN.96,qt}{\ensuremath{(0.5620 \pm 0.0500 \pm 0.0480) \cdot 10^{-2} }}%
\htdef{Gamma40.qt}{\ensuremath{(0.3810 \pm 0.0129) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma40.pub.BARATE.98E,qt}{\ensuremath{(0.2940 \pm 0.0730 \pm 0.0370) \cdot 10^{-2} }}%
\htdef{ALEPH.Gamma40.pub.BARATE.99K,qt}{\ensuremath{(0.3470 \pm 0.0530 \pm 0.0370) \cdot 10^{-2} }}%
\htdef{Belle.Gamma40.pub.RYU.14vpc,qt}{\ensuremath{(0.3860 \pm 0.0031 \pm 0.0135) \cdot 10^{-2} }}%
\htdef{L3.Gamma40.pub.ACCIARRI.95F,qt}{\ensuremath{(0.4100 \pm 0.1200 \pm 0.0300) \cdot 10^{-2} }}%
\htdef{Gamma42.qt}{\ensuremath{(0.1499 \pm 0.0070) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma42.pub.BARATE.98E,qt}{\ensuremath{(0.1520 \pm 0.0760 \pm 0.0210) \cdot 10^{-2} }}%
\htdef{ALEPH.Gamma42.pub.BARATE.99K,qt}{\ensuremath{(0.1430 \pm 0.0250 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{Belle.Gamma42.pub.RYU.14vpc,qt}{\ensuremath{(0.1496 \pm 0.0019 \pm 0.0073) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma42.pub.COAN.96,qt}{\ensuremath{(0.1450 \pm 0.0360 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{Gamma43.qt}{\ensuremath{(0.4045 \pm 0.0260) \cdot 10^{-2}}}%
\htdef{OPAL.Gamma43.pub.ABBIENDI.00C,qt}{\ensuremath{(0.3240 \pm 0.0740 \pm 0.0660) \cdot 10^{-2} }}%
\htdef{Gamma44.qt}{\ensuremath{(2.342 \pm 2.306) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma44.pub.BARATE.99R,qt}{\ensuremath{(2.600 \pm 2.400 \pm 0.000) \cdot 10^{-4} }}%
\htdef{Gamma46.qt}{\ensuremath{(0.1517 \pm 0.0247) \cdot 10^{-2}}}%
\htdef{Gamma47.qt}{\ensuremath{(2.349 \pm 0.065) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma47.pub.BARATE.98E,qt}{\ensuremath{(2.600 \pm 1.000 \pm 0.500) \cdot 10^{-4} }}%
\htdef{BaBar.Gamma47.pub.LEES.12Y,qt}{\ensuremath{(2.310 \pm 0.040 \pm 0.080) \cdot 10^{-4} }}%
\htdef{Belle.Gamma47.pub.RYU.14vpc,qt}{\ensuremath{(2.330 \pm 0.033 \pm 0.093) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma47.pub.COAN.96,qt}{\ensuremath{(2.300 \pm 0.500 \pm 0.300) \cdot 10^{-4} }}%
\htdef{Gamma48.qt}{\ensuremath{(0.1048 \pm 0.0247) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma48.pub.BARATE.98E,qt}{\ensuremath{(0.1010 \pm 0.0230 \pm 0.0130) \cdot 10^{-2} }}%
\htdef{Gamma49.qt}{\ensuremath{(3.543 \pm 1.193) \cdot 10^{-4}}}%
\htdef{Gamma50.qt}{\ensuremath{(1.820 \pm 0.207) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma50.pub.LEES.12Y,qt}{\ensuremath{(1.600 \pm 0.200 \pm 0.220) \cdot 10^{-5} }}%
\htdef{Belle.Gamma50.pub.RYU.14vpc,qt}{\ensuremath{(2.000 \pm 0.216 \pm 0.202) \cdot 10^{-5} }}%
\htdef{Gamma51.qt}{\ensuremath{(3.179 \pm 1.192) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma51.pub.BARATE.98E,qt}{\ensuremath{(3.100 \pm 1.100 \pm 0.500) \cdot 10^{-4} }}%
\htdef{Gamma53.qt}{\ensuremath{(2.223 \pm 2.024) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma53.pub.BARATE.98E,qt}{\ensuremath{(2.300 \pm 1.900 \pm 0.700) \cdot 10^{-4} }}%
\htdef{Gamma54.qt}{\ensuremath{0.15193 \pm 0.00063}}%
\htdef{CELLO.Gamma54.pub.BEHREND.89B,qt}{\ensuremath{0.15000 \pm 0.00400 \pm 0.00300}}%
\htdef{L3.Gamma54.pub.ADEVA.91F,qt}{\ensuremath{0.14400 \pm 0.00600 \pm 0.00300}}%
\htdef{TPC.Gamma54.pub.AIHARA.87B,qt}{\ensuremath{0.15100 \pm 0.00800 \pm 0.00600}}%
\htdef{Gamma55.qt}{\ensuremath{0.14545 \pm 0.00058}}%
\htdef{L3.Gamma55.pub.ACHARD.01D,qt}{\ensuremath{0.14556 \pm 0.00105 \pm 0.00076}}%
\htdef{OPAL.Gamma55.pub.AKERS.95Y,qt}{\ensuremath{0.14960 \pm 0.00090 \pm 0.00220}}%
\htdef{Gamma56.qt}{\ensuremath{(9.790 \pm 0.055) \cdot 10^{-2}}}%
\htdef{Gamma57.qt}{\ensuremath{(9.449 \pm 0.054) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma57.pub.BALEST.95C,qt}{\ensuremath{(9.510 \pm 0.070 \pm 0.200) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma57.pub.ABDALLAH.06A,qt}{\ensuremath{(9.317 \pm 0.090 \pm 0.082) \cdot 10^{-2} }}%
\htdef{Gamma57by55.qt}{\ensuremath{0.6496 \pm 0.0031}}%
\htdef{OPAL.Gamma57by55.pub.AKERS.95Y,qt}{\ensuremath{0.6600 \pm 0.0040 \pm 0.0140}}%
\htdef{Gamma58.qt}{\ensuremath{(9.419 \pm 0.054) \cdot 10^{-2}}}%
\htdef{Gamma59.qt}{\ensuremath{(9.300 \pm 0.052) \cdot 10^{-2}}}%
\htdef{Gamma60.qt}{\ensuremath{(9.010 \pm 0.052) \cdot 10^{-2}}}%
\htdef{BaBar.Gamma60.pub.AUBERT.08,qt}{\ensuremath{(8.830 \pm 0.010 \pm 0.130) \cdot 10^{-2} }}%
\htdef{Belle.Gamma60.pub.LEE.10,qt}{\ensuremath{(8.420 \pm 0.000 {}^{+0.260}_{-0.250}) \cdot 10^{-2} }}%
\htdef{CLEO3.Gamma60.pub.BRIERE.03,qt}{\ensuremath{(9.130 \pm 0.050 \pm 0.460) \cdot 10^{-2} }}%
\htdef{Gamma62.qt}{\ensuremath{(8.981 \pm 0.052) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma62.pub.SCHAEL.05C,qt}{\ensuremath{(9.041 \pm 0.060 \pm 0.076) \cdot 10^{-2} }}%
\htdef{Gamma63.qt}{\ensuremath{(5.293 \pm 0.052) \cdot 10^{-2}}}%
\htdef{Gamma64.qt}{\ensuremath{(5.088 \pm 0.052) \cdot 10^{-2}}}%
\htdef{Gamma65.qt}{\ensuremath{(4.757 \pm 0.054) \cdot 10^{-2}}}%
\htdef{Gamma66.qt}{\ensuremath{(4.573 \pm 0.054) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma66.pub.BALEST.95C,qt}{\ensuremath{(4.230 \pm 0.060 \pm 0.220) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma66.pub.ABDALLAH.06A,qt}{\ensuremath{(4.545 \pm 0.106 \pm 0.103) \cdot 10^{-2} }}%
\htdef{Gamma67.qt}{\ensuremath{(2.791 \pm 0.071) \cdot 10^{-2}}}%
\htdef{Gamma68.qt}{\ensuremath{(4.620 \pm 0.054) \cdot 10^{-2}}}%
\htdef{Gamma69.qt}{\ensuremath{(4.488 \pm 0.054) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma69.pub.SCHAEL.05C,qt}{\ensuremath{(4.598 \pm 0.057 \pm 0.064) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma69.pub.EDWARDS.00A,qt}{\ensuremath{(4.190 \pm 0.100 \pm 0.210) \cdot 10^{-2} }}%
\htdef{Gamma70.qt}{\ensuremath{(2.743 \pm 0.071) \cdot 10^{-2}}}%
\htdef{Gamma74.qt}{\ensuremath{(0.5154 \pm 0.0312) \cdot 10^{-2}}}%
\htdef{DELPHI.Gamma74.pub.ABDALLAH.06A,qt}{\ensuremath{(0.5610 \pm 0.0680 \pm 0.0950) \cdot 10^{-2} }}%
\htdef{Gamma75.qt}{\ensuremath{(0.5041 \pm 0.0311) \cdot 10^{-2}}}%
\htdef{Gamma76.qt}{\ensuremath{(0.4942 \pm 0.0311) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma76.pub.SCHAEL.05C,qt}{\ensuremath{(0.4350 \pm 0.0300 \pm 0.0350) \cdot 10^{-2} }}%
\htdef{Gamma76by54.qt}{\ensuremath{(3.252 \pm 0.203) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma76by54.pub.BORTOLETTO.93,qt}{\ensuremath{(3.400 \pm 0.200 \pm 0.300) \cdot 10^{-2} }}%
\htdef{Gamma77.qt}{\ensuremath{(9.790 \pm 3.562) \cdot 10^{-4}}}%
\htdef{Gamma78.qt}{\ensuremath{(2.124 \pm 0.299) \cdot 10^{-4}}}%
\htdef{CLEO.Gamma78.pub.ANASTASSOV.01,qt}{\ensuremath{(2.200 \pm 0.300 \pm 0.400) \cdot 10^{-4} }}%
\htdef{Gamma79.qt}{\ensuremath{(0.6276 \pm 0.0140) \cdot 10^{-2}}}%
\htdef{Gamma80.qt}{\ensuremath{(0.4364 \pm 0.0073) \cdot 10^{-2}}}%
\htdef{Gamma80by60.qt}{\ensuremath{(4.843 \pm 0.079) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma80by60.pub.RICHICHI.99,qt}{\ensuremath{(5.440 \pm 0.210 \pm 0.530) \cdot 10^{-2} }}%
\htdef{Gamma81.qt}{\ensuremath{(8.498 \pm 1.169) \cdot 10^{-4}}}%
\htdef{Gamma81by69.qt}{\ensuremath{(1.893 \pm 0.264) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma81by69.pub.RICHICHI.99,qt}{\ensuremath{(2.610 \pm 0.450 \pm 0.420) \cdot 10^{-2} }}%
\htdef{Gamma82.qt}{\ensuremath{(0.4759 \pm 0.0136) \cdot 10^{-2}}}%
\htdef{TPC.Gamma82.pub.BAUER.94,qt}{\ensuremath{(0.5800 {}^{+0.1500}_{-0.1300} \pm 0.1200) \cdot 10^{-2} }}%
\htdef{Gamma83.qt}{\ensuremath{(0.3719 \pm 0.0134) \cdot 10^{-2}}}%
\htdef{Gamma84.qt}{\ensuremath{(0.3444 \pm 0.0069) \cdot 10^{-2}}}%
\htdef{Gamma85.qt}{\ensuremath{(0.2930 \pm 0.0068) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma85.pub.BARATE.98,qt}{\ensuremath{(0.2140 \pm 0.0370 \pm 0.0290) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma85.pub.AUBERT.08,qt}{\ensuremath{(0.2730 \pm 0.0020 \pm 0.0090) \cdot 10^{-2} }}%
\htdef{Belle.Gamma85.pub.LEE.10,qt}{\ensuremath{(0.3300 \pm 0.0010 {}^{+0.0160}_{-0.0170}) \cdot 10^{-2} }}%
\htdef{CLEO3.Gamma85.pub.BRIERE.03,qt}{\ensuremath{(0.3840 \pm 0.0140 \pm 0.0380) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma85.pub.ABBIENDI.04J,qt}{\ensuremath{(0.4150 \pm 0.0530 \pm 0.0400) \cdot 10^{-2} }}%
\htdef{Gamma85by60.qt}{\ensuremath{(3.252 \pm 0.074) \cdot 10^{-2}}}%
\htdef{Gamma87.qt}{\ensuremath{(0.1308 \pm 0.0119) \cdot 10^{-2}}}%
\htdef{Gamma88.qt}{\ensuremath{(7.891 \pm 1.161) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma88.pub.BARATE.98,qt}{\ensuremath{(6.100 \pm 3.900 \pm 1.800) \cdot 10^{-4} }}%
\htdef{CLEO3.Gamma88.pub.ARMS.05,qt}{\ensuremath{(7.400 \pm 0.800 \pm 1.100) \cdot 10^{-4} }}%
\htdef{Gamma89.qt}{\ensuremath{(7.536 \pm 1.161) \cdot 10^{-4}}}%
\htdef{Gamma92.qt}{\ensuremath{(0.1495 \pm 0.0033) \cdot 10^{-2}}}%
\htdef{OPAL.Gamma92.pub.ABBIENDI.00D,qt}{\ensuremath{(0.1590 \pm 0.0530 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{TPC.Gamma92.pub.BAUER.94,qt}{\ensuremath{(0.1500 {}^{+0.0900}_{-0.0700} \pm 0.0300) \cdot 10^{-2} }}%
\htdef{Gamma93.qt}{\ensuremath{(0.1434 \pm 0.0027) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma93.pub.BARATE.98,qt}{\ensuremath{(0.1630 \pm 0.0210 \pm 0.0170) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma93.pub.AUBERT.08,qt}{\ensuremath{(0.1346 \pm 0.0010 \pm 0.0036) \cdot 10^{-2} }}%
\htdef{Belle.Gamma93.pub.LEE.10,qt}{\ensuremath{(0.1550 \pm 0.0010 {}^{+0.0060}_{-0.0050}) \cdot 10^{-2} }}%
\htdef{CLEO3.Gamma93.pub.BRIERE.03,qt}{\ensuremath{(0.1550 \pm 0.0060 \pm 0.0090) \cdot 10^{-2} }}%
\htdef{Gamma93by60.qt}{\ensuremath{(1.592 \pm 0.030) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma93by60.pub.RICHICHI.99,qt}{\ensuremath{(1.600 \pm 0.150 \pm 0.300) \cdot 10^{-2} }}%
\htdef{Gamma94.qt}{\ensuremath{(0.607 \pm 0.183) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma94.pub.BARATE.98,qt}{\ensuremath{(7.500 \pm 2.900 \pm 1.500) \cdot 10^{-4} }}%
\htdef{CLEO3.Gamma94.pub.ARMS.05,qt}{\ensuremath{(0.550 \pm 0.140 \pm 0.120) \cdot 10^{-4} }}%
\htdef{Gamma94by69.qt}{\ensuremath{(0.1352 \pm 0.0408) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma94by69.pub.RICHICHI.99,qt}{\ensuremath{(0.7900 \pm 0.4400 \pm 0.1600) \cdot 10^{-2} }}%
\htdef{Gamma96.qt}{\ensuremath{(2.169 \pm 0.800) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma96.pub.AUBERT.08,qt}{\ensuremath{(1.578 \pm 0.130 \pm 0.123) \cdot 10^{-5} }}%
\htdef{Belle.Gamma96.pub.LEE.10,qt}{\ensuremath{(3.290 \pm 0.170 {}^{+0.190}_{-0.200}) \cdot 10^{-5} }}%
\htdef{Gamma102.qt}{\ensuremath{(0.0993 \pm 0.0037) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma102.pub.GIBAUT.94B,qt}{\ensuremath{(0.0970 \pm 0.0050 \pm 0.0110) \cdot 10^{-2} }}%
\htdef{HRS.Gamma102.pub.BYLSMA.87,qt}{\ensuremath{(0.1020 \pm 0.0290 \pm 0.0000) \cdot 10^{-2} }}%
\htdef{L3.Gamma102.pub.ACHARD.01D,qt}{\ensuremath{(0.1700 \pm 0.0220 \pm 0.0260) \cdot 10^{-2} }}%
\htdef{Gamma103.qt}{\ensuremath{(8.281 \pm 0.314) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma103.pub.SCHAEL.05C,qt}{\ensuremath{(7.200 \pm 0.900 \pm 1.200) \cdot 10^{-4} }}%
\htdef{ARGUS.Gamma103.pub.ALBRECHT.88B,qt}{\ensuremath{(6.400 \pm 2.300 \pm 1.000) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma103.pub.GIBAUT.94B,qt}{\ensuremath{(7.700 \pm 0.500 \pm 0.900) \cdot 10^{-4} }}%
\htdef{DELPHI.Gamma103.pub.ABDALLAH.06A,qt}{\ensuremath{(9.700 \pm 1.500 \pm 0.500) \cdot 10^{-4} }}%
\htdef{HRS.Gamma103.pub.BYLSMA.87,qt}{\ensuremath{(5.100 \pm 2.000 \pm 0.000) \cdot 10^{-4} }}%
\htdef{OPAL.Gamma103.pub.ACKERSTAFF.99E,qt}{\ensuremath{(9.100 \pm 1.400 \pm 0.600) \cdot 10^{-4} }}%
\htdef{Gamma104.qt}{\ensuremath{(1.645 \pm 0.114) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma104.pub.SCHAEL.05C,qt}{\ensuremath{(2.100 \pm 0.700 \pm 0.900) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma104.pub.ANASTASSOV.01,qt}{\ensuremath{(1.700 \pm 0.200 \pm 0.200) \cdot 10^{-4} }}%
\htdef{DELPHI.Gamma104.pub.ABDALLAH.06A,qt}{\ensuremath{(1.600 \pm 1.200 \pm 0.600) \cdot 10^{-4} }}%
\htdef{OPAL.Gamma104.pub.ACKERSTAFF.99E,qt}{\ensuremath{(2.700 \pm 1.800 \pm 0.900) \cdot 10^{-4} }}%
\htdef{Gamma106.qt}{\ensuremath{(0.7793 \pm 0.0534) \cdot 10^{-2}}}%
\htdef{Gamma110.qt}{\ensuremath{(2.908 \pm 0.048) \cdot 10^{-2}}}%
\htdef{Gamma126.qt}{\ensuremath{(0.1386 \pm 0.0072) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma126.pub.BUSKULIC.97C,qt}{\ensuremath{(0.1800 \pm 0.0400 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{Belle.Gamma126.pub.INAMI.09,qt}{\ensuremath{(0.1350 \pm 0.0030 \pm 0.0070) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma126.pub.ARTUSO.92,qt}{\ensuremath{(0.1700 \pm 0.0200 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{Gamma128.qt}{\ensuremath{(1.547 \pm 0.080) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma128.pub.BUSKULIC.97C,qt}{\ensuremath{(2.900 {}^{+1.300}_{-1.200} \pm 0.700) \cdot 10^{-4} }}%
\htdef{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,qt}{\ensuremath{(1.420 \pm 0.110 \pm 0.070) \cdot 10^{-4} }}%
\htdef{Belle.Gamma128.pub.INAMI.09,qt}{\ensuremath{(1.580 \pm 0.050 \pm 0.090) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma128.pub.BARTELT.96,qt}{\ensuremath{(2.600 \pm 0.500 \pm 0.500) \cdot 10^{-4} }}%
\htdef{Gamma130.qt}{\ensuremath{(0.483 \pm 0.116) \cdot 10^{-4}}}%
\htdef{Belle.Gamma130.pub.INAMI.09,qt}{\ensuremath{(0.460 \pm 0.110 \pm 0.040) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma130.pub.BISHAI.99,qt}{\ensuremath{(1.770 \pm 0.560 \pm 0.710) \cdot 10^{-4} }}%
\htdef{Gamma132.qt}{\ensuremath{(0.937 \pm 0.149) \cdot 10^{-4}}}%
\htdef{Belle.Gamma132.pub.INAMI.09,qt}{\ensuremath{(0.880 \pm 0.140 \pm 0.060) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma132.pub.BISHAI.99,qt}{\ensuremath{(2.200 \pm 0.700 \pm 0.220) \cdot 10^{-4} }}%
\htdef{Gamma136.qt}{\ensuremath{(2.202 \pm 0.129) \cdot 10^{-4}}}%
\htdef{Gamma149.qt}{\ensuremath{(2.395 \pm 0.075) \cdot 10^{-2}}}%
\htdef{Gamma150.qt}{\ensuremath{(1.988 \pm 0.064) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma150.pub.BUSKULIC.97C,qt}{\ensuremath{(1.910 \pm 0.070 \pm 0.060) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma150.pub.BARINGER.87,qt}{\ensuremath{(1.600 \pm 0.270 \pm 0.410) \cdot 10^{-2} }}%
\htdef{Gamma150by66.qt}{\ensuremath{0.4348 \pm 0.0140}}%
\htdef{ALEPH.Gamma150by66.pub.BUSKULIC.96,qt}{\ensuremath{0.4310 \pm 0.0330 \pm 0.0000}}%
\htdef{CLEO.Gamma150by66.pub.BALEST.95C,qt}{\ensuremath{0.4640 \pm 0.0160 \pm 0.0170}}%
\htdef{Gamma151.qt}{\ensuremath{(4.101 \pm 0.922) \cdot 10^{-4}}}%
\htdef{CLEO3.Gamma151.pub.ARMS.05,qt}{\ensuremath{(4.100 \pm 0.600 \pm 0.700) \cdot 10^{-4} }}%
\htdef{Gamma152.qt}{\ensuremath{(0.4069 \pm 0.0419) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma152.pub.BUSKULIC.97C,qt}{\ensuremath{(0.4300 \pm 0.0600 \pm 0.0500) \cdot 10^{-2} }}%
\htdef{Gamma152by54.qt}{\ensuremath{(2.678 \pm 0.275) \cdot 10^{-2}}}%
\htdef{Gamma152by76.qt}{\ensuremath{0.8235 \pm 0.0757}}%
\htdef{CLEO.Gamma152by76.pub.BORTOLETTO.93,qt}{\ensuremath{0.8100 \pm 0.0600 \pm 0.0600}}%
\htdef{Gamma167.qt}{\ensuremath{(4.408 \pm 1.626) \cdot 10^{-5}}}%
\htdef{Gamma168.qt}{\ensuremath{(2.169 \pm 0.800) \cdot 10^{-5}}}%
\htdef{Gamma169.qt}{\ensuremath{(1.499 \pm 0.553) \cdot 10^{-5}}}%
\htdef{Gamma800.qt}{\ensuremath{(1.947 \pm 0.065) \cdot 10^{-2}}}%
\htdef{Gamma802.qt}{\ensuremath{(0.2924 \pm 0.0068) \cdot 10^{-2}}}%
\htdef{Gamma803.qt}{\ensuremath{(3.874 \pm 1.423) \cdot 10^{-4}}}%
\htdef{Gamma804.qt}{\ensuremath{(2.349 \pm 0.065) \cdot 10^{-4}}}%
\htdef{Gamma805.qt}{\ensuremath{(4.000 \pm 2.000) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma805.pub.SCHAEL.05C,qt}{\ensuremath{(4.000 \pm 2.000 \pm 0.000) \cdot 10^{-4} }}%
\htdef{Gamma806.qt}{\ensuremath{(1.820 \pm 0.207) \cdot 10^{-5}}}%
\htdef{Gamma810.qt}{\ensuremath{(1.940 \pm 0.298) \cdot 10^{-4}}}%
\htdef{Gamma811.qt}{\ensuremath{(7.164 \pm 1.586) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma811.pub.LEES.12X,qt}{\ensuremath{(7.300 \pm 1.200 \pm 1.200) \cdot 10^{-5} }}%
\htdef{Gamma812.qt}{\ensuremath{(1.353 \pm 2.683) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma812.pub.LEES.12X,qt}{\ensuremath{(1.000 \pm 0.800 \pm 3.000) \cdot 10^{-5} }}%
\htdef{Gamma820.qt}{\ensuremath{(8.262 \pm 0.313) \cdot 10^{-4}}}%
\htdef{Gamma821.qt}{\ensuremath{(7.738 \pm 0.295) \cdot 10^{-4}}}%
\htdef{BaBar.Gamma821.pub.LEES.12X,qt}{\ensuremath{(7.680 \pm 0.040 \pm 0.400) \cdot 10^{-4} }}%
\htdef{Gamma822.qt}{\ensuremath{(0.593 \pm 1.208) \cdot 10^{-6}}}%
\htdef{BaBar.Gamma822.pub.LEES.12X,qt}{\ensuremath{(0.600 \pm 0.500 \pm 1.100) \cdot 10^{-6} }}%
\htdef{Gamma830.qt}{\ensuremath{(1.633 \pm 0.113) \cdot 10^{-4}}}%
\htdef{Gamma831.qt}{\ensuremath{(8.417 \pm 0.624) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma831.pub.LEES.12X,qt}{\ensuremath{(8.400 \pm 0.400 \pm 0.600) \cdot 10^{-5} }}%
\htdef{Gamma832.qt}{\ensuremath{(3.772 \pm 0.874) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma832.pub.LEES.12X,qt}{\ensuremath{(3.600 \pm 0.300 \pm 0.900) \cdot 10^{-5} }}%
\htdef{Gamma833.qt}{\ensuremath{(1.107 \pm 0.566) \cdot 10^{-6}}}%
\htdef{BaBar.Gamma833.pub.LEES.12X,qt}{\ensuremath{(1.100 \pm 0.400 \pm 0.400) \cdot 10^{-6} }}%
\htdef{Gamma910.qt}{\ensuremath{(7.195 \pm 0.422) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma910.pub.LEES.12X,qt}{\ensuremath{(8.270 \pm 0.880 \pm 0.810) \cdot 10^{-5} }}%
\htdef{Gamma911.qt}{\ensuremath{(4.457 \pm 0.867) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma911.pub.LEES.12X,qt}{\ensuremath{(4.570 \pm 0.770 \pm 0.500) \cdot 10^{-5} }}%
\htdef{Gamma920.qt}{\ensuremath{(5.237 \pm 0.444) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma920.pub.LEES.12X,qt}{\ensuremath{(5.200 \pm 0.310 \pm 0.370) \cdot 10^{-5} }}%
\htdef{Gamma930.qt}{\ensuremath{(5.046 \pm 0.296) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma930.pub.LEES.12X,qt}{\ensuremath{(5.390 \pm 0.270 \pm 0.410) \cdot 10^{-5} }}%
\htdef{Gamma944.qt}{\ensuremath{(8.676 \pm 0.509) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma944.pub.LEES.12X,qt}{\ensuremath{(8.260 \pm 0.350 \pm 0.510) \cdot 10^{-5} }}%
\htdef{Gamma945.qt}{\ensuremath{(1.945 \pm 0.378) \cdot 10^{-4}}}%
\htdef{Gamma998.qt}{\ensuremath{(0.0684 \pm 0.1068) \cdot 10^{-2}}}%
\htdef{Gamma1.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma1.gn} = \htuse{Gamma1.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma1.qt} & average &}%
\htdef{Gamma2.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma2.gn} = \htuse{Gamma2.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma2.qt} & average &}%
\htdef{Gamma3.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma3.qt} & average & \\
\htuse{ALEPH.Gamma3.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma3.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma3.pub.SCHAEL.05C,ref} \\
\htuse{DELPHI.Gamma3.pub.ABREU.99X,qt} & \htuse{DELPHI.Gamma3.pub.ABREU.99X,exp} & \htuse{DELPHI.Gamma3.pub.ABREU.99X,ref} \\
\htuse{L3.Gamma3.pub.ACCIARRI.01F,qt} & \htuse{L3.Gamma3.pub.ACCIARRI.01F,exp} & \htuse{L3.Gamma3.pub.ACCIARRI.01F,ref} \\
\htuse{OPAL.Gamma3.pub.ABBIENDI.03,qt} & \htuse{OPAL.Gamma3.pub.ABBIENDI.03,exp} & \htuse{OPAL.Gamma3.pub.ABBIENDI.03,ref}
}%
\htdef{Gamma3by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma3by5.qt} & average & \\
\htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D,qt} & \htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D,exp} & \htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D,ref} \\
\htuse{BaBar.Gamma3by5.pub.AUBERT.10F,qt} & \htuse{BaBar.Gamma3by5.pub.AUBERT.10F,exp} & \htuse{BaBar.Gamma3by5.pub.AUBERT.10F,ref} \\
\htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97,qt} & \htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97,exp} & \htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97,ref}
}%
\htdef{Gamma5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma5.qt} & average & \\
\htuse{ALEPH.Gamma5.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma5.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma5.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma5.pub.ANASTASSOV.97,qt} & \htuse{CLEO.Gamma5.pub.ANASTASSOV.97,exp} & \htuse{CLEO.Gamma5.pub.ANASTASSOV.97,ref} \\
\htuse{DELPHI.Gamma5.pub.ABREU.99X,qt} & \htuse{DELPHI.Gamma5.pub.ABREU.99X,exp} & \htuse{DELPHI.Gamma5.pub.ABREU.99X,ref} \\
\htuse{L3.Gamma5.pub.ACCIARRI.01F,qt} & \htuse{L3.Gamma5.pub.ACCIARRI.01F,exp} & \htuse{L3.Gamma5.pub.ACCIARRI.01F,ref} \\
\htuse{OPAL.Gamma5.pub.ABBIENDI.99H,qt} & \htuse{OPAL.Gamma5.pub.ABBIENDI.99H,exp} & \htuse{OPAL.Gamma5.pub.ABBIENDI.99H,ref}
}%
\htdef{Gamma7.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma7.qt} & average & \\
\htuse{DELPHI.Gamma7.pub.ABREU.92N,qt} & \htuse{DELPHI.Gamma7.pub.ABREU.92N,exp} & \htuse{DELPHI.Gamma7.pub.ABREU.92N,ref} \\
\htuse{L3.Gamma7.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma7.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma7.pub.ACCIARRI.95,ref} \\
\htuse{OPAL.Gamma7.pub.ALEXANDER.91D,qt} & \htuse{OPAL.Gamma7.pub.ALEXANDER.91D,exp} & \htuse{OPAL.Gamma7.pub.ALEXANDER.91D,ref}
}%
\htdef{Gamma8.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma8.qt} & average & \\
\htuse{CLEO.Gamma8.pub.ANASTASSOV.97,qt} & \htuse{CLEO.Gamma8.pub.ANASTASSOV.97,exp} & \htuse{CLEO.Gamma8.pub.ANASTASSOV.97,ref} \\
\htuse{DELPHI.Gamma8.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma8.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma8.pub.ABDALLAH.06A,ref} \\
\htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M,qt} & \htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M,exp} & \htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M,ref}
}%
\htdef{Gamma8by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma8by5.gn} = \htuse{Gamma8by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma8by5.qt} & average &}%
\htdef{Gamma9.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma9.gn} = \htuse{Gamma9.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma9.qt} & average & \\
\htuse{ALEPH.Gamma9.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma9.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma9.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma9by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma9by5.gn} = \htuse{Gamma9by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma9by5.qt} & average & \\
\htuse{BaBar.Gamma9by5.pub.AUBERT.10F,qt} & \htuse{BaBar.Gamma9by5.pub.AUBERT.10F,exp} & \htuse{BaBar.Gamma9by5.pub.AUBERT.10F,ref}
}%
\htdef{Gamma10.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma10.qt} & average & \\
\htuse{ALEPH.Gamma10.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma10.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma10.pub.BARATE.99K,ref} \\
\htuse{CLEO.Gamma10.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma10.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma10.pub.BATTLE.94,ref} \\
\htuse{DELPHI.Gamma10.pub.ABREU.94K,qt} & \htuse{DELPHI.Gamma10.pub.ABREU.94K,exp} & \htuse{DELPHI.Gamma10.pub.ABREU.94K,ref} \\
\htuse{OPAL.Gamma10.pub.ABBIENDI.01J,qt} & \htuse{OPAL.Gamma10.pub.ABBIENDI.01J,exp} & \htuse{OPAL.Gamma10.pub.ABBIENDI.01J,ref}
}%
\htdef{Gamma10by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma10by5.gn} = \htuse{Gamma10by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma10by5.qt} & average & \\
\htuse{BaBar.Gamma10by5.pub.AUBERT.10F,qt} & \htuse{BaBar.Gamma10by5.pub.AUBERT.10F,exp} & \htuse{BaBar.Gamma10by5.pub.AUBERT.10F,ref}
}%
\htdef{Gamma10by9.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma10by9.gn} = \htuse{Gamma10by9.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma10by9.qt} & average &}%
\htdef{Gamma11.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma11.gn} = \htuse{Gamma11.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma11.qt} & average &}%
\htdef{Gamma12.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma12.gn} = \htuse{Gamma12.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma12.qt} & average &}%
\htdef{Gamma13.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma13.qt} & average & \\
\htuse{Belle.Gamma13.pub.FUJIKAWA.08,qt} & \htuse{Belle.Gamma13.pub.FUJIKAWA.08,exp} & \htuse{Belle.Gamma13.pub.FUJIKAWA.08,ref} \\
\htuse{CLEO.Gamma13.pub.ARTUSO.94,qt} & \htuse{CLEO.Gamma13.pub.ARTUSO.94,exp} & \htuse{CLEO.Gamma13.pub.ARTUSO.94,ref} \\
\htuse{DELPHI.Gamma13.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma13.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma13.pub.ABDALLAH.06A,ref} \\
\htuse{L3.Gamma13.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma13.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma13.pub.ACCIARRI.95,ref} \\
\htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M,qt} & \htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M,exp} & \htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M,ref}
}%
\htdef{Gamma14.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma14.gn} = \htuse{Gamma14.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma14.qt} & average & \\
\htuse{ALEPH.Gamma14.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma14.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma14.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma16.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma16.qt} & average & \\
\htuse{ALEPH.Gamma16.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma16.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma16.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma16.pub.AUBERT.07AP,qt} & \htuse{BaBar.Gamma16.pub.AUBERT.07AP,exp} & \htuse{BaBar.Gamma16.pub.AUBERT.07AP,ref} \\
\htuse{CLEO.Gamma16.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma16.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma16.pub.BATTLE.94,ref} \\
\htuse{OPAL.Gamma16.pub.ABBIENDI.04J,qt} & \htuse{OPAL.Gamma16.pub.ABBIENDI.04J,exp} & \htuse{OPAL.Gamma16.pub.ABBIENDI.04J,ref}
}%
\htdef{Gamma17.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma17.gn} = \htuse{Gamma17.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma17.qt} & average & \\
\htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M,qt} & \htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M,exp} & \htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M,ref}
}%
\htdef{Gamma18.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma18.gn} = \htuse{Gamma18.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma18.qt} & average &}%
\htdef{Gamma19.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma19.qt} & average & \\
\htuse{DELPHI.Gamma19.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma19.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma19.pub.ABDALLAH.06A,ref} \\
\htuse{L3.Gamma19.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma19.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma19.pub.ACCIARRI.95,ref}
}%
\htdef{Gamma19by13.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma19by13.gn} = \htuse{Gamma19by13.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma19by13.qt} & average & \\
\htuse{CLEO.Gamma19by13.pub.PROCARIO.93,qt} & \htuse{CLEO.Gamma19by13.pub.PROCARIO.93,exp} & \htuse{CLEO.Gamma19by13.pub.PROCARIO.93,ref}
}%
\htdef{Gamma20.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma20.gn} = \htuse{Gamma20.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma20.qt} & average & \\
\htuse{ALEPH.Gamma20.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma20.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma20.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma23.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma23.qt} & average & \\
\htuse{ALEPH.Gamma23.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma23.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma23.pub.BARATE.99K,ref} \\
\htuse{CLEO.Gamma23.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma23.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma23.pub.BATTLE.94,ref}
}%
\htdef{Gamma24.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma24.gn} = \htuse{Gamma24.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma24.qt} & average &}%
\htdef{Gamma25.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma25.gn} = \htuse{Gamma25.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma25.qt} & average & \\
\htuse{DELPHI.Gamma25.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma25.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma25.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma26.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma26.gn} = \htuse{Gamma26.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma26.qt} & average & \\
\htuse{L3.Gamma26.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma26.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma26.pub.ACCIARRI.95,ref}
}%
\htdef{Gamma26by13.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma26by13.gn} = \htuse{Gamma26by13.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma26by13.qt} & average & \\
\htuse{CLEO.Gamma26by13.pub.PROCARIO.93,qt} & \htuse{CLEO.Gamma26by13.pub.PROCARIO.93,exp} & \htuse{CLEO.Gamma26by13.pub.PROCARIO.93,ref}
}%
\htdef{Gamma27.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma27.gn} = \htuse{Gamma27.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma27.qt} & average & \\
\htuse{ALEPH.Gamma27.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma27.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma27.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma28.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma28.gn} = \htuse{Gamma28.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma28.qt} & average & \\
\htuse{ALEPH.Gamma28.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma28.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma28.pub.BARATE.99K,ref}
}%
\htdef{Gamma29.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma29.gn} = \htuse{Gamma29.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma29.qt} & average & \\
\htuse{CLEO.Gamma29.pub.PROCARIO.93,qt} & \htuse{CLEO.Gamma29.pub.PROCARIO.93,exp} & \htuse{CLEO.Gamma29.pub.PROCARIO.93,ref}
}%
\htdef{Gamma30.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma30.gn} = \htuse{Gamma30.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma30.qt} & average & \\
\htuse{ALEPH.Gamma30.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma30.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma30.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma31.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma31.qt} & average & \\
\htuse{CLEO.Gamma31.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma31.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma31.pub.BATTLE.94,ref} \\
\htuse{DELPHI.Gamma31.pub.ABREU.94K,qt} & \htuse{DELPHI.Gamma31.pub.ABREU.94K,exp} & \htuse{DELPHI.Gamma31.pub.ABREU.94K,ref} \\
\htuse{OPAL.Gamma31.pub.ABBIENDI.01J,qt} & \htuse{OPAL.Gamma31.pub.ABBIENDI.01J,exp} & \htuse{OPAL.Gamma31.pub.ABBIENDI.01J,ref}
}%
\htdef{Gamma32.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma32.gn} = \htuse{Gamma32.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma32.qt} & average &}%
\htdef{Gamma33.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma33.gn} = \htuse{Gamma33.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma33.qt} & average & \\
\htuse{ALEPH.Gamma33.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma33.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma33.pub.BARATE.98E,ref} \\
\htuse{OPAL.Gamma33.pub.AKERS.94G,qt} & \htuse{OPAL.Gamma33.pub.AKERS.94G,exp} & \htuse{OPAL.Gamma33.pub.AKERS.94G,ref}
}%
\htdef{Gamma34.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma34.gn} = \htuse{Gamma34.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma34.qt} & average & \\
\htuse{CLEO.Gamma34.pub.COAN.96,qt} & \htuse{CLEO.Gamma34.pub.COAN.96,exp} & \htuse{CLEO.Gamma34.pub.COAN.96,ref}
}%
\htdef{Gamma35.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma35.qt} & average & \\
\htuse{ALEPH.Gamma35.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma35.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma35.pub.BARATE.99K,ref} \\
\htuse{Belle.Gamma35.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma35.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma35.pub.RYU.14vpc,ref} \\
\htuse{L3.Gamma35.pub.ACCIARRI.95F,qt} & \htuse{L3.Gamma35.pub.ACCIARRI.95F,exp} & \htuse{L3.Gamma35.pub.ACCIARRI.95F,ref} \\
\htuse{OPAL.Gamma35.pub.ABBIENDI.00C,qt} & \htuse{OPAL.Gamma35.pub.ABBIENDI.00C,exp} & \htuse{OPAL.Gamma35.pub.ABBIENDI.00C,ref}
}%
\htdef{Gamma37.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma37.qt} & average & \\
\htuse{ALEPH.Gamma37.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma37.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma37.pub.BARATE.98E,ref} \\
\htuse{ALEPH.Gamma37.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma37.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma37.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma37.pub.LEES.18B,qt} & \htuse{BaBar.Gamma37.pub.LEES.18B,exp} & \htuse{BaBar.Gamma37.pub.LEES.18B,ref} \\
\htuse{Belle.Gamma37.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma37.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma37.pub.RYU.14vpc,ref} \\
\htuse{CLEO.Gamma37.pub.COAN.96,qt} & \htuse{CLEO.Gamma37.pub.COAN.96,exp} & \htuse{CLEO.Gamma37.pub.COAN.96,ref}
}%
\htdef{Gamma38.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma38.gn} = \htuse{Gamma38.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma38.qt} & average & \\
\htuse{OPAL.Gamma38.pub.ABBIENDI.00C,qt} & \htuse{OPAL.Gamma38.pub.ABBIENDI.00C,exp} & \htuse{OPAL.Gamma38.pub.ABBIENDI.00C,ref}
}%
\htdef{Gamma39.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma39.gn} = \htuse{Gamma39.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma39.qt} & average & \\
\htuse{CLEO.Gamma39.pub.COAN.96,qt} & \htuse{CLEO.Gamma39.pub.COAN.96,exp} & \htuse{CLEO.Gamma39.pub.COAN.96,ref}
}%
\htdef{Gamma40.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma40.qt} & average & \\
\htuse{ALEPH.Gamma40.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma40.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma40.pub.BARATE.98E,ref} \\
\htuse{ALEPH.Gamma40.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma40.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma40.pub.BARATE.99K,ref} \\
\htuse{Belle.Gamma40.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma40.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma40.pub.RYU.14vpc,ref} \\
\htuse{L3.Gamma40.pub.ACCIARRI.95F,qt} & \htuse{L3.Gamma40.pub.ACCIARRI.95F,exp} & \htuse{L3.Gamma40.pub.ACCIARRI.95F,ref}
}%
\htdef{Gamma42.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma42.qt} & average & \\
\htuse{ALEPH.Gamma42.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma42.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma42.pub.BARATE.98E,ref} \\
\htuse{ALEPH.Gamma42.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma42.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma42.pub.BARATE.99K,ref} \\
\htuse{Belle.Gamma42.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma42.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma42.pub.RYU.14vpc,ref} \\
\htuse{CLEO.Gamma42.pub.COAN.96,qt} & \htuse{CLEO.Gamma42.pub.COAN.96,exp} & \htuse{CLEO.Gamma42.pub.COAN.96,ref}
}%
\htdef{Gamma43.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma43.gn} = \htuse{Gamma43.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma43.qt} & average & \\
\htuse{OPAL.Gamma43.pub.ABBIENDI.00C,qt} & \htuse{OPAL.Gamma43.pub.ABBIENDI.00C,exp} & \htuse{OPAL.Gamma43.pub.ABBIENDI.00C,ref}
}%
\htdef{Gamma44.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma44.gn} = \htuse{Gamma44.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma44.qt} & average & \\
\htuse{ALEPH.Gamma44.pub.BARATE.99R,qt} & \htuse{ALEPH.Gamma44.pub.BARATE.99R,exp} & \htuse{ALEPH.Gamma44.pub.BARATE.99R,ref}
}%
\htdef{Gamma46.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma46.gn} = \htuse{Gamma46.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma46.qt} & average &}%
\htdef{Gamma47.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma47.qt} & average & \\
\htuse{ALEPH.Gamma47.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma47.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma47.pub.BARATE.98E,ref} \\
\htuse{BaBar.Gamma47.pub.LEES.12Y,qt} & \htuse{BaBar.Gamma47.pub.LEES.12Y,exp} & \htuse{BaBar.Gamma47.pub.LEES.12Y,ref} \\
\htuse{Belle.Gamma47.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma47.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma47.pub.RYU.14vpc,ref} \\
\htuse{CLEO.Gamma47.pub.COAN.96,qt} & \htuse{CLEO.Gamma47.pub.COAN.96,exp} & \htuse{CLEO.Gamma47.pub.COAN.96,ref}
}%
\htdef{Gamma48.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma48.gn} = \htuse{Gamma48.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma48.qt} & average & \\
\htuse{ALEPH.Gamma48.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma48.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma48.pub.BARATE.98E,ref}
}%
\htdef{Gamma49.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma49.gn} = \htuse{Gamma49.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma49.qt} & average &}%
\htdef{Gamma50.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma50.gn} = \htuse{Gamma50.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma50.qt} & average & \\
\htuse{BaBar.Gamma50.pub.LEES.12Y,qt} & \htuse{BaBar.Gamma50.pub.LEES.12Y,exp} & \htuse{BaBar.Gamma50.pub.LEES.12Y,ref} \\
\htuse{Belle.Gamma50.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma50.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma50.pub.RYU.14vpc,ref}
}%
\htdef{Gamma51.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma51.gn} = \htuse{Gamma51.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma51.qt} & average & \\
\htuse{ALEPH.Gamma51.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma51.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma51.pub.BARATE.98E,ref}
}%
\htdef{Gamma53.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma53.gn} = \htuse{Gamma53.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma53.qt} & average & \\
\htuse{ALEPH.Gamma53.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma53.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma53.pub.BARATE.98E,ref}
}%
\htdef{Gamma54.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma54.qt} & average & \\
\htuse{CELLO.Gamma54.pub.BEHREND.89B,qt} & \htuse{CELLO.Gamma54.pub.BEHREND.89B,exp} & \htuse{CELLO.Gamma54.pub.BEHREND.89B,ref} \\
\htuse{L3.Gamma54.pub.ADEVA.91F,qt} & \htuse{L3.Gamma54.pub.ADEVA.91F,exp} & \htuse{L3.Gamma54.pub.ADEVA.91F,ref} \\
\htuse{TPC.Gamma54.pub.AIHARA.87B,qt} & \htuse{TPC.Gamma54.pub.AIHARA.87B,exp} & \htuse{TPC.Gamma54.pub.AIHARA.87B,ref}
}%
\htdef{Gamma55.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma55.gn} = \htuse{Gamma55.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma55.qt} & average & \\
\htuse{L3.Gamma55.pub.ACHARD.01D,qt} & \htuse{L3.Gamma55.pub.ACHARD.01D,exp} & \htuse{L3.Gamma55.pub.ACHARD.01D,ref} \\
\htuse{OPAL.Gamma55.pub.AKERS.95Y,qt} & \htuse{OPAL.Gamma55.pub.AKERS.95Y,exp} & \htuse{OPAL.Gamma55.pub.AKERS.95Y,ref}
}%
\htdef{Gamma56.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma56.gn} = \htuse{Gamma56.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma56.qt} & average &}%
\htdef{Gamma57.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma57.gn} = \htuse{Gamma57.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma57.qt} & average & \\
\htuse{CLEO.Gamma57.pub.BALEST.95C,qt} & \htuse{CLEO.Gamma57.pub.BALEST.95C,exp} & \htuse{CLEO.Gamma57.pub.BALEST.95C,ref} \\
\htuse{DELPHI.Gamma57.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma57.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma57.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma57by55.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma57by55.gn} = \htuse{Gamma57by55.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma57by55.qt} & average & \\
\htuse{OPAL.Gamma57by55.pub.AKERS.95Y,qt} & \htuse{OPAL.Gamma57by55.pub.AKERS.95Y,exp} & \htuse{OPAL.Gamma57by55.pub.AKERS.95Y,ref}
}%
\htdef{Gamma58.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma58.gn} = \htuse{Gamma58.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma58.qt} & average &}%
\htdef{Gamma59.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma59.gn} = \htuse{Gamma59.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma59.qt} & average &}%
\htdef{Gamma60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma60.qt} & average & \\
\htuse{BaBar.Gamma60.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma60.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma60.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma60.pub.LEE.10,qt} & \htuse{Belle.Gamma60.pub.LEE.10,exp} & \htuse{Belle.Gamma60.pub.LEE.10,ref} \\
\htuse{CLEO3.Gamma60.pub.BRIERE.03,qt} & \htuse{CLEO3.Gamma60.pub.BRIERE.03,exp} & \htuse{CLEO3.Gamma60.pub.BRIERE.03,ref}
}%
\htdef{Gamma62.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma62.gn} = \htuse{Gamma62.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma62.qt} & average & \\
\htuse{ALEPH.Gamma62.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma62.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma62.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma63.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma63.gn} = \htuse{Gamma63.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma63.qt} & average &}%
\htdef{Gamma64.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma64.gn} = \htuse{Gamma64.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma64.qt} & average &}%
\htdef{Gamma65.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma65.gn} = \htuse{Gamma65.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma65.qt} & average &}%
\htdef{Gamma66.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma66.qt} & average & \\
\htuse{CLEO.Gamma66.pub.BALEST.95C,qt} & \htuse{CLEO.Gamma66.pub.BALEST.95C,exp} & \htuse{CLEO.Gamma66.pub.BALEST.95C,ref} \\
\htuse{DELPHI.Gamma66.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma66.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma66.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma67.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma67.gn} = \htuse{Gamma67.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma67.qt} & average &}%
\htdef{Gamma68.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma68.gn} = \htuse{Gamma68.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma68.qt} & average &}%
\htdef{Gamma69.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma69.gn} = \htuse{Gamma69.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma69.qt} & average & \\
\htuse{ALEPH.Gamma69.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma69.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma69.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma69.pub.EDWARDS.00A,qt} & \htuse{CLEO.Gamma69.pub.EDWARDS.00A,exp} & \htuse{CLEO.Gamma69.pub.EDWARDS.00A,ref}
}%
\htdef{Gamma70.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma70.gn} = \htuse{Gamma70.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma70.qt} & average &}%
\htdef{Gamma74.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma74.gn} = \htuse{Gamma74.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma74.qt} & average & \\
\htuse{DELPHI.Gamma74.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma74.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma74.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma75.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma75.gn} = \htuse{Gamma75.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma75.qt} & average &}%
\htdef{Gamma76.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma76.gn} = \htuse{Gamma76.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma76.qt} & average & \\
\htuse{ALEPH.Gamma76.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma76.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma76.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma76by54.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma76by54.gn} = \htuse{Gamma76by54.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma76by54.qt} & average & \\
\htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93,qt} & \htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93,exp} & \htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93,ref}
}%
\htdef{Gamma77.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma77.gn} = \htuse{Gamma77.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma77.qt} & average &}%
\htdef{Gamma78.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma78.gn} = \htuse{Gamma78.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma78.qt} & average & \\
\htuse{CLEO.Gamma78.pub.ANASTASSOV.01,qt} & \htuse{CLEO.Gamma78.pub.ANASTASSOV.01,exp} & \htuse{CLEO.Gamma78.pub.ANASTASSOV.01,ref}
}%
\htdef{Gamma79.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma79.gn} = \htuse{Gamma79.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma79.qt} & average &}%
\htdef{Gamma80.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma80.gn} = \htuse{Gamma80.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma80.qt} & average &}%
\htdef{Gamma80by60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma80by60.gn} = \htuse{Gamma80by60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma80by60.qt} & average & \\
\htuse{CLEO.Gamma80by60.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma80by60.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma80by60.pub.RICHICHI.99,ref}
}%
\htdef{Gamma81.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma81.gn} = \htuse{Gamma81.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma81.qt} & average &}%
\htdef{Gamma81by69.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma81by69.gn} = \htuse{Gamma81by69.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma81by69.qt} & average & \\
\htuse{CLEO.Gamma81by69.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma81by69.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma81by69.pub.RICHICHI.99,ref}
}%
\htdef{Gamma82.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma82.gn} = \htuse{Gamma82.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma82.qt} & average & \\
\htuse{TPC.Gamma82.pub.BAUER.94,qt} & \htuse{TPC.Gamma82.pub.BAUER.94,exp} & \htuse{TPC.Gamma82.pub.BAUER.94,ref}
}%
\htdef{Gamma83.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma83.gn} = \htuse{Gamma83.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma83.qt} & average &}%
\htdef{Gamma84.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma84.gn} = \htuse{Gamma84.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma84.qt} & average &}%
\htdef{Gamma85.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma85.qt} & average & \\
\htuse{ALEPH.Gamma85.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma85.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma85.pub.BARATE.98,ref} \\
\htuse{BaBar.Gamma85.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma85.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma85.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma85.pub.LEE.10,qt} & \htuse{Belle.Gamma85.pub.LEE.10,exp} & \htuse{Belle.Gamma85.pub.LEE.10,ref} \\
\htuse{CLEO3.Gamma85.pub.BRIERE.03,qt} & \htuse{CLEO3.Gamma85.pub.BRIERE.03,exp} & \htuse{CLEO3.Gamma85.pub.BRIERE.03,ref} \\
\htuse{OPAL.Gamma85.pub.ABBIENDI.04J,qt} & \htuse{OPAL.Gamma85.pub.ABBIENDI.04J,exp} & \htuse{OPAL.Gamma85.pub.ABBIENDI.04J,ref}
}%
\htdef{Gamma85by60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma85by60.gn} = \htuse{Gamma85by60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma85by60.qt} & average &}%
\htdef{Gamma87.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma87.gn} = \htuse{Gamma87.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma87.qt} & average &}%
\htdef{Gamma88.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma88.gn} = \htuse{Gamma88.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma88.qt} & average & \\
\htuse{ALEPH.Gamma88.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma88.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma88.pub.BARATE.98,ref} \\
\htuse{CLEO3.Gamma88.pub.ARMS.05,qt} & \htuse{CLEO3.Gamma88.pub.ARMS.05,exp} & \htuse{CLEO3.Gamma88.pub.ARMS.05,ref}
}%
\htdef{Gamma89.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma89.gn} = \htuse{Gamma89.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma89.qt} & average &}%
\htdef{Gamma92.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma92.gn} = \htuse{Gamma92.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma92.qt} & average & \\
\htuse{OPAL.Gamma92.pub.ABBIENDI.00D,qt} & \htuse{OPAL.Gamma92.pub.ABBIENDI.00D,exp} & \htuse{OPAL.Gamma92.pub.ABBIENDI.00D,ref} \\
\htuse{TPC.Gamma92.pub.BAUER.94,qt} & \htuse{TPC.Gamma92.pub.BAUER.94,exp} & \htuse{TPC.Gamma92.pub.BAUER.94,ref}
}%
\htdef{Gamma93.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma93.qt} & average & \\
\htuse{ALEPH.Gamma93.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma93.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma93.pub.BARATE.98,ref} \\
\htuse{BaBar.Gamma93.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma93.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma93.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma93.pub.LEE.10,qt} & \htuse{Belle.Gamma93.pub.LEE.10,exp} & \htuse{Belle.Gamma93.pub.LEE.10,ref} \\
\htuse{CLEO3.Gamma93.pub.BRIERE.03,qt} & \htuse{CLEO3.Gamma93.pub.BRIERE.03,exp} & \htuse{CLEO3.Gamma93.pub.BRIERE.03,ref}
}%
\htdef{Gamma93by60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma93by60.gn} = \htuse{Gamma93by60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma93by60.qt} & average & \\
\htuse{CLEO.Gamma93by60.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma93by60.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma93by60.pub.RICHICHI.99,ref}
}%
\htdef{Gamma94.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma94.gn} = \htuse{Gamma94.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma94.qt} & average & \\
\htuse{ALEPH.Gamma94.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma94.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma94.pub.BARATE.98,ref} \\
\htuse{CLEO3.Gamma94.pub.ARMS.05,qt} & \htuse{CLEO3.Gamma94.pub.ARMS.05,exp} & \htuse{CLEO3.Gamma94.pub.ARMS.05,ref}
}%
\htdef{Gamma94by69.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma94by69.gn} = \htuse{Gamma94by69.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma94by69.qt} & average & \\
\htuse{CLEO.Gamma94by69.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma94by69.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma94by69.pub.RICHICHI.99,ref}
}%
\htdef{Gamma96.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma96.gn} = \htuse{Gamma96.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma96.qt} & average & \\
\htuse{BaBar.Gamma96.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma96.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma96.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma96.pub.LEE.10,qt} & \htuse{Belle.Gamma96.pub.LEE.10,exp} & \htuse{Belle.Gamma96.pub.LEE.10,ref}
}%
\htdef{Gamma102.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma102.qt} & average & \\
\htuse{CLEO.Gamma102.pub.GIBAUT.94B,qt} & \htuse{CLEO.Gamma102.pub.GIBAUT.94B,exp} & \htuse{CLEO.Gamma102.pub.GIBAUT.94B,ref} \\
\htuse{HRS.Gamma102.pub.BYLSMA.87,qt} & \htuse{HRS.Gamma102.pub.BYLSMA.87,exp} & \htuse{HRS.Gamma102.pub.BYLSMA.87,ref} \\
\htuse{L3.Gamma102.pub.ACHARD.01D,qt} & \htuse{L3.Gamma102.pub.ACHARD.01D,exp} & \htuse{L3.Gamma102.pub.ACHARD.01D,ref}
}%
\htdef{Gamma103.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma103.qt} & average & \\
\htuse{ALEPH.Gamma103.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma103.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma103.pub.SCHAEL.05C,ref} \\
\htuse{ARGUS.Gamma103.pub.ALBRECHT.88B,qt} & \htuse{ARGUS.Gamma103.pub.ALBRECHT.88B,exp} & \htuse{ARGUS.Gamma103.pub.ALBRECHT.88B,ref} \\
\htuse{CLEO.Gamma103.pub.GIBAUT.94B,qt} & \htuse{CLEO.Gamma103.pub.GIBAUT.94B,exp} & \htuse{CLEO.Gamma103.pub.GIBAUT.94B,ref} \\
\htuse{DELPHI.Gamma103.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma103.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma103.pub.ABDALLAH.06A,ref} \\
\htuse{HRS.Gamma103.pub.BYLSMA.87,qt} & \htuse{HRS.Gamma103.pub.BYLSMA.87,exp} & \htuse{HRS.Gamma103.pub.BYLSMA.87,ref} \\
\htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E,qt} & \htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E,exp} & \htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E,ref}
}%
\htdef{Gamma104.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma104.qt} & average & \\
\htuse{ALEPH.Gamma104.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma104.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma104.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma104.pub.ANASTASSOV.01,qt} & \htuse{CLEO.Gamma104.pub.ANASTASSOV.01,exp} & \htuse{CLEO.Gamma104.pub.ANASTASSOV.01,ref} \\
\htuse{DELPHI.Gamma104.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma104.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma104.pub.ABDALLAH.06A,ref} \\
\htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E,qt} & \htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E,exp} & \htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E,ref}
}%
\htdef{Gamma106.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma106.gn} = \htuse{Gamma106.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma106.qt} & average &}%
\htdef{Gamma110.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma110.gn} = \htuse{Gamma110.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma110.qt} & average &}%
\htdef{Gamma126.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma126.qt} & average & \\
\htuse{ALEPH.Gamma126.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma126.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma126.pub.BUSKULIC.97C,ref} \\
\htuse{Belle.Gamma126.pub.INAMI.09,qt} & \htuse{Belle.Gamma126.pub.INAMI.09,exp} & \htuse{Belle.Gamma126.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma126.pub.ARTUSO.92,qt} & \htuse{CLEO.Gamma126.pub.ARTUSO.92,exp} & \htuse{CLEO.Gamma126.pub.ARTUSO.92,ref}
}%
\htdef{Gamma128.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma128.qt} & average & \\
\htuse{ALEPH.Gamma128.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma128.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma128.pub.BUSKULIC.97C,ref} \\
\htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,qt} & \htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,exp} & \htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,ref} \\
\htuse{Belle.Gamma128.pub.INAMI.09,qt} & \htuse{Belle.Gamma128.pub.INAMI.09,exp} & \htuse{Belle.Gamma128.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma128.pub.BARTELT.96,qt} & \htuse{CLEO.Gamma128.pub.BARTELT.96,exp} & \htuse{CLEO.Gamma128.pub.BARTELT.96,ref}
}%
\htdef{Gamma130.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma130.gn} = \htuse{Gamma130.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma130.qt} & average & \\
\htuse{Belle.Gamma130.pub.INAMI.09,qt} & \htuse{Belle.Gamma130.pub.INAMI.09,exp} & \htuse{Belle.Gamma130.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma130.pub.BISHAI.99,qt} & \htuse{CLEO.Gamma130.pub.BISHAI.99,exp} & \htuse{CLEO.Gamma130.pub.BISHAI.99,ref}
}%
\htdef{Gamma132.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma132.gn} = \htuse{Gamma132.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma132.qt} & average & \\
\htuse{Belle.Gamma132.pub.INAMI.09,qt} & \htuse{Belle.Gamma132.pub.INAMI.09,exp} & \htuse{Belle.Gamma132.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma132.pub.BISHAI.99,qt} & \htuse{CLEO.Gamma132.pub.BISHAI.99,exp} & \htuse{CLEO.Gamma132.pub.BISHAI.99,ref}
}%
\htdef{Gamma136.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma136.gn} = \htuse{Gamma136.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma136.qt} & average &}%
\htdef{Gamma149.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma149.gn} = \htuse{Gamma149.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma149.qt} & average &}%
\htdef{Gamma150.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma150.gn} = \htuse{Gamma150.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma150.qt} & average & \\
\htuse{ALEPH.Gamma150.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma150.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma150.pub.BUSKULIC.97C,ref} \\
\htuse{CLEO.Gamma150.pub.BARINGER.87,qt} & \htuse{CLEO.Gamma150.pub.BARINGER.87,exp} & \htuse{CLEO.Gamma150.pub.BARINGER.87,ref}
}%
\htdef{Gamma150by66.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma150by66.gn} = \htuse{Gamma150by66.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma150by66.qt} & average & \\
\htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96,qt} & \htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96,exp} & \htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96,ref} \\
\htuse{CLEO.Gamma150by66.pub.BALEST.95C,qt} & \htuse{CLEO.Gamma150by66.pub.BALEST.95C,exp} & \htuse{CLEO.Gamma150by66.pub.BALEST.95C,ref}
}%
\htdef{Gamma151.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma151.gn} = \htuse{Gamma151.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma151.qt} & average & \\
\htuse{CLEO3.Gamma151.pub.ARMS.05,qt} & \htuse{CLEO3.Gamma151.pub.ARMS.05,exp} & \htuse{CLEO3.Gamma151.pub.ARMS.05,ref}
}%
\htdef{Gamma152.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma152.gn} = \htuse{Gamma152.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma152.qt} & average & \\
\htuse{ALEPH.Gamma152.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma152.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma152.pub.BUSKULIC.97C,ref}
}%
\htdef{Gamma152by54.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma152by54.gn} = \htuse{Gamma152by54.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma152by54.qt} & average &}%
\htdef{Gamma152by76.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma152by76.gn} = \htuse{Gamma152by76.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma152by76.qt} & average & \\
\htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93,qt} & \htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93,exp} & \htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93,ref}
}%
\htdef{Gamma167.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma167.gn} = \htuse{Gamma167.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma167.qt} & average &}%
\htdef{Gamma168.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma168.gn} = \htuse{Gamma168.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma168.qt} & average &}%
\htdef{Gamma169.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma169.gn} = \htuse{Gamma169.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma169.qt} & average &}%
\htdef{Gamma800.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma800.gn} = \htuse{Gamma800.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma800.qt} & average &}%
\htdef{Gamma802.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma802.gn} = \htuse{Gamma802.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma802.qt} & average &}%
\htdef{Gamma803.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma803.gn} = \htuse{Gamma803.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma803.qt} & average &}%
\htdef{Gamma804.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma804.gn} = \htuse{Gamma804.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma804.qt} & average &}%
\htdef{Gamma805.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma805.gn} = \htuse{Gamma805.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma805.qt} & average & \\
\htuse{ALEPH.Gamma805.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma805.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma805.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma806.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma806.gn} = \htuse{Gamma806.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma806.qt} & average &}%
\htdef{Gamma810.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma810.gn} = \htuse{Gamma810.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma810.qt} & average &}%
\htdef{Gamma811.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma811.gn} = \htuse{Gamma811.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma811.qt} & average & \\
\htuse{BaBar.Gamma811.pub.LEES.12X,qt} & \htuse{BaBar.Gamma811.pub.LEES.12X,exp} & \htuse{BaBar.Gamma811.pub.LEES.12X,ref}
}%
\htdef{Gamma812.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma812.gn} = \htuse{Gamma812.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma812.qt} & average & \\
\htuse{BaBar.Gamma812.pub.LEES.12X,qt} & \htuse{BaBar.Gamma812.pub.LEES.12X,exp} & \htuse{BaBar.Gamma812.pub.LEES.12X,ref}
}%
\htdef{Gamma820.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma820.gn} = \htuse{Gamma820.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma820.qt} & average &}%
\htdef{Gamma821.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma821.gn} = \htuse{Gamma821.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma821.qt} & average & \\
\htuse{BaBar.Gamma821.pub.LEES.12X,qt} & \htuse{BaBar.Gamma821.pub.LEES.12X,exp} & \htuse{BaBar.Gamma821.pub.LEES.12X,ref}
}%
\htdef{Gamma822.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma822.gn} = \htuse{Gamma822.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma822.qt} & average & \\
\htuse{BaBar.Gamma822.pub.LEES.12X,qt} & \htuse{BaBar.Gamma822.pub.LEES.12X,exp} & \htuse{BaBar.Gamma822.pub.LEES.12X,ref}
}%
\htdef{Gamma830.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma830.gn} = \htuse{Gamma830.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma830.qt} & average &}%
\htdef{Gamma831.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma831.gn} = \htuse{Gamma831.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma831.qt} & average & \\
\htuse{BaBar.Gamma831.pub.LEES.12X,qt} & \htuse{BaBar.Gamma831.pub.LEES.12X,exp} & \htuse{BaBar.Gamma831.pub.LEES.12X,ref}
}%
\htdef{Gamma832.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma832.gn} = \htuse{Gamma832.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma832.qt} & average & \\
\htuse{BaBar.Gamma832.pub.LEES.12X,qt} & \htuse{BaBar.Gamma832.pub.LEES.12X,exp} & \htuse{BaBar.Gamma832.pub.LEES.12X,ref}
}%
\htdef{Gamma833.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma833.gn} = \htuse{Gamma833.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma833.qt} & average & \\
\htuse{BaBar.Gamma833.pub.LEES.12X,qt} & \htuse{BaBar.Gamma833.pub.LEES.12X,exp} & \htuse{BaBar.Gamma833.pub.LEES.12X,ref}
}%
\htdef{Gamma910.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma910.gn} = \htuse{Gamma910.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma910.qt} & average & \\
\htuse{BaBar.Gamma910.pub.LEES.12X,qt} & \htuse{BaBar.Gamma910.pub.LEES.12X,exp} & \htuse{BaBar.Gamma910.pub.LEES.12X,ref}
}%
\htdef{Gamma911.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma911.gn} = \htuse{Gamma911.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma911.qt} & average & \\
\htuse{BaBar.Gamma911.pub.LEES.12X,qt} & \htuse{BaBar.Gamma911.pub.LEES.12X,exp} & \htuse{BaBar.Gamma911.pub.LEES.12X,ref}
}%
\htdef{Gamma920.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma920.gn} = \htuse{Gamma920.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma920.qt} & average & \\
\htuse{BaBar.Gamma920.pub.LEES.12X,qt} & \htuse{BaBar.Gamma920.pub.LEES.12X,exp} & \htuse{BaBar.Gamma920.pub.LEES.12X,ref}
}%
\htdef{Gamma930.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma930.gn} = \htuse{Gamma930.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma930.qt} & average & \\
\htuse{BaBar.Gamma930.pub.LEES.12X,qt} & \htuse{BaBar.Gamma930.pub.LEES.12X,exp} & \htuse{BaBar.Gamma930.pub.LEES.12X,ref}
}%
\htdef{Gamma944.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma944.gn} = \htuse{Gamma944.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma944.qt} & average & \\
\htuse{BaBar.Gamma944.pub.LEES.12X,qt} & \htuse{BaBar.Gamma944.pub.LEES.12X,exp} & \htuse{BaBar.Gamma944.pub.LEES.12X,ref}
}%
\htdef{Gamma945.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma945.gn} = \htuse{Gamma945.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma945.qt} & average &}%
\htdef{Gamma998.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma998.gn} = \htuse{Gamma998.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma998.qt} & average &}%
\htdef{BrVal}{%
\htuse{Gamma1.qm} \\
\midrule
\htuse{Gamma2.qm} \\
\midrule
\htuse{Gamma3.qm} \\
\midrule
\htuse{Gamma3by5.qm} \\
\midrule
\htuse{Gamma5.qm} \\
\midrule
\htuse{Gamma7.qm} \\
\midrule
\htuse{Gamma8.qm} \\
\midrule
\htuse{Gamma8by5.qm} \\
\midrule
\htuse{Gamma9.qm} \\
\midrule
\htuse{Gamma9by5.qm} \\
\midrule
\htuse{Gamma10.qm} \\
\midrule
\htuse{Gamma10by5.qm} \\
\midrule
\htuse{Gamma10by9.qm} \\
\midrule
\htuse{Gamma11.qm} \\
\midrule
\htuse{Gamma12.qm} \\
\midrule
\htuse{Gamma13.qm} \\
\midrule
\htuse{Gamma14.qm} \\
\midrule
\htuse{Gamma16.qm} \\
\midrule
\htuse{Gamma17.qm} \\
\midrule
\htuse{Gamma18.qm} \\
\midrule
\htuse{Gamma19.qm} \\
\midrule
\htuse{Gamma19by13.qm} \\
\midrule
\htuse{Gamma20.qm} \\
\midrule
\htuse{Gamma23.qm} \\
\midrule
\htuse{Gamma24.qm} \\
\midrule
\htuse{Gamma25.qm} \\
\midrule
\htuse{Gamma26.qm} \\
\midrule
\htuse{Gamma26by13.qm} \\
\midrule
\htuse{Gamma27.qm} \\
\midrule
\htuse{Gamma28.qm} \\
\midrule
\htuse{Gamma29.qm} \\
\midrule
\htuse{Gamma30.qm} \\
\midrule
\htuse{Gamma31.qm} \\
\midrule
\htuse{Gamma32.qm} \\
\midrule
\htuse{Gamma33.qm} \\
\midrule
\htuse{Gamma34.qm} \\
\midrule
\htuse{Gamma35.qm} \\
\midrule
\htuse{Gamma37.qm} \\
\midrule
\htuse{Gamma38.qm} \\
\midrule
\htuse{Gamma39.qm} \\
\midrule
\htuse{Gamma40.qm} \\
\midrule
\htuse{Gamma42.qm} \\
\midrule
\htuse{Gamma43.qm} \\
\midrule
\htuse{Gamma44.qm} \\
\midrule
\htuse{Gamma46.qm} \\
\midrule
\htuse{Gamma47.qm} \\
\midrule
\htuse{Gamma48.qm} \\
\midrule
\htuse{Gamma49.qm} \\
\midrule
\htuse{Gamma50.qm} \\
\midrule
\htuse{Gamma51.qm} \\
\midrule
\htuse{Gamma53.qm} \\
\midrule
\htuse{Gamma54.qm} \\
\midrule
\htuse{Gamma55.qm} \\
\midrule
\htuse{Gamma56.qm} \\
\midrule
\htuse{Gamma57.qm} \\
\midrule
\htuse{Gamma57by55.qm} \\
\midrule
\htuse{Gamma58.qm} \\
\midrule
\htuse{Gamma59.qm} \\
\midrule
\htuse{Gamma60.qm} \\
\midrule
\htuse{Gamma62.qm} \\
\midrule
\htuse{Gamma63.qm} \\
\midrule
\htuse{Gamma64.qm} \\
\midrule
\htuse{Gamma65.qm} \\
\midrule
\htuse{Gamma66.qm} \\
\midrule
\htuse{Gamma67.qm} \\
\midrule
\htuse{Gamma68.qm} \\
\midrule
\htuse{Gamma69.qm} \\
\midrule
\htuse{Gamma70.qm} \\
\midrule
\htuse{Gamma74.qm} \\
\midrule
\htuse{Gamma75.qm} \\
\midrule
\htuse{Gamma76.qm} \\
\midrule
\htuse{Gamma76by54.qm} \\
\midrule
\htuse{Gamma77.qm} \\
\midrule
\htuse{Gamma78.qm} \\
\midrule
\htuse{Gamma79.qm} \\
\midrule
\htuse{Gamma80.qm} \\
\midrule
\htuse{Gamma80by60.qm} \\
\midrule
\htuse{Gamma81.qm} \\
\midrule
\htuse{Gamma81by69.qm} \\
\midrule
\htuse{Gamma82.qm} \\
\midrule
\htuse{Gamma83.qm} \\
\midrule
\htuse{Gamma84.qm} \\
\midrule
\htuse{Gamma85.qm} \\
\midrule
\htuse{Gamma85by60.qm} \\
\midrule
\htuse{Gamma87.qm} \\
\midrule
\htuse{Gamma88.qm} \\
\midrule
\htuse{Gamma89.qm} \\
\midrule
\htuse{Gamma92.qm} \\
\midrule
\htuse{Gamma93.qm} \\
\midrule
\htuse{Gamma93by60.qm} \\
\midrule
\htuse{Gamma94.qm} \\
\midrule
\htuse{Gamma94by69.qm} \\
\midrule
\htuse{Gamma96.qm} \\
\midrule
\htuse{Gamma102.qm} \\
\midrule
\htuse{Gamma103.qm} \\
\midrule
\htuse{Gamma104.qm} \\
\midrule
\htuse{Gamma106.qm} \\
\midrule
\htuse{Gamma110.qm} \\
\midrule
\htuse{Gamma126.qm} \\
\midrule
\htuse{Gamma128.qm} \\
\midrule
\htuse{Gamma130.qm} \\
\midrule
\htuse{Gamma132.qm} \\
\midrule
\htuse{Gamma136.qm} \\
\midrule
\htuse{Gamma149.qm} \\
\midrule
\htuse{Gamma150.qm} \\
\midrule
\htuse{Gamma150by66.qm} \\
\midrule
\htuse{Gamma151.qm} \\
\midrule
\htuse{Gamma152.qm} \\
\midrule
\htuse{Gamma152by54.qm} \\
\midrule
\htuse{Gamma152by76.qm} \\
\midrule
\htuse{Gamma167.qm} \\
\midrule
\htuse{Gamma168.qm} \\
\midrule
\htuse{Gamma169.qm} \\
\midrule
\htuse{Gamma800.qm} \\
\midrule
\htuse{Gamma802.qm} \\
\midrule
\htuse{Gamma803.qm} \\
\midrule
\htuse{Gamma804.qm} \\
\midrule
\htuse{Gamma805.qm} \\
\midrule
\htuse{Gamma806.qm} \\
\midrule
\htuse{Gamma810.qm} \\
\midrule
\htuse{Gamma811.qm} \\
\midrule
\htuse{Gamma812.qm} \\
\midrule
\htuse{Gamma820.qm} \\
\midrule
\htuse{Gamma821.qm} \\
\midrule
\htuse{Gamma822.qm} \\
\midrule
\htuse{Gamma830.qm} \\
\midrule
\htuse{Gamma831.qm} \\
\midrule
\htuse{Gamma832.qm} \\
\midrule
\htuse{Gamma833.qm} \\
\midrule
\htuse{Gamma910.qm} \\
\midrule
\htuse{Gamma911.qm} \\
\midrule
\htuse{Gamma920.qm} \\
\midrule
\htuse{Gamma930.qm} \\
\midrule
\htuse{Gamma944.qm} \\
\midrule
\htuse{Gamma945.qm} \\
\midrule
\htuse{Gamma998.qm}}%
\htdef{BARATE 98.cite}{\cite{Barate:1997ma}}%
\htdef{BARATE 98.collab}{ALEPH}%
\htdef{BARATE 98.ref}{BARATE 98 (ALEPH) \cite{Barate:1997ma}}%
\htdef{BARATE 98.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma85.pub.BARATE.98}
\\
\begin{ensuredisplaymath}
\htuse{Gamma88.gn} = \htuse{Gamma88.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma88.pub.BARATE.98}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma93.pub.BARATE.98}
\\
\begin{ensuredisplaymath}
\htuse{Gamma94.gn} = \htuse{Gamma94.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma94.pub.BARATE.98}}%
\htdef{BARATE 98E.cite}{\cite{Barate:1997tt}}%
\htdef{BARATE 98E.collab}{ALEPH}%
\htdef{BARATE 98E.ref}{BARATE 98E (ALEPH) \cite{Barate:1997tt}}%
\htdef{BARATE 98E.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma33.gn} = \htuse{Gamma33.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma33.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma37.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma40.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma42.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma47.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma48.gn} = \htuse{Gamma48.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma48.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma51.gn} = \htuse{Gamma51.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma51.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma53.gn} = \htuse{Gamma53.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma53.pub.BARATE.98E}}%
\htdef{BARATE 99K.cite}{\cite{Barate:1999hi}}%
\htdef{BARATE 99K.collab}{ALEPH}%
\htdef{BARATE 99K.ref}{BARATE 99K (ALEPH) \cite{Barate:1999hi}}%
\htdef{BARATE 99K.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma10.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma16.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma23.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma28.gn} = \htuse{Gamma28.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma28.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma35.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma37.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma40.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma42.pub.BARATE.99K}}%
\htdef{BARATE 99R.cite}{\cite{Barate:1999hj}}%
\htdef{BARATE 99R.collab}{ALEPH}%
\htdef{BARATE 99R.ref}{BARATE 99R (ALEPH) \cite{Barate:1999hj}}%
\htdef{BARATE 99R.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma44.gn} = \htuse{Gamma44.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma44.pub.BARATE.99R}}%
\htdef{BUSKULIC 96.cite}{\cite{Buskulic:1995ty}}%
\htdef{BUSKULIC 96.collab}{ALEPH}%
\htdef{BUSKULIC 96.ref}{BUSKULIC 96 (ALEPH) \cite{Buskulic:1995ty}}%
\htdef{BUSKULIC 96.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma150by66.gn} = \htuse{Gamma150by66.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96}}%
\htdef{BUSKULIC 97C.cite}{\cite{Buskulic:1996qs}}%
\htdef{BUSKULIC 97C.collab}{ALEPH}%
\htdef{BUSKULIC 97C.ref}{BUSKULIC 97C (ALEPH) \cite{Buskulic:1996qs}}%
\htdef{BUSKULIC 97C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma126.pub.BUSKULIC.97C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma128.pub.BUSKULIC.97C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma150.gn} = \htuse{Gamma150.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma150.pub.BUSKULIC.97C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma152.gn} = \htuse{Gamma152.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma152.pub.BUSKULIC.97C}}%
\htdef{SCHAEL 05C.cite}{\cite{Schael:2005am}}%
\htdef{SCHAEL 05C.collab}{ALEPH}%
\htdef{SCHAEL 05C.ref}{SCHAEL 05C (ALEPH) \cite{Schael:2005am}}%
\htdef{SCHAEL 05C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma3.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma5.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma9.gn} = \htuse{Gamma9.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma9.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma14.gn} = \htuse{Gamma14.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma14.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma20.gn} = \htuse{Gamma20.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma20.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma27.gn} = \htuse{Gamma27.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma27.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma30.gn} = \htuse{Gamma30.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma30.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma62.gn} = \htuse{Gamma62.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma62.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma69.gn} = \htuse{Gamma69.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma69.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma76.gn} = \htuse{Gamma76.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma76.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma103.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma104.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma805.gn} = \htuse{Gamma805.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma805.pub.SCHAEL.05C}}%
\htdef{ALBRECHT 88B.cite}{\cite{Albrecht:1987zf}}%
\htdef{ALBRECHT 88B.collab}{ARGUS}%
\htdef{ALBRECHT 88B.ref}{ALBRECHT 88B (ARGUS) \cite{Albrecht:1987zf}}%
\htdef{ALBRECHT 88B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{ARGUS.Gamma103.pub.ALBRECHT.88B}}%
\htdef{ALBRECHT 92D.cite}{\cite{Albrecht:1991rh}}%
\htdef{ALBRECHT 92D.collab}{ARGUS}%
\htdef{ALBRECHT 92D.ref}{ALBRECHT 92D (ARGUS) \cite{Albrecht:1991rh}}%
\htdef{ALBRECHT 92D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & \htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D}}%
\htdef{AUBERT 07AP.cite}{\cite{Aubert:2007jh}}%
\htdef{AUBERT 07AP.collab}{\babar}%
\htdef{AUBERT 07AP.ref}{AUBERT 07AP (\babar) \cite{Aubert:2007jh}}%
\htdef{AUBERT 07AP.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma16.pub.AUBERT.07AP}}%
\htdef{AUBERT 08.cite}{\cite{Aubert:2007mh}}%
\htdef{AUBERT 08.collab}{\babar}%
\htdef{AUBERT 08.ref}{AUBERT 08 (\babar) \cite{Aubert:2007mh}}%
\htdef{AUBERT 08.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma60.pub.AUBERT.08}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma85.pub.AUBERT.08}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma93.pub.AUBERT.08}
\\
\begin{ensuredisplaymath}
\htuse{Gamma96.gn} = \htuse{Gamma96.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma96.pub.AUBERT.08}}%
\htdef{AUBERT 10F.cite}{\cite{Aubert:2009qj}}%
\htdef{AUBERT 10F.collab}{\babar}%
\htdef{AUBERT 10F.ref}{AUBERT 10F (\babar) \cite{Aubert:2009qj}}%
\htdef{AUBERT 10F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma3by5.pub.AUBERT.10F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma9by5.gn} = \htuse{Gamma9by5.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma9by5.pub.AUBERT.10F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma10by5.gn} = \htuse{Gamma10by5.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma10by5.pub.AUBERT.10F}}%
\htdef{DEL-AMO-SANCHEZ 11E.cite}{\cite{delAmoSanchez:2010pc}}%
\htdef{DEL-AMO-SANCHEZ 11E.collab}{\babar}%
\htdef{DEL-AMO-SANCHEZ 11E.ref}{DEL-AMO-SANCHEZ 11E (\babar) \cite{delAmoSanchez:2010pc}}%
\htdef{DEL-AMO-SANCHEZ 11E.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E}}%
\htdef{LEES 12X.cite}{\cite{Lees:2012ks}}%
\htdef{LEES 12X.collab}{\babar}%
\htdef{LEES 12X.ref}{LEES 12X (\babar) \cite{Lees:2012ks}}%
\htdef{LEES 12X.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma811.gn} = \htuse{Gamma811.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma811.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma812.gn} = \htuse{Gamma812.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma812.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma821.gn} = \htuse{Gamma821.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma821.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma822.gn} = \htuse{Gamma822.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma822.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma831.gn} = \htuse{Gamma831.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma831.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma832.gn} = \htuse{Gamma832.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma832.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma833.gn} = \htuse{Gamma833.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma833.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma910.gn} = \htuse{Gamma910.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma910.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma911.gn} = \htuse{Gamma911.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma911.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma920.gn} = \htuse{Gamma920.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma920.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma930.gn} = \htuse{Gamma930.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma930.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma944.gn} = \htuse{Gamma944.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma944.pub.LEES.12X}}%
\htdef{LEES 12Y.cite}{\cite{Lees:2012de}}%
\htdef{LEES 12Y.collab}{\babar}%
\htdef{LEES 12Y.ref}{LEES 12Y (\babar) \cite{Lees:2012de}}%
\htdef{LEES 12Y.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma47.pub.LEES.12Y}
\\
\begin{ensuredisplaymath}
\htuse{Gamma50.gn} = \htuse{Gamma50.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma50.pub.LEES.12Y}}%
\htdef{LEES 18B.cite}{\cite{BaBar:2018qry}}%
\htdef{LEES 18B.collab}{\babar}%
\htdef{LEES 18B.ref}{LEES 18B (\babar) \cite{BaBar:2018qry}}%
\htdef{LEES 18B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma37.pub.LEES.18B}}%
\htdef{FUJIKAWA 08.cite}{\cite{Fujikawa:2008ma}}%
\htdef{FUJIKAWA 08.collab}{Belle}%
\htdef{FUJIKAWA 08.ref}{FUJIKAWA 08 (Belle) \cite{Fujikawa:2008ma}}%
\htdef{FUJIKAWA 08.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma13.pub.FUJIKAWA.08}}%
\htdef{INAMI 09.cite}{\cite{Inami:2008ar}}%
\htdef{INAMI 09.collab}{Belle}%
\htdef{INAMI 09.ref}{INAMI 09 (Belle) \cite{Inami:2008ar}}%
\htdef{INAMI 09.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma126.pub.INAMI.09}
\\
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma128.pub.INAMI.09}
\\
\begin{ensuredisplaymath}
\htuse{Gamma130.gn} = \htuse{Gamma130.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma130.pub.INAMI.09}
\\
\begin{ensuredisplaymath}
\htuse{Gamma132.gn} = \htuse{Gamma132.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma132.pub.INAMI.09}}%
\htdef{LEE 10.cite}{\cite{Lee:2010tc}}%
\htdef{LEE 10.collab}{Belle}%
\htdef{LEE 10.ref}{LEE 10 (Belle) \cite{Lee:2010tc}}%
\htdef{LEE 10.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma60.pub.LEE.10}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma85.pub.LEE.10}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma93.pub.LEE.10}
\\
\begin{ensuredisplaymath}
\htuse{Gamma96.gn} = \htuse{Gamma96.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma96.pub.LEE.10}}%
\htdef{RYU 14vpc.cite}{\cite{Ryu:2014vpc}}%
\htdef{RYU 14vpc.collab}{Belle}%
\htdef{RYU 14vpc.ref}{RYU 14vpc (Belle) \cite{Ryu:2014vpc}}%
\htdef{RYU 14vpc.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma35.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma37.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma40.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma42.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma47.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma50.gn} = \htuse{Gamma50.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma50.pub.RYU.14vpc}}%
\htdef{BEHREND 89B.cite}{\cite{Behrend:1989wc}}%
\htdef{BEHREND 89B.collab}{CELLO}%
\htdef{BEHREND 89B.ref}{BEHREND 89B (CELLO) \cite{Behrend:1989wc}}%
\htdef{BEHREND 89B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & \htuse{CELLO.Gamma54.pub.BEHREND.89B}}%
\htdef{ANASTASSOV 01.cite}{\cite{Anastassov:2000xu}}%
\htdef{ANASTASSOV 01.collab}{CLEO}%
\htdef{ANASTASSOV 01.ref}{ANASTASSOV 01 (CLEO) \cite{Anastassov:2000xu}}%
\htdef{ANASTASSOV 01.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma78.gn} = \htuse{Gamma78.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma78.pub.ANASTASSOV.01}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma104.pub.ANASTASSOV.01}}%
\htdef{ANASTASSOV 97.cite}{\cite{Anastassov:1996tc}}%
\htdef{ANASTASSOV 97.collab}{CLEO}%
\htdef{ANASTASSOV 97.ref}{ANASTASSOV 97 (CLEO) \cite{Anastassov:1996tc}}%
\htdef{ANASTASSOV 97.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma5.pub.ANASTASSOV.97}
\\
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma8.pub.ANASTASSOV.97}}%
\htdef{ARTUSO 92.cite}{\cite{Artuso:1992qu}}%
\htdef{ARTUSO 92.collab}{CLEO}%
\htdef{ARTUSO 92.ref}{ARTUSO 92 (CLEO) \cite{Artuso:1992qu}}%
\htdef{ARTUSO 92.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma126.pub.ARTUSO.92}}%
\htdef{ARTUSO 94.cite}{\cite{Artuso:1994ii}}%
\htdef{ARTUSO 94.collab}{CLEO}%
\htdef{ARTUSO 94.ref}{ARTUSO 94 (CLEO) \cite{Artuso:1994ii}}%
\htdef{ARTUSO 94.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma13.pub.ARTUSO.94}}%
\htdef{BALEST 95C.cite}{\cite{Balest:1995kq}}%
\htdef{BALEST 95C.collab}{CLEO}%
\htdef{BALEST 95C.ref}{BALEST 95C (CLEO) \cite{Balest:1995kq}}%
\htdef{BALEST 95C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma57.gn} = \htuse{Gamma57.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma57.pub.BALEST.95C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma66.pub.BALEST.95C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma150by66.gn} = \htuse{Gamma150by66.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma150by66.pub.BALEST.95C}}%
\htdef{BARINGER 87.cite}{\cite{Baringer:1987tr}}%
\htdef{BARINGER 87.collab}{CLEO}%
\htdef{BARINGER 87.ref}{BARINGER 87 (CLEO) \cite{Baringer:1987tr}}%
\htdef{BARINGER 87.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma150.gn} = \htuse{Gamma150.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma150.pub.BARINGER.87}}%
\htdef{BARTELT 96.cite}{\cite{Bartelt:1996iv}}%
\htdef{BARTELT 96.collab}{CLEO}%
\htdef{BARTELT 96.ref}{BARTELT 96 (CLEO) \cite{Bartelt:1996iv}}%
\htdef{BARTELT 96.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma128.pub.BARTELT.96}}%
\htdef{BATTLE 94.cite}{\cite{Battle:1994by}}%
\htdef{BATTLE 94.collab}{CLEO}%
\htdef{BATTLE 94.ref}{BATTLE 94 (CLEO) \cite{Battle:1994by}}%
\htdef{BATTLE 94.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma10.pub.BATTLE.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma16.pub.BATTLE.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma23.pub.BATTLE.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma31.pub.BATTLE.94}}%
\htdef{BISHAI 99.cite}{\cite{Bishai:1998gf}}%
\htdef{BISHAI 99.collab}{CLEO}%
\htdef{BISHAI 99.ref}{BISHAI 99 (CLEO) \cite{Bishai:1998gf}}%
\htdef{BISHAI 99.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma130.gn} = \htuse{Gamma130.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma130.pub.BISHAI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma132.gn} = \htuse{Gamma132.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma132.pub.BISHAI.99}}%
\htdef{BORTOLETTO 93.cite}{\cite{Bortoletto:1993px}}%
\htdef{BORTOLETTO 93.collab}{CLEO}%
\htdef{BORTOLETTO 93.ref}{BORTOLETTO 93 (CLEO) \cite{Bortoletto:1993px}}%
\htdef{BORTOLETTO 93.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma76by54.gn} = \htuse{Gamma76by54.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93}
\\
\begin{ensuredisplaymath}
\htuse{Gamma152by76.gn} = \htuse{Gamma152by76.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93}}%
\htdef{COAN 96.cite}{\cite{Coan:1996iu}}%
\htdef{COAN 96.collab}{CLEO}%
\htdef{COAN 96.ref}{COAN 96 (CLEO) \cite{Coan:1996iu}}%
\htdef{COAN 96.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma34.gn} = \htuse{Gamma34.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma34.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma37.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma39.gn} = \htuse{Gamma39.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma39.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma42.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma47.pub.COAN.96}}%
\htdef{EDWARDS 00A.cite}{\cite{Edwards:1999fj}}%
\htdef{EDWARDS 00A.collab}{CLEO}%
\htdef{EDWARDS 00A.ref}{EDWARDS 00A (CLEO) \cite{Edwards:1999fj}}%
\htdef{EDWARDS 00A.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma69.gn} = \htuse{Gamma69.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma69.pub.EDWARDS.00A}}%
\htdef{GIBAUT 94B.cite}{\cite{Gibaut:1994ik}}%
\htdef{GIBAUT 94B.collab}{CLEO}%
\htdef{GIBAUT 94B.ref}{GIBAUT 94B (CLEO) \cite{Gibaut:1994ik}}%
\htdef{GIBAUT 94B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma102.pub.GIBAUT.94B}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma103.pub.GIBAUT.94B}}%
\htdef{PROCARIO 93.cite}{\cite{Procario:1992hd}}%
\htdef{PROCARIO 93.collab}{CLEO}%
\htdef{PROCARIO 93.ref}{PROCARIO 93 (CLEO) \cite{Procario:1992hd}}%
\htdef{PROCARIO 93.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma19by13.gn} = \htuse{Gamma19by13.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma19by13.pub.PROCARIO.93}
\\
\begin{ensuredisplaymath}
\htuse{Gamma26by13.gn} = \htuse{Gamma26by13.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma26by13.pub.PROCARIO.93}
\\
\begin{ensuredisplaymath}
\htuse{Gamma29.gn} = \htuse{Gamma29.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma29.pub.PROCARIO.93}}%
\htdef{RICHICHI 99.cite}{\cite{Richichi:1998bc}}%
\htdef{RICHICHI 99.collab}{CLEO}%
\htdef{RICHICHI 99.ref}{RICHICHI 99 (CLEO) \cite{Richichi:1998bc}}%
\htdef{RICHICHI 99.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma80by60.gn} = \htuse{Gamma80by60.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma80by60.pub.RICHICHI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma81by69.gn} = \htuse{Gamma81by69.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma81by69.pub.RICHICHI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93by60.gn} = \htuse{Gamma93by60.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma93by60.pub.RICHICHI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma94by69.gn} = \htuse{Gamma94by69.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma94by69.pub.RICHICHI.99}}%
\htdef{ARMS 05.cite}{\cite{Arms:2005qg}}%
\htdef{ARMS 05.collab}{CLEO3}%
\htdef{ARMS 05.ref}{ARMS 05 (CLEO3) \cite{Arms:2005qg}}%
\htdef{ARMS 05.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma88.gn} = \htuse{Gamma88.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma88.pub.ARMS.05}
\\
\begin{ensuredisplaymath}
\htuse{Gamma94.gn} = \htuse{Gamma94.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma94.pub.ARMS.05}
\\
\begin{ensuredisplaymath}
\htuse{Gamma151.gn} = \htuse{Gamma151.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma151.pub.ARMS.05}}%
\htdef{BRIERE 03.cite}{\cite{Briere:2003fr}}%
\htdef{BRIERE 03.collab}{CLEO3}%
\htdef{BRIERE 03.ref}{BRIERE 03 (CLEO3) \cite{Briere:2003fr}}%
\htdef{BRIERE 03.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma60.pub.BRIERE.03}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma85.pub.BRIERE.03}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma93.pub.BRIERE.03}}%
\htdef{ABDALLAH 06A.cite}{\cite{Abdallah:2003cw}}%
\htdef{ABDALLAH 06A.collab}{DELPHI}%
\htdef{ABDALLAH 06A.ref}{ABDALLAH 06A (DELPHI) \cite{Abdallah:2003cw}}%
\htdef{ABDALLAH 06A.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma8.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma13.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma19.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma25.gn} = \htuse{Gamma25.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma25.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma57.gn} = \htuse{Gamma57.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma57.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma66.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma74.gn} = \htuse{Gamma74.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma74.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma103.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma104.pub.ABDALLAH.06A}}%
\htdef{ABREU 92N.cite}{\cite{Abreu:1992gn}}%
\htdef{ABREU 92N.collab}{DELPHI}%
\htdef{ABREU 92N.ref}{ABREU 92N (DELPHI) \cite{Abreu:1992gn}}%
\htdef{ABREU 92N.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma7.pub.ABREU.92N}}%
\htdef{ABREU 94K.cite}{\cite{Abreu:1994fi}}%
\htdef{ABREU 94K.collab}{DELPHI}%
\htdef{ABREU 94K.ref}{ABREU 94K (DELPHI) \cite{Abreu:1994fi}}%
\htdef{ABREU 94K.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma10.pub.ABREU.94K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma31.pub.ABREU.94K}}%
\htdef{ABREU 99X.cite}{\cite{Abreu:1999rb}}%
\htdef{ABREU 99X.collab}{DELPHI}%
\htdef{ABREU 99X.ref}{ABREU 99X (DELPHI) \cite{Abreu:1999rb}}%
\htdef{ABREU 99X.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma3.pub.ABREU.99X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma5.pub.ABREU.99X}}%
\htdef{BYLSMA 87.cite}{\cite{Bylsma:1986zy}}%
\htdef{BYLSMA 87.collab}{HRS}%
\htdef{BYLSMA 87.ref}{BYLSMA 87 (HRS) \cite{Bylsma:1986zy}}%
\htdef{BYLSMA 87.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & \htuse{HRS.Gamma102.pub.BYLSMA.87}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{HRS.Gamma103.pub.BYLSMA.87}}%
\htdef{ACCIARRI 01F.cite}{\cite{Acciarri:2001sg}}%
\htdef{ACCIARRI 01F.collab}{L3}%
\htdef{ACCIARRI 01F.ref}{ACCIARRI 01F (L3) \cite{Acciarri:2001sg}}%
\htdef{ACCIARRI 01F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma3.pub.ACCIARRI.01F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma5.pub.ACCIARRI.01F}}%
\htdef{ACCIARRI 95.cite}{\cite{Acciarri:1994vr}}%
\htdef{ACCIARRI 95.collab}{L3}%
\htdef{ACCIARRI 95.ref}{ACCIARRI 95 (L3) \cite{Acciarri:1994vr}}%
\htdef{ACCIARRI 95.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma7.pub.ACCIARRI.95}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma13.pub.ACCIARRI.95}
\\
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma19.pub.ACCIARRI.95}
\\
\begin{ensuredisplaymath}
\htuse{Gamma26.gn} = \htuse{Gamma26.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma26.pub.ACCIARRI.95}}%
\htdef{ACCIARRI 95F.cite}{\cite{Acciarri:1995kx}}%
\htdef{ACCIARRI 95F.collab}{L3}%
\htdef{ACCIARRI 95F.ref}{ACCIARRI 95F (L3) \cite{Acciarri:1995kx}}%
\htdef{ACCIARRI 95F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma35.pub.ACCIARRI.95F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma40.pub.ACCIARRI.95F}}%
\htdef{ACHARD 01D.cite}{\cite{Achard:2001pk}}%
\htdef{ACHARD 01D.collab}{L3}%
\htdef{ACHARD 01D.ref}{ACHARD 01D (L3) \cite{Achard:2001pk}}%
\htdef{ACHARD 01D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma55.gn} = \htuse{Gamma55.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma55.pub.ACHARD.01D}
\\
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma102.pub.ACHARD.01D}}%
\htdef{ADEVA 91F.cite}{\cite{Adeva:1991qq}}%
\htdef{ADEVA 91F.collab}{L3}%
\htdef{ADEVA 91F.ref}{ADEVA 91F (L3) \cite{Adeva:1991qq}}%
\htdef{ADEVA 91F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma54.pub.ADEVA.91F}}%
\htdef{ABBIENDI 00C.cite}{\cite{Abbiendi:1999pm}}%
\htdef{ABBIENDI 00C.collab}{OPAL}%
\htdef{ABBIENDI 00C.ref}{ABBIENDI 00C (OPAL) \cite{Abbiendi:1999pm}}%
\htdef{ABBIENDI 00C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma35.pub.ABBIENDI.00C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma38.gn} = \htuse{Gamma38.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma38.pub.ABBIENDI.00C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma43.gn} = \htuse{Gamma43.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma43.pub.ABBIENDI.00C}}%
\htdef{ABBIENDI 00D.cite}{\cite{Abbiendi:1999cq}}%
\htdef{ABBIENDI 00D.collab}{OPAL}%
\htdef{ABBIENDI 00D.ref}{ABBIENDI 00D (OPAL) \cite{Abbiendi:1999cq}}%
\htdef{ABBIENDI 00D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma92.gn} = \htuse{Gamma92.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma92.pub.ABBIENDI.00D}}%
\htdef{ABBIENDI 01J.cite}{\cite{Abbiendi:2000ee}}%
\htdef{ABBIENDI 01J.collab}{OPAL}%
\htdef{ABBIENDI 01J.ref}{ABBIENDI 01J (OPAL) \cite{Abbiendi:2000ee}}%
\htdef{ABBIENDI 01J.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma10.pub.ABBIENDI.01J}
\\
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma31.pub.ABBIENDI.01J}}%
\htdef{ABBIENDI 03.cite}{\cite{Abbiendi:2002jw}}%
\htdef{ABBIENDI 03.collab}{OPAL}%
\htdef{ABBIENDI 03.ref}{ABBIENDI 03 (OPAL) \cite{Abbiendi:2002jw}}%
\htdef{ABBIENDI 03.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma3.pub.ABBIENDI.03}}%
\htdef{ABBIENDI 04J.cite}{\cite{Abbiendi:2004xa}}%
\htdef{ABBIENDI 04J.collab}{OPAL}%
\htdef{ABBIENDI 04J.ref}{ABBIENDI 04J (OPAL) \cite{Abbiendi:2004xa}}%
\htdef{ABBIENDI 04J.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma16.pub.ABBIENDI.04J}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma85.pub.ABBIENDI.04J}}%
\htdef{ABBIENDI 99H.cite}{\cite{Abbiendi:1998cx}}%
\htdef{ABBIENDI 99H.collab}{OPAL}%
\htdef{ABBIENDI 99H.ref}{ABBIENDI 99H (OPAL) \cite{Abbiendi:1998cx}}%
\htdef{ABBIENDI 99H.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma5.pub.ABBIENDI.99H}}%
\htdef{ACKERSTAFF 98M.cite}{\cite{Ackerstaff:1997tx}}%
\htdef{ACKERSTAFF 98M.collab}{OPAL}%
\htdef{ACKERSTAFF 98M.ref}{ACKERSTAFF 98M (OPAL) \cite{Ackerstaff:1997tx}}%
\htdef{ACKERSTAFF 98M.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M}
\\
\begin{ensuredisplaymath}
\htuse{Gamma17.gn} = \htuse{Gamma17.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M}}%
\htdef{ACKERSTAFF 99E.cite}{\cite{Ackerstaff:1998ia}}%
\htdef{ACKERSTAFF 99E.collab}{OPAL}%
\htdef{ACKERSTAFF 99E.ref}{ACKERSTAFF 99E (OPAL) \cite{Ackerstaff:1998ia}}%
\htdef{ACKERSTAFF 99E.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E}}%
\htdef{AKERS 94G.cite}{\cite{Akers:1994td}}%
\htdef{AKERS 94G.collab}{OPAL}%
\htdef{AKERS 94G.ref}{AKERS 94G (OPAL) \cite{Akers:1994td}}%
\htdef{AKERS 94G.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma33.gn} = \htuse{Gamma33.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma33.pub.AKERS.94G}}%
\htdef{AKERS 95Y.cite}{\cite{Akers:1995ry}}%
\htdef{AKERS 95Y.collab}{OPAL}%
\htdef{AKERS 95Y.ref}{AKERS 95Y (OPAL) \cite{Akers:1995ry}}%
\htdef{AKERS 95Y.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma55.gn} = \htuse{Gamma55.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma55.pub.AKERS.95Y}
\\
\begin{ensuredisplaymath}
\htuse{Gamma57by55.gn} = \htuse{Gamma57by55.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma57by55.pub.AKERS.95Y}}%
\htdef{ALEXANDER 91D.cite}{\cite{Alexander:1991am}}%
\htdef{ALEXANDER 91D.collab}{OPAL}%
\htdef{ALEXANDER 91D.ref}{ALEXANDER 91D (OPAL) \cite{Alexander:1991am}}%
\htdef{ALEXANDER 91D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma7.pub.ALEXANDER.91D}}%
\htdef{AIHARA 87B.cite}{\cite{Aihara:1986mw}}%
\htdef{AIHARA 87B.collab}{TPC}%
\htdef{AIHARA 87B.ref}{AIHARA 87B (TPC) \cite{Aihara:1986mw}}%
\htdef{AIHARA 87B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & \htuse{TPC.Gamma54.pub.AIHARA.87B}}%
\htdef{BAUER 94.cite}{\cite{Bauer:1993wn}}%
\htdef{BAUER 94.collab}{TPC}%
\htdef{BAUER 94.ref}{BAUER 94 (TPC) \cite{Bauer:1993wn}}%
\htdef{BAUER 94.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma82.gn} = \htuse{Gamma82.td}
\end{ensuredisplaymath} & \htuse{TPC.Gamma82.pub.BAUER.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma92.gn} = \htuse{Gamma92.td}
\end{ensuredisplaymath} & \htuse{TPC.Gamma92.pub.BAUER.94}}%
\htdef{MeasPaper}{%
\multicolumn{2}{l}{\htuse{BARATE 98.ref}} \\
\htuse{BARATE 98.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARATE 98E.ref}} \\
\htuse{BARATE 98E.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARATE 99K.ref}} \\
\htuse{BARATE 99K.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARATE 99R.ref}} \\
\htuse{BARATE 99R.meas} \\\hline
\multicolumn{2}{l}{\htuse{BUSKULIC 96.ref}} \\
\htuse{BUSKULIC 96.meas} \\\hline
\multicolumn{2}{l}{\htuse{BUSKULIC 97C.ref}} \\
\htuse{BUSKULIC 97C.meas} \\\hline
\multicolumn{2}{l}{\htuse{SCHAEL 05C.ref}} \\
\htuse{SCHAEL 05C.meas} \\\hline
\multicolumn{2}{l}{\htuse{ALBRECHT 88B.ref}} \\
\htuse{ALBRECHT 88B.meas} \\\hline
\multicolumn{2}{l}{\htuse{ALBRECHT 92D.ref}} \\
\htuse{ALBRECHT 92D.meas} \\\hline
\multicolumn{2}{l}{\htuse{AUBERT 07AP.ref}} \\
\htuse{AUBERT 07AP.meas} \\\hline
\multicolumn{2}{l}{\htuse{AUBERT 08.ref}} \\
\htuse{AUBERT 08.meas} \\\hline
\multicolumn{2}{l}{\htuse{AUBERT 10F.ref}} \\
\htuse{AUBERT 10F.meas} \\\hline
\multicolumn{2}{l}{\htuse{DEL-AMO-SANCHEZ 11E.ref}} \\
\htuse{DEL-AMO-SANCHEZ 11E.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEES 12X.ref}} \\
\htuse{LEES 12X.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEES 12Y.ref}} \\
\htuse{LEES 12Y.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEES 18B.ref}} \\
\htuse{LEES 18B.meas} \\\hline
\multicolumn{2}{l}{\htuse{FUJIKAWA 08.ref}} \\
\htuse{FUJIKAWA 08.meas} \\\hline
\multicolumn{2}{l}{\htuse{INAMI 09.ref}} \\
\htuse{INAMI 09.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEE 10.ref}} \\
\htuse{LEE 10.meas} \\\hline
\multicolumn{2}{l}{\htuse{RYU 14vpc.ref}} \\
\htuse{RYU 14vpc.meas} \\\hline
\multicolumn{2}{l}{\htuse{BEHREND 89B.ref}} \\
\htuse{BEHREND 89B.meas} \\\hline
\multicolumn{2}{l}{\htuse{ANASTASSOV 01.ref}} \\
\htuse{ANASTASSOV 01.meas} \\\hline
\multicolumn{2}{l}{\htuse{ANASTASSOV 97.ref}} \\
\htuse{ANASTASSOV 97.meas} \\\hline
\multicolumn{2}{l}{\htuse{ARTUSO 92.ref}} \\
\htuse{ARTUSO 92.meas} \\\hline
\multicolumn{2}{l}{\htuse{ARTUSO 94.ref}} \\
\htuse{ARTUSO 94.meas} \\\hline
\multicolumn{2}{l}{\htuse{BALEST 95C.ref}} \\
\htuse{BALEST 95C.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARINGER 87.ref}} \\
\htuse{BARINGER 87.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARTELT 96.ref}} \\
\htuse{BARTELT 96.meas} \\\hline
\multicolumn{2}{l}{\htuse{BATTLE 94.ref}} \\
\htuse{BATTLE 94.meas} \\\hline
\multicolumn{2}{l}{\htuse{BISHAI 99.ref}} \\
\htuse{BISHAI 99.meas} \\\hline
\multicolumn{2}{l}{\htuse{BORTOLETTO 93.ref}} \\
\htuse{BORTOLETTO 93.meas} \\\hline
\multicolumn{2}{l}{\htuse{COAN 96.ref}} \\
\htuse{COAN 96.meas} \\\hline
\multicolumn{2}{l}{\htuse{EDWARDS 00A.ref}} \\
\htuse{EDWARDS 00A.meas} \\\hline
\multicolumn{2}{l}{\htuse{GIBAUT 94B.ref}} \\
\htuse{GIBAUT 94B.meas} \\\hline
\multicolumn{2}{l}{\htuse{PROCARIO 93.ref}} \\
\htuse{PROCARIO 93.meas} \\\hline
\multicolumn{2}{l}{\htuse{RICHICHI 99.ref}} \\
\htuse{RICHICHI 99.meas} \\\hline
\multicolumn{2}{l}{\htuse{ARMS 05.ref}} \\
\htuse{ARMS 05.meas} \\\hline
\multicolumn{2}{l}{\htuse{BRIERE 03.ref}} \\
\htuse{BRIERE 03.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABDALLAH 06A.ref}} \\
\htuse{ABDALLAH 06A.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABREU 92N.ref}} \\
\htuse{ABREU 92N.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABREU 94K.ref}} \\
\htuse{ABREU 94K.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABREU 99X.ref}} \\
\htuse{ABREU 99X.meas} \\\hline
\multicolumn{2}{l}{\htuse{BYLSMA 87.ref}} \\
\htuse{BYLSMA 87.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACCIARRI 01F.ref}} \\
\htuse{ACCIARRI 01F.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACCIARRI 95.ref}} \\
\htuse{ACCIARRI 95.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACCIARRI 95F.ref}} \\
\htuse{ACCIARRI 95F.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACHARD 01D.ref}} \\
\htuse{ACHARD 01D.meas} \\\hline
\multicolumn{2}{l}{\htuse{ADEVA 91F.ref}} \\
\htuse{ADEVA 91F.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 00C.ref}} \\
\htuse{ABBIENDI 00C.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 00D.ref}} \\
\htuse{ABBIENDI 00D.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 01J.ref}} \\
\htuse{ABBIENDI 01J.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 03.ref}} \\
\htuse{ABBIENDI 03.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 04J.ref}} \\
\htuse{ABBIENDI 04J.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 99H.ref}} \\
\htuse{ABBIENDI 99H.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACKERSTAFF 98M.ref}} \\
\htuse{ACKERSTAFF 98M.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACKERSTAFF 99E.ref}} \\
\htuse{ACKERSTAFF 99E.meas} \\\hline
\multicolumn{2}{l}{\htuse{AKERS 94G.ref}} \\
\htuse{AKERS 94G.meas} \\\hline
\multicolumn{2}{l}{\htuse{AKERS 95Y.ref}} \\
\htuse{AKERS 95Y.meas} \\\hline
\multicolumn{2}{l}{\htuse{ALEXANDER 91D.ref}} \\
\htuse{ALEXANDER 91D.meas} \\\hline
\multicolumn{2}{l}{\htuse{AIHARA 87B.ref}} \\
\htuse{AIHARA 87B.meas} \\\hline
\multicolumn{2}{l}{\htuse{BAUER 94.ref}} \\
\htuse{BAUER 94.meas}}%
\htdef{BrStrangeVal}{%
\htQuantLine{Gamma10}{0.6957 \pm 0.0096}{-2} 
\htQuantLine{Gamma16}{0.4322 \pm 0.0148}{-2} 
\htQuantLine{Gamma23}{0.0634 \pm 0.0219}{-2} 
\htQuantLine{Gamma28}{0.0465 \pm 0.0213}{-2} 
\htQuantLine{Gamma35}{0.8375 \pm 0.0139}{-2} 
\htQuantLine{Gamma40}{0.3810 \pm 0.0129}{-2} 
\htQuantLine{Gamma44}{0.0234 \pm 0.0231}{-2} 
\htQuantLine{Gamma53}{0.0222 \pm 0.0202}{-2} 
\htQuantLine{Gamma128}{0.0155 \pm 0.0008}{-2} 
\htQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\htQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\htQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\htQuantLine{Gamma168}{0.0022 \pm 0.0008}{-2} 
\htQuantLine{Gamma169}{0.0015 \pm 0.0006}{-2} 
\htQuantLine{Gamma802}{0.2924 \pm 0.0068}{-2} 
\htQuantLine{Gamma803}{0.0387 \pm 0.0142}{-2} 
\htQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\htQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2}}%
\htdef{BrStrangeTotVal}{%
\htQuantLine{Gamma110}{2.9076 \pm 0.0478}{-2}}%
\htdef{UnitarityQuants}{%
\htConstrLine{Gamma3}{17.3875 \pm 0.0396}{1.0000}{-2}{0} 
\htConstrLine{Gamma5}{17.8111 \pm 0.0410}{1.0000}{-2}{0} 
\htConstrLine{Gamma9}{10.8082 \pm 0.0527}{1.0000}{-2}{0} 
\htConstrLine{Gamma10}{0.6957 \pm 0.0096}{1.0000}{-2}{0} 
\htConstrLine{Gamma14}{25.4857 \pm 0.0902}{1.0000}{-2}{0} 
\htConstrLine{Gamma16}{0.4322 \pm 0.0148}{1.0000}{-2}{0} 
\htConstrLine{Gamma20}{9.2454 \pm 0.0988}{1.0000}{-2}{0} 
\htConstrLine{Gamma23}{0.0634 \pm 0.0219}{1.0000}{-2}{0} 
\htConstrLine{Gamma27}{1.0401 \pm 0.0708}{1.0000}{-2}{0} 
\htConstrLine{Gamma28}{0.0465 \pm 0.0213}{1.0000}{-2}{0} 
\htConstrLine{Gamma30}{0.1118 \pm 0.0391}{1.0000}{-2}{0} 
\htConstrLine{Gamma35}{0.8375 \pm 0.0139}{1.0000}{-2}{0} 
\htConstrLine{Gamma37}{0.1486 \pm 0.0034}{1.0000}{-2}{0} 
\htConstrLine{Gamma40}{0.3810 \pm 0.0129}{1.0000}{-2}{0} 
\htConstrLine{Gamma42}{0.1499 \pm 0.0070}{1.0000}{-2}{0} 
\htConstrLine{Gamma44}{0.0234 \pm 0.0231}{1.0000}{-2}{0} 
\htConstrLine{Gamma47}{0.0235 \pm 0.0006}{2.0000}{-2}{0} 
\htConstrLine{Gamma48}{0.1048 \pm 0.0247}{1.0000}{-2}{0} 
\htConstrLine{Gamma50}{0.0018 \pm 0.0002}{2.0000}{-2}{0} 
\htConstrLine{Gamma51}{0.0318 \pm 0.0119}{1.0000}{-2}{0} 
\htConstrLine{Gamma53}{0.0222 \pm 0.0202}{1.0000}{-2}{0} 
\htConstrLine{Gamma62}{8.9807 \pm 0.0521}{1.0000}{-2}{0} 
\htConstrLine{Gamma70}{2.7427 \pm 0.0714}{1.0000}{-2}{0} 
\htConstrLine{Gamma77}{0.0979 \pm 0.0356}{1.0000}{-2}{0} 
\htConstrLine{Gamma93}{0.1434 \pm 0.0027}{1.0000}{-2}{0} 
\htConstrLine{Gamma94}{0.0061 \pm 0.0018}{1.0000}{-2}{0} 
\htConstrLine{Gamma126}{0.1386 \pm 0.0072}{1.0000}{-2}{0} 
\htConstrLine{Gamma128}{0.0155 \pm 0.0008}{1.0000}{-2}{0} 
\htConstrLine{Gamma130}{0.0048 \pm 0.0012}{1.0000}{-2}{0} 
\htConstrLine{Gamma132}{0.0094 \pm 0.0015}{1.0000}{-2}{0} 
\htConstrLine{Gamma136}{0.0220 \pm 0.0013}{1.0000}{-2}{0} 
\htConstrLine{Gamma151}{0.0410 \pm 0.0092}{1.0000}{-2}{0} 
\htConstrLine{Gamma152}{0.4069 \pm 0.0419}{1.0000}{-2}{0} 
\htConstrLine{Gamma167}{0.0044 \pm 0.0016}{0.8320}{-2}{0} 
\htConstrLine{Gamma800}{1.9474 \pm 0.0646}{1.0000}{-2}{0} 
\htConstrLine{Gamma802}{0.2924 \pm 0.0068}{1.0000}{-2}{0} 
\htConstrLine{Gamma803}{0.0387 \pm 0.0142}{1.0000}{-2}{0} 
\htConstrLine{Gamma805}{0.0400 \pm 0.0200}{1.0000}{-2}{0} 
\htConstrLine{Gamma811}{0.0072 \pm 0.0016}{1.0000}{-2}{0} 
\htConstrLine{Gamma812}{0.0014 \pm 0.0027}{1.0000}{-2}{0} 
\htConstrLine{Gamma821}{0.0774 \pm 0.0030}{1.0000}{-2}{0} 
\htConstrLine{Gamma822}{0.0001 \pm 0.0001}{1.0000}{-2}{0} 
\htConstrLine{Gamma831}{0.0084 \pm 0.0006}{1.0000}{-2}{0} 
\htConstrLine{Gamma832}{0.0038 \pm 0.0009}{1.0000}{-2}{0} 
\htConstrLine{Gamma833}{0.0001 \pm 0.0001}{1.0000}{-2}{0} 
\htConstrLine{Gamma920}{0.0052 \pm 0.0004}{1.0000}{-2}{0} 
\htConstrLine{Gamma945}{0.0194 \pm 0.0038}{1.0000}{-2}{0} 
\htConstrLine{Gamma998}{0.0684 \pm 0.1068}{1.0000}{-2}{0}}%
\htdef{BaseQuants}{%
\htQuantLine{Gamma3}{17.3875 \pm 0.0396}{-2} 
\htQuantLine{Gamma5}{17.8111 \pm 0.0410}{-2} 
\htQuantLine{Gamma9}{10.8082 \pm 0.0527}{-2} 
\htQuantLine{Gamma10}{0.6957 \pm 0.0096}{-2} 
\htQuantLine{Gamma14}{25.4857 \pm 0.0902}{-2} 
\htQuantLine{Gamma16}{0.4322 \pm 0.0148}{-2} 
\htQuantLine{Gamma20}{9.2454 \pm 0.0988}{-2} 
\htQuantLine{Gamma23}{0.0634 \pm 0.0219}{-2} 
\htQuantLine{Gamma27}{1.0401 \pm 0.0708}{-2} 
\htQuantLine{Gamma28}{0.0465 \pm 0.0213}{-2} 
\htQuantLine{Gamma30}{0.1118 \pm 0.0391}{-2} 
\htQuantLine{Gamma35}{0.8375 \pm 0.0139}{-2} 
\htQuantLine{Gamma37}{0.1486 \pm 0.0034}{-2} 
\htQuantLine{Gamma40}{0.3810 \pm 0.0129}{-2} 
\htQuantLine{Gamma42}{0.1499 \pm 0.0070}{-2} 
\htQuantLine{Gamma44}{0.0234 \pm 0.0231}{-2} 
\htQuantLine{Gamma47}{0.0235 \pm 0.0006}{-2} 
\htQuantLine{Gamma48}{0.1048 \pm 0.0247}{-2} 
\htQuantLine{Gamma50}{0.0018 \pm 0.0002}{-2} 
\htQuantLine{Gamma51}{0.0318 \pm 0.0119}{-2} 
\htQuantLine{Gamma53}{0.0222 \pm 0.0202}{-2} 
\htQuantLine{Gamma62}{8.9807 \pm 0.0521}{-2} 
\htQuantLine{Gamma70}{2.7427 \pm 0.0714}{-2} 
\htQuantLine{Gamma77}{0.0979 \pm 0.0356}{-2} 
\htQuantLine{Gamma93}{0.1434 \pm 0.0027}{-2} 
\htQuantLine{Gamma94}{0.0061 \pm 0.0018}{-2} 
\htQuantLine{Gamma126}{0.1386 \pm 0.0072}{-2} 
\htQuantLine{Gamma128}{0.0155 \pm 0.0008}{-2} 
\htQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\htQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\htQuantLine{Gamma136}{0.0220 \pm 0.0013}{-2} 
\htQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\htQuantLine{Gamma152}{0.4069 \pm 0.0419}{-2} 
\htQuantLine{Gamma167}{0.0044 \pm 0.0016}{-2} 
\htQuantLine{Gamma800}{1.9474 \pm 0.0646}{-2} 
\htQuantLine{Gamma802}{0.2924 \pm 0.0068}{-2} 
\htQuantLine{Gamma803}{0.0387 \pm 0.0142}{-2} 
\htQuantLine{Gamma805}{0.0400 \pm 0.0200}{-2} 
\htQuantLine{Gamma811}{0.0072 \pm 0.0016}{-2} 
\htQuantLine{Gamma812}{0.0014 \pm 0.0027}{-2} 
\htQuantLine{Gamma821}{0.0774 \pm 0.0030}{-2} 
\htQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\htQuantLine{Gamma831}{0.0084 \pm 0.0006}{-2} 
\htQuantLine{Gamma832}{0.0038 \pm 0.0009}{-2} 
\htQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2} 
\htQuantLine{Gamma920}{0.0052 \pm 0.0004}{-2} 
\htQuantLine{Gamma945}{0.0194 \pm 0.0038}{-2}}%
\htdef{BrCorr}{%
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 1.\label{tab:tau:br-fit-corr1}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 1.}\label{tab:tau:br-fit-corr1}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{5} \) &   23 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{9} \) &    8 &    5 &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{10} \) &    5 &    7 &    7 &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{14} \) &  -14 &  -15 &  -13 &   -3 &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{16} \) &    1 &    1 &    2 &   -1 &   -8 &  &  &  &  &  &  &  &  &  \\
\( \BR_{20} \) &   -5 &   -5 &   -8 &   -1 &  -41 &    1 &  &  &  &  &  &  &  &  \\
\( \BR_{23} \) &    2 &    2 &    0 &   -2 &    0 &  -13 &   -7 &  &  &  &  &  &  &  \\
\( \BR_{27} \) &   -5 &   -4 &   -8 &   -1 &    1 &    1 &  -36 &    1 &  &  &  &  &  &  \\
\( \BR_{28} \) &    2 &    2 &    1 &   -1 &    1 &  -13 &   -1 &  -22 &  -10 &  &  &  &  &  \\
\( \BR_{30} \) &   -4 &   -3 &  -10 &   -1 &   -8 &    0 &    6 &   -2 &  -44 &    2 &  &  &  &  \\
\( \BR_{35} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  \\
\( \BR_{37} \) &    0 &   -1 &    1 &    0 &    0 &    0 &    0 &   -2 &    0 &   -2 &    0 &  -15 &  &  \\
\( \BR_{40} \) &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    1 &   -1 &    1 &    0 &  -12 &    2 &  \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 2.\label{tab:tau:br-fit-corr2}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 2.}\label{tab:tau:br-fit-corr2}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{42} \) &    0 &    0 &    0 &    0 &    0 &   -3 &    1 &   -5 &    0 &   -5 &    0 &   -1 &  -14 &  -20 \\
\( \BR_{44} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -4 \\
\( \BR_{47} \) &    0 &   -1 &    2 &    0 &    0 &    2 &    0 &    0 &    0 &    0 &    0 &   -1 &    3 &   -4 \\
\( \BR_{48} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &    0 &   -2 \\
\( \BR_{50} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    5 &    0 \\
\( \BR_{51} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 \\
\( \BR_{53} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{62} \) &   -2 &   -4 &    8 &    0 &   -3 &    4 &   -7 &    0 &   -6 &    0 &   -5 &   -1 &    3 &    0 \\
\( \BR_{70} \) &   -6 &   -6 &   -7 &   -1 &  -10 &    0 &   -1 &    0 &   -1 &    0 &    3 &    0 &   -1 &    0 \\
\( \BR_{77} \) &   -1 &    0 &   -3 &    0 &   -2 &    0 &    0 &    0 &    2 &    0 &    2 &    0 &    0 &    0 \\
\( \BR_{93} \) &    0 &   -1 &    3 &    0 &   -1 &    2 &   -1 &    0 &   -1 &    0 &   -1 &    0 &    2 &    0 \\
\( \BR_{94} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{126} \) &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &   -2 &    0 &    0 &    0 \\
\( \BR_{128} \) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &   -1 &    0 &   -1 &    0 &    0 &    1 &    0 \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 3.\label{tab:tau:br-fit-corr3}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 3.}\label{tab:tau:br-fit-corr3}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{130} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{132} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{136} \) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\
\( \BR_{151} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{152} \) &   -1 &   -1 &   -3 &    0 &   -2 &    0 &   -1 &    0 &    2 &    0 &    2 &    0 &    0 &    0 \\
\( \BR_{167} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{800} \) &   -1 &   -1 &   -2 &    0 &   -3 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{802} \) &    1 &    0 &    1 &    0 &    0 &    0 &   -2 &    0 &   -1 &    0 &   -1 &    0 &    0 &    0 \\
\( \BR_{803} \) &    2 &    2 &    1 &    0 &    2 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 \\
\( \BR_{805} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{811} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{812} \) &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{821} \) &    0 &    0 &    2 &    0 &    0 &    1 &   -1 &    0 &   -1 &    0 &   -1 &    0 &    1 &    0 \\
\( \BR_{822} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 4.\label{tab:tau:br-fit-corr4}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 4.}\label{tab:tau:br-fit-corr4}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{831} \) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\
\( \BR_{832} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{833} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{920} \) &    0 &    0 &    1 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &   -1 &    0 &    1 &    0 \\
\( \BR_{945} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 5.\label{tab:tau:br-fit-corr5}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 5.}\label{tab:tau:br-fit-corr5}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{44} \) &    0 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{47} \) &    1 &    0 &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{48} \) &   -1 &   -6 &    0 &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{50} \) &    6 &    0 &   -7 &    0 &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{51} \) &    0 &   -3 &    0 &   -6 &    0 &  &  &  &  &  &  &  &  &  \\
\( \BR_{53} \) &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  &  &  &  &  &  \\
\( \BR_{62} \) &   -1 &    0 &    5 &    0 &    1 &    0 &    0 &  &  &  &  &  &  &  \\
\( \BR_{70} \) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &  -20 &  &  &  &  &  &  \\
\( \BR_{77} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -7 &  &  &  &  &  \\
\( \BR_{93} \) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &   16 &   -4 &    0 &  &  &  &  \\
\( \BR_{94} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &  &  &  \\
\( \BR_{126} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &   -5 &    0 &    0 &  &  \\
\( \BR_{128} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &    0 &    0 &    1 &    0 &    4 &  \\
 & \( \BR_{42} \) & \( \BR_{44} \) & \( \BR_{47} \) & \( \BR_{48} \) & \( \BR_{50} \) & \( \BR_{51} \) & \( \BR_{53} \) & \( \BR_{62} \) & \( \BR_{70} \) & \( \BR_{77} \) & \( \BR_{93} \) & \( \BR_{94} \) & \( \BR_{126} \) & \( \BR_{128} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 6.\label{tab:tau:br-fit-corr6}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 6.}\label{tab:tau:br-fit-corr6}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{130} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    1 \\
\( \BR_{132} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    1 \\
\( \BR_{136} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{151} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   12 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{152} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  -11 &  -64 &    0 &    0 &    0 &    0 \\
\( \BR_{167} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{800} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -8 &  -67 &   -3 &   -1 &    0 &    0 &    0 \\
\( \BR_{802} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   20 &   -7 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{803} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &  -14 &   -1 &   -1 &   -3 &    0 &   -1 \\
\( \BR_{805} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{811} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{812} \) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{821} \) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &    3 &   -1 &    0 &    1 &    0 &    0 &    1 \\
\( \BR_{822} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{42} \) & \( \BR_{44} \) & \( \BR_{47} \) & \( \BR_{48} \) & \( \BR_{50} \) & \( \BR_{51} \) & \( \BR_{53} \) & \( \BR_{62} \) & \( \BR_{70} \) & \( \BR_{77} \) & \( \BR_{93} \) & \( \BR_{94} \) & \( \BR_{126} \) & \( \BR_{128} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 7.\label{tab:tau:br-fit-corr7}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 7.}\label{tab:tau:br-fit-corr7}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{831} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{832} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{833} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{920} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{945} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{42} \) & \( \BR_{44} \) & \( \BR_{47} \) & \( \BR_{48} \) & \( \BR_{50} \) & \( \BR_{51} \) & \( \BR_{53} \) & \( \BR_{62} \) & \( \BR_{70} \) & \( \BR_{77} \) & \( \BR_{93} \) & \( \BR_{94} \) & \( \BR_{126} \) & \( \BR_{128} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 8.\label{tab:tau:br-fit-corr8}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 8.}\label{tab:tau:br-fit-corr8}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{132} \) &    0 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{136} \) &    0 &    0 &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{151} \) &    0 &    0 &    0 &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{152} \) &    0 &    0 &    0 &    0 &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{167} \) &    0 &    0 &    0 &    0 &    0 &  &  &  &  &  &  &  &  &  \\
\( \BR_{800} \) &    0 &    0 &    0 &  -14 &   -3 &    0 &  &  &  &  &  &  &  &  \\
\( \BR_{802} \) &    0 &    0 &    0 &   -2 &    0 &    1 &   -2 &  &  &  &  &  &  &  \\
\( \BR_{803} \) &    0 &    0 &    0 &  -58 &   -1 &    0 &   10 &    0 &  &  &  &  &  &  \\
\( \BR_{805} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  &  &  \\
\( \BR_{811} \) &    0 &   -1 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  &  \\
\( \BR_{812} \) &    0 &   -2 &   -8 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  -16 &  &  &  \\
\( \BR_{821} \) &    0 &    0 &   46 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    8 &   -4 &  &  \\
\( \BR_{822} \) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  \\
 & \( \BR_{130} \) & \( \BR_{132} \) & \( \BR_{136} \) & \( \BR_{151} \) & \( \BR_{152} \) & \( \BR_{167} \) & \( \BR_{800} \) & \( \BR_{802} \) & \( \BR_{803} \) & \( \BR_{805} \) & \( \BR_{811} \) & \( \BR_{812} \) & \( \BR_{821} \) & \( \BR_{822} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 9.\label{tab:tau:br-fit-corr9}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 9.}\label{tab:tau:br-fit-corr9}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{831} \) &    0 &    0 &   39 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   14 &   -4 &   39 &   -1 \\
\( \BR_{832} \) &    0 &    0 &    3 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    3 &    0 \\
\( \BR_{833} \) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 \\
\( \BR_{920} \) &    0 &    0 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    3 &   -2 &   34 &   -1 \\
\( \BR_{945} \) &    0 &   -1 &   25 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   10 &  -11 &   10 &    0 \\
 & \( \BR_{130} \) & \( \BR_{132} \) & \( \BR_{136} \) & \( \BR_{151} \) & \( \BR_{152} \) & \( \BR_{167} \) & \( \BR_{800} \) & \( \BR_{802} \) & \( \BR_{803} \) & \( \BR_{805} \) & \( \BR_{811} \) & \( \BR_{812} \) & \( \BR_{821} \) & \( \BR_{822} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 10.\label{tab:tau:br-fit-corr10}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 10.}\label{tab:tau:br-fit-corr10}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrr}
\hline
\( \BR_{832} \) &   -2 &  &  &  &  \\
\( \BR_{833} \) &   -1 &   -1 &  &  &  \\
\( \BR_{920} \) &   17 &    1 &    0 &  &  \\
\( \BR_{945} \) &   17 &    2 &    0 &    4 &  \\
 & \( \BR_{831} \) & \( \BR_{832} \) & \( \BR_{833} \) & \( \BR_{920} \) & \( \BR_{945} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi}%
\htconstrdef{Gamma1.c}{\BR_{1}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} + \BR_{40} + \BR_{44} + \BR_{37} + \BR_{42} + \BR_{47} + \BR_{48} + \BR_{804} + \BR_{50} + \BR_{51} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16}  \\ 
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}  \\ 
  {}& + \BR_{40} + \BR_{44} + \BR_{37} + \BR_{42} + \BR_{47} + \BR_{48}  \\ 
  {}& + \BR_{804} + \BR_{50} + \BR_{51} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma}  \\ 
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}%
\htconstrdef{Gamma2.c}{\BR_{2}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{40}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{44}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{37}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{42}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^0\pi^0} + \BR_{804} + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^0\pi^0} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}(\BR_{\eta\to\text{neutral}}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>})) + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16}  \\ 
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\ 
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{40}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{44}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\ 
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{37}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{42}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\ 
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^0\pi^0}  \\ 
  {}& + \BR_{804} + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^0\pi^0}  \\ 
  {}& + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{132}\cdot{}(\BR_{\eta\to\text{neutral}}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>})) + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}  \\ 
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma3by5.c}{\frac{\BR_{3}}{\BR_{5}}}{\frac{\BR_{3}}{\BR_{5}}}{\frac{\BR_{3}}{\BR_{5}}}%
\htconstrdef{Gamma7.c}{\BR_{7}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_L>} + \BR_{9} + \BR_{804} + \BR_{37}\cdot{}\BR_{<K^0|K_L>} + \BR_{10}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_L>} + \BR_{9} + \BR_{804} + \BR_{37}\cdot{}\BR_{<K^0|K_L>}  \\ 
  {}& + \BR_{10}}%
\htconstrdef{Gamma8.c}{\BR_{8}}{\BR_{9} + \BR_{10}}{\BR_{9} + \BR_{10}}%
\htconstrdef{Gamma8by5.c}{\frac{\BR_{8}}{\BR_{5}}}{\frac{\BR_{8}}{\BR_{5}}}{\frac{\BR_{8}}{\BR_{5}}}%
\htconstrdef{Gamma9by5.c}{\frac{\BR_{9}}{\BR_{5}}}{\frac{\BR_{9}}{\BR_{5}}}{\frac{\BR_{9}}{\BR_{5}}}%
\htconstrdef{Gamma10by5.c}{\frac{\BR_{10}}{\BR_{5}}}{\frac{\BR_{10}}{\BR_{5}}}{\frac{\BR_{10}}{\BR_{5}}}%
\htconstrdef{Gamma10by9.c}{\frac{\BR_{10}}{\BR_{9}}}{\frac{\BR_{10}}{\BR_{9}}}{\frac{\BR_{10}}{\BR_{9}}}%
\htconstrdef{Gamma11.c}{\BR_{11}}{\BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}}{\BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28}  \\ 
  {}& + \BR_{30} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma}  \\ 
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}}%
\htconstrdef{Gamma12.c}{\BR_{12}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{14}  \\ 
  {}& + \BR_{16} + \BR_{20} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma13.c}{\BR_{13}}{\BR_{14} + \BR_{16}}{\BR_{14} + \BR_{16}}%
\htconstrdef{Gamma17.c}{\BR_{17}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{27} + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{20} + \BR_{27} + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma18.c}{\BR_{18}}{\BR_{23} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{23} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma19.c}{\BR_{19}}{\BR_{23} + \BR_{20}}{\BR_{23} + \BR_{20}}%
\htconstrdef{Gamma19by13.c}{\frac{\BR_{19}}{\BR_{13}}}{\frac{\BR_{19}}{\BR_{13}}}{\frac{\BR_{19}}{\BR_{13}}}%
\htconstrdef{Gamma24.c}{\BR_{24}}{\BR_{27} + \BR_{28} + \BR_{30} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to3\pi^0})}{\BR_{27} + \BR_{28} + \BR_{30} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to3\pi^0}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to3\pi^0})}%
\htconstrdef{Gamma25.c}{\BR_{25}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{28} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{28} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma26.c}{\BR_{26}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{28} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{27}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{28} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{27}}%
\htconstrdef{Gamma26by13.c}{\frac{\BR_{26}}{\BR_{13}}}{\frac{\BR_{26}}{\BR_{13}}}{\frac{\BR_{26}}{\BR_{13}}}%
\htconstrdef{Gamma29.c}{\BR_{29}}{\BR_{30} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{30} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma31.c}{\BR_{31}}{\BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{23} + \BR_{28} + \BR_{42} + \BR_{16} + \BR_{37} + \BR_{10} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{23} + \BR_{28} + \BR_{42} + \BR_{16}  \\ 
  {}& + \BR_{37} + \BR_{10} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma32.c}{\BR_{32}}{\BR_{16} + \BR_{23} + \BR_{28} + \BR_{37} + \BR_{42} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{16} + \BR_{23} + \BR_{28} + \BR_{37} + \BR_{42} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma33.c}{\BR_{33}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{40}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{42}\cdot{}\BR_{<K^0|K_S>} + \BR_{47} + \BR_{48} + \BR_{50} + \BR_{51} + \BR_{37}\cdot{}\BR_{<K^0|K_S>} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{40}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{42}\cdot{}\BR_{<K^0|K_S>}  \\ 
  {}& + \BR_{47} + \BR_{48} + \BR_{50} + \BR_{51} + \BR_{37}\cdot{}\BR_{<K^0|K_S>}  \\ 
  {}& + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}%
\htconstrdef{Gamma34.c}{\BR_{34}}{\BR_{35} + \BR_{37}}{\BR_{35} + \BR_{37}}%
\htconstrdef{Gamma38.c}{\BR_{38}}{\BR_{42} + \BR_{37}}{\BR_{42} + \BR_{37}}%
\htconstrdef{Gamma39.c}{\BR_{39}}{\BR_{40} + \BR_{42}}{\BR_{40} + \BR_{42}}%
\htconstrdef{Gamma43.c}{\BR_{43}}{\BR_{40} + \BR_{44}}{\BR_{40} + \BR_{44}}%
\htconstrdef{Gamma46.c}{\BR_{46}}{\BR_{48} + \BR_{47} + \BR_{804}}{\BR_{48} + \BR_{47} + \BR_{804}}%
\htconstrdef{Gamma49.c}{\BR_{49}}{\BR_{50} + \BR_{51} + \BR_{806}}{\BR_{50} + \BR_{51} + \BR_{806}}%
\htconstrdef{Gamma54.c}{\BR_{54}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^+\pi^-} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^+\pi^-} + \BR_{53}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{93} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_L>}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-} + \BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^+\pi^-}  \\ 
  {}& + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^+\pi^-}  \\ 
  {}& + \BR_{53}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{62} + \BR_{70}  \\ 
  {}& + \BR_{77} + \BR_{78} + \BR_{93} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_L>}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})  \\ 
  {}& + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})  \\ 
  {}& + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-} + \BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803}  \\ 
  {}& + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}%
\htconstrdef{Gamma55.c}{\BR_{55}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{78} + \BR_{77} + \BR_{94} + \BR_{62} + \BR_{70} + \BR_{93} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{168}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{78}  \\ 
  {}& + \BR_{77} + \BR_{94} + \BR_{62} + \BR_{70} + \BR_{93} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}}  \\ 
  {}& + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{168}}%
\htconstrdef{Gamma56.c}{\BR_{56}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{93} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{168}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{93} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{168}}%
\htconstrdef{Gamma57.c}{\BR_{57}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}  \\ 
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma57by55.c}{\frac{\BR_{57}}{\BR_{55}}}{\frac{\BR_{57}}{\BR_{55}}}{\frac{\BR_{57}}{\BR_{55}}}%
\htconstrdef{Gamma58.c}{\BR_{58}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma59.c}{\BR_{59}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma60.c}{\BR_{60}}{\BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma63.c}{\BR_{63}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{charged}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{charged}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma64.c}{\BR_{64}}{\BR_{78} + \BR_{77} + \BR_{94} + \BR_{70} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{803}}{\BR_{78} + \BR_{77} + \BR_{94} + \BR_{70} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{803}}%
\htconstrdef{Gamma65.c}{\BR_{65}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma66.c}{\BR_{66}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma67.c}{\BR_{67}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma68.c}{\BR_{68}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-}  \\ 
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma69.c}{\BR_{69}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{70} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{70} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma74.c}{\BR_{74}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{78} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{78} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma75.c}{\BR_{75}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma76.c}{\BR_{76}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma76by54.c}{\frac{\BR_{76}}{\BR_{54}}}{\frac{\BR_{76}}{\BR_{54}}}{\frac{\BR_{76}}{\BR_{54}}}%
\htconstrdef{Gamma78.c}{\BR_{78}}{\BR_{810} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})}{\BR_{810} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})}%
\htconstrdef{Gamma79.c}{\BR_{79}}{\BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{93} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{168} + \BR_{802} + \BR_{803}}{\BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{93} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{168} + \BR_{802} + \BR_{803}}%
\htconstrdef{Gamma80.c}{\BR_{80}}{\BR_{93} + \BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{93} + \BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma80by60.c}{\frac{\BR_{80}}{\BR_{60}}}{\frac{\BR_{80}}{\BR_{60}}}{\frac{\BR_{80}}{\BR_{60}}}%
\htconstrdef{Gamma81.c}{\BR_{81}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{94} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{94} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma81by69.c}{\frac{\BR_{81}}{\BR_{69}}}{\frac{\BR_{81}}{\BR_{69}}}{\frac{\BR_{81}}{\BR_{69}}}%
\htconstrdef{Gamma82.c}{\BR_{82}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802}  \\ 
  {}& + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}%
\htconstrdef{Gamma83.c}{\BR_{83}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-})}%
\htconstrdef{Gamma84.c}{\BR_{84}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}%
\htconstrdef{Gamma85.c}{\BR_{85}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma85by60.c}{\frac{\BR_{85}}{\BR_{60}}}{\frac{\BR_{85}}{\BR_{60}}}{\frac{\BR_{85}}{\BR_{60}}}%
\htconstrdef{Gamma87.c}{\BR_{87}}{\BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{803}}%
\htconstrdef{Gamma88.c}{\BR_{88}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma89.c}{\BR_{89}}{\BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma92.c}{\BR_{92}}{\BR_{94} + \BR_{93}}{\BR_{94} + \BR_{93}}%
\htconstrdef{Gamma93by60.c}{\frac{\BR_{93}}{\BR_{60}}}{\frac{\BR_{93}}{\BR_{60}}}{\frac{\BR_{93}}{\BR_{60}}}%
\htconstrdef{Gamma94by69.c}{\frac{\BR_{94}}{\BR_{69}}}{\frac{\BR_{94}}{\BR_{69}}}{\frac{\BR_{94}}{\BR_{69}}}%
\htconstrdef{Gamma96.c}{\BR_{96}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma102.c}{\BR_{102}}{\BR_{103} + \BR_{104}}{\BR_{103} + \BR_{104}}%
\htconstrdef{Gamma103.c}{\BR_{103}}{\BR_{820} + \BR_{822} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{820} + \BR_{822} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma104.c}{\BR_{104}}{\BR_{830} + \BR_{833}}{\BR_{830} + \BR_{833}}%
\htconstrdef{Gamma106.c}{\BR_{106}}{\BR_{30} + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{47} + \BR_{53}\cdot{}\BR_{<K^0|K_S>} + \BR_{77} + \BR_{103} + \BR_{126}\cdot{}(\BR_{\eta\to3\pi^0}+\BR_{\eta\to\pi^+\pi^-\pi^0}) + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{30} + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{47} + \BR_{53}\cdot{}\BR_{<K^0|K_S>}  \\ 
  {}& + \BR_{77} + \BR_{103} + \BR_{126}\cdot{}(\BR_{\eta\to3\pi^0}+\BR_{\eta\to\pi^+\pi^-\pi^0}) + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma110.c}{\BR_{110}}{\BR_{10} + \BR_{16} + \BR_{23} + \BR_{28} + \BR_{35} + \BR_{40} + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{151} + \BR_{130} + \BR_{132} + \BR_{44} + \BR_{53} + \BR_{168} + \BR_{169} + \BR_{822} + \BR_{833}}{\BR_{10} + \BR_{16} + \BR_{23} + \BR_{28} + \BR_{35} + \BR_{40}  \\ 
  {}& + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{151} + \BR_{130} + \BR_{132}  \\ 
  {}& + \BR_{44} + \BR_{53} + \BR_{168} + \BR_{169} + \BR_{822} + \BR_{833}}%
\htconstrdef{Gamma149.c}{\BR_{149}}{\BR_{152} + \BR_{800} + \BR_{151}}{\BR_{152} + \BR_{800} + \BR_{151}}%
\htconstrdef{Gamma150.c}{\BR_{150}}{\BR_{800} + \BR_{151}}{\BR_{800} + \BR_{151}}%
\htconstrdef{Gamma150by66.c}{\frac{\BR_{150}}{\BR_{66}}}{\frac{\BR_{150}}{\BR_{66}}}{\frac{\BR_{150}}{\BR_{66}}}%
\htconstrdef{Gamma152by54.c}{\frac{\BR_{152}}{\BR_{54}}}{\frac{\BR_{152}}{\BR_{54}}}{\frac{\BR_{152}}{\BR_{54}}}%
\htconstrdef{Gamma152by76.c}{\frac{\BR_{152}}{\BR_{76}}}{\frac{\BR_{152}}{\BR_{76}}}{\frac{\BR_{152}}{\BR_{76}}}%
\htconstrdef{Gamma168.c}{\BR_{168}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma169.c}{\BR_{169}}{\BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}{\BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}%
\htconstrdef{Gamma804.c}{\BR_{804}}{\BR_{47} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}{\BR_{47} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}%
\htconstrdef{Gamma806.c}{\BR_{806}}{\BR_{50} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}{\BR_{50} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}%
\htconstrdef{Gamma810.c}{\BR_{810}}{\BR_{910} + \BR_{911} + \BR_{811}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{812}}{\BR_{910} + \BR_{911} + \BR_{811}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{812}}%
\htconstrdef{Gamma820.c}{\BR_{820}}{\BR_{920} + \BR_{821}}{\BR_{920} + \BR_{821}}%
\htconstrdef{Gamma830.c}{\BR_{830}}{\BR_{930} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{832}}{\BR_{930} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{832}}%
\htconstrdef{Gamma910.c}{\BR_{910}}{\BR_{136}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{136}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma911.c}{\BR_{911}}{\BR_{945}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{945}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma930.c}{\BR_{930}}{\BR_{136}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{136}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma944.c}{\BR_{944}}{\BR_{136}\cdot{}\BR_{\eta\to\gamma\gamma}}{\BR_{136}\cdot{}\BR_{\eta\to\gamma\gamma}}%
\htconstrdef{GammaAll.c}{\BR_{\text{All}}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} + \BR_{37} + \BR_{40} + \BR_{42} + \BR_{47}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) + \BR_{48} + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{811} + \BR_{812} + \BR_{93} + \BR_{94} + \BR_{832} + \BR_{833} + \BR_{126} + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{800} + \BR_{151} + \BR_{130} + \BR_{132} + \BR_{44} + \BR_{53} + \BR_{50}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) + \BR_{51} + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-}+\BR_{\phi\to K_S K_L}) + \BR_{152} + \BR_{920} + \BR_{821} + \BR_{822} + \BR_{831} + \BR_{136} + \BR_{945} + \BR_{805}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16}  \\ 
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}  \\ 
  {}& + \BR_{37} + \BR_{40} + \BR_{42} + \BR_{47}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>})))  \\ 
  {}& + \BR_{48} + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{811} + \BR_{812}  \\ 
  {}& + \BR_{93} + \BR_{94} + \BR_{832} + \BR_{833} + \BR_{126} + \BR_{128}  \\ 
  {}& + \BR_{802} + \BR_{803} + \BR_{800} + \BR_{151} + \BR_{130} + \BR_{132}  \\ 
  {}& + \BR_{44} + \BR_{53} + \BR_{50}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>})))  \\ 
  {}& + \BR_{51} + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-}+\BR_{\phi\to K_S K_L}) + \BR_{152} + \BR_{920}  \\ 
  {}& + \BR_{821} + \BR_{822} + \BR_{831} + \BR_{136} + \BR_{945} + \BR_{805}}%
\htconstrdef{Unitarity}{1}{\BR_{\text{All}} + \BR_{998}}{\BR_{\text{All}} + \BR_{998}}%
\htdef{ConstrEqs}{%
\begin{align*}
\htuse{Gamma1.c.left} ={}& \htuse{Gamma1.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma2.c.left} ={}& \htuse{Gamma2.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma3by5.c.left} ={}& \htuse{Gamma3by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma7.c.left} ={}& \htuse{Gamma7.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma8.c.left} ={}& \htuse{Gamma8.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma8by5.c.left} ={}& \htuse{Gamma8by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma9by5.c.left} ={}& \htuse{Gamma9by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma10by5.c.left} ={}& \htuse{Gamma10by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma10by9.c.left} ={}& \htuse{Gamma10by9.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma11.c.left} ={}& \htuse{Gamma11.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma12.c.left} ={}& \htuse{Gamma12.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma13.c.left} ={}& \htuse{Gamma13.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma17.c.left} ={}& \htuse{Gamma17.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma18.c.left} ={}& \htuse{Gamma18.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma19.c.left} ={}& \htuse{Gamma19.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma19by13.c.left} ={}& \htuse{Gamma19by13.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma24.c.left} ={}& \htuse{Gamma24.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma25.c.left} ={}& \htuse{Gamma25.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma26.c.left} ={}& \htuse{Gamma26.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma26by13.c.left} ={}& \htuse{Gamma26by13.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma29.c.left} ={}& \htuse{Gamma29.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma31.c.left} ={}& \htuse{Gamma31.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma32.c.left} ={}& \htuse{Gamma32.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma33.c.left} ={}& \htuse{Gamma33.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma34.c.left} ={}& \htuse{Gamma34.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma38.c.left} ={}& \htuse{Gamma38.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma39.c.left} ={}& \htuse{Gamma39.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma43.c.left} ={}& \htuse{Gamma43.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma46.c.left} ={}& \htuse{Gamma46.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma49.c.left} ={}& \htuse{Gamma49.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma54.c.left} ={}& \htuse{Gamma54.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma55.c.left} ={}& \htuse{Gamma55.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma56.c.left} ={}& \htuse{Gamma56.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma57.c.left} ={}& \htuse{Gamma57.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma57by55.c.left} ={}& \htuse{Gamma57by55.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma58.c.left} ={}& \htuse{Gamma58.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma59.c.left} ={}& \htuse{Gamma59.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma60.c.left} ={}& \htuse{Gamma60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma63.c.left} ={}& \htuse{Gamma63.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma64.c.left} ={}& \htuse{Gamma64.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma65.c.left} ={}& \htuse{Gamma65.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma66.c.left} ={}& \htuse{Gamma66.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma67.c.left} ={}& \htuse{Gamma67.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma68.c.left} ={}& \htuse{Gamma68.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma69.c.left} ={}& \htuse{Gamma69.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma74.c.left} ={}& \htuse{Gamma74.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma75.c.left} ={}& \htuse{Gamma75.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma76.c.left} ={}& \htuse{Gamma76.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma76by54.c.left} ={}& \htuse{Gamma76by54.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma78.c.left} ={}& \htuse{Gamma78.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma79.c.left} ={}& \htuse{Gamma79.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma80.c.left} ={}& \htuse{Gamma80.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma80by60.c.left} ={}& \htuse{Gamma80by60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma81.c.left} ={}& \htuse{Gamma81.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma81by69.c.left} ={}& \htuse{Gamma81by69.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma82.c.left} ={}& \htuse{Gamma82.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma83.c.left} ={}& \htuse{Gamma83.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma84.c.left} ={}& \htuse{Gamma84.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma85.c.left} ={}& \htuse{Gamma85.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma85by60.c.left} ={}& \htuse{Gamma85by60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma87.c.left} ={}& \htuse{Gamma87.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma88.c.left} ={}& \htuse{Gamma88.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma89.c.left} ={}& \htuse{Gamma89.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma92.c.left} ={}& \htuse{Gamma92.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma93by60.c.left} ={}& \htuse{Gamma93by60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma94by69.c.left} ={}& \htuse{Gamma94by69.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma96.c.left} ={}& \htuse{Gamma96.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma102.c.left} ={}& \htuse{Gamma102.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma103.c.left} ={}& \htuse{Gamma103.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma104.c.left} ={}& \htuse{Gamma104.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma106.c.left} ={}& \htuse{Gamma106.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma110.c.left} ={}& \htuse{Gamma110.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma149.c.left} ={}& \htuse{Gamma149.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma150.c.left} ={}& \htuse{Gamma150.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma150by66.c.left} ={}& \htuse{Gamma150by66.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma152by54.c.left} ={}& \htuse{Gamma152by54.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma152by76.c.left} ={}& \htuse{Gamma152by76.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma168.c.left} ={}& \htuse{Gamma168.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma169.c.left} ={}& \htuse{Gamma169.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma804.c.left} ={}& \htuse{Gamma804.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma806.c.left} ={}& \htuse{Gamma806.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma810.c.left} ={}& \htuse{Gamma810.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma820.c.left} ={}& \htuse{Gamma820.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma830.c.left} ={}& \htuse{Gamma830.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma910.c.left} ={}& \htuse{Gamma910.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma911.c.left} ={}& \htuse{Gamma911.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma930.c.left} ={}& \htuse{Gamma930.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma944.c.left} ={}& \htuse{Gamma944.c.right.split}
\end{align*}
\begin{align*}
\htuse{GammaAll.c.left} ={}& \htuse{GammaAll.c.right.split}
\end{align*}}%
\htdef{NumMeasALEPH}{39}%
\htdef{NumMeasARGUS}{2}%
\htdef{NumMeasBaBar}{24}%
\htdef{NumMeasBelle}{15}%
\htdef{NumMeasCELLO}{1}%
\htdef{NumMeasCLEO}{35}%
\htdef{NumMeasCLEO3}{6}%
\htdef{NumMeasDELPHI}{14}%
\htdef{NumMeasHRS}{2}%
\htdef{NumMeasL3}{11}%
\htdef{NumMeasOPAL}{19}%
\htdef{NumMeasTPC}{3}%


==> tau/tau-br-fit-meas-byref.tex <==
%
%
\subsection{Branching fractions fit measurement list by reference}
\cutname{br-fit-meas-byref.html}

Table~\ref{tab:tau:measPerPaper} reports the measurements used for the
\hfagtau branching fraction fit grouped by their bibliographic reference.

%
%
%
\begin{center}
\begin{envsmall}
\renewcommand*{\arraystretch}{1.3}%
\ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
\begin{longtable}{ll}
\caption{By-reference measurements list.\label{tab:tau:measPerPaper}}%
\\
\hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endfirsthead
\multicolumn{2}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endhead
\htuse{MeasPaper} \\
\hline
\end{longtable}
\end{envsmall}
\end{center}


==> tau/tau-defs.tex <==
\newcommand{\BRF}[2]{#2}
%
%
%
%

%
\newcommand{\lepth}{\alpha}
\newcommand{\leptl}{\beta}

%
\newcommand{\radRatio}{R}
%
\newcommand{\radDelta}{\delta R}

%
\newcommand{\Rhad}{\ensuremath{R_{\text{had}}}\xspace}
\newcommand{\BRhad}{\ensuremath{\BR_{\text{had}}}\xspace}
\newcommand{\Gammahad}{\ensuremath{\Gamma_{\text{had}}}\xspace}
%
\newcommand{\Rstrange}{\ensuremath{R_s}\xspace}
\newcommand{\BRstrange}{\ensuremath{\BR_s}\xspace}
\newcommand{\Gammastrange}{\ensuremath{\Gamma_s}\xspace}
\newcommand{\Rnonstrange}{\ensuremath{R_{\text{VA}}}\xspace}
\newcommand{\BRnonstrange}{\ensuremath{\BR_{\text{VA}}}\xspace}
\newcommand{\Gammanonstrange}{\ensuremath{\Gamma_{\text{VA}}}\xspace}
\newcommand{\tauknu}{\ensuremath{\tau^{-} \to K^{-} \nut}\xspace}
\newcommand{\taupinu}{\ensuremath{\tau^{-} \to \pi^{-} \nut}\xspace}
\newcommand{\BFtautoknu}{\ensuremath{\BR(\tauknu)}\xspace}
\newcommand{\BFtautopinu}{\ensuremath{\BR(\taupinu)}\xspace}
\newcommand{\VusUni}{\ensuremath{\Vus_{\text{uni}}}\xspace}
\newcommand{\VusTauIncl}{\ensuremath{\Vus_{\tau s}}\xspace}
\newcommand{\VusTauKpi}{\ensuremath{\Vus_{\tau K/\pi}}\xspace}
\newcommand{\VusTauKnu}{\ensuremath{\Vus_{\tau K}}\xspace}
\newcommand{\VusTauKPinu}{\ensuremath{\Vus_{\tau K\pi}}\xspace}
%
\newcommand{\hfagtau}{HFLAV-Tau\xspace}
%
\newcommand{\dRradTauhHmu}{\ensuremath{\radDelta_{\tau/h}}\xspace}
\newcommand{\dRradTaupiPimu}{\ensuremath{\radDelta_{\tau/\pi}}\xspace}
\newcommand{\dRradTaukKmu}{\ensuremath{\radDelta_{\tau/K}}\xspace}
\newcommand{\RradKmuPimu}{\ensuremath{\radRatio_{K/\pi}}\xspace}
%
\providecommand{\slashLikeH}{%
  \raisebox{.9ex}{%
    \scalebox{.7}{%
      \rotatebox[origin=c]{18}{$-$}%
    }%
  }%
}
\providecommand{\hslash}{%
  {%
   \vphantom{h}%
   \ooalign{\kern.05em\smash{\slashLikeH}\hidewidth\cr$h$\cr}%
   \kern.05em
  }%
}


==> tau/tau-header.tex <==
%
%
%
%
\newcommand{\hfagTauTag}{2021\xspace}
\newcommand{\hfagFitLabel}{HFLAV \hfagTauTag fit}

%
%
%
%
\newif\ifhevea\heveafalse
%

%
\makeatletter
\newenvironment*{fleqn}[1][\leftmargini minus\leftmargini]{\@fleqntrue
  \setlength\@mathmargin{#1}\ignorespaces
}{%
  \ignorespacesafterend
}
\makeatother

\ifhevea
\renewcommand{\babar}{BaBar\xspace}
\else
\makeatletter
\providecommand{\cutname}[1]{}

%
\newenvironment{envsmall}%
  {\small}%
  {}

%
\newenvironment{ceqn}{\@fleqnfalse
  \@mathmargin\@centering \ignorespaces
}{%
  \ignorespacesafterend
}

%
\newenvironment{citenoleadsp}{\@fleqnfalse
  \let\cite@adjust\@empty
}{%
  \ignorespacesafterend
}

%
\newenvironment{ensuredisplaymath}
  {\(\displaystyle}
  {\)}
\makeatother
\fi

%
%
%
\makeatletter

%
\newcommand{\htdef}[2]{%
  \@namedef{hfagtau@#1}{#2}%
}

%
\ifhevea
\newcommand{\htuse}[1]{%
  \@nameuse{hfagtau@#1}}%
\else
\newcommand{\htuse}[1]{%
  \ifcsname hfagtau@#1\endcsname
  \@nameuse{hfagtau@#1}%
  \else
  \@latex@error{Undefined name hfagtau@#1}\@eha
  \fi}
\fi

%
\ifhevea
\newcommand{\htquantdef}[6]{%
  \@namedef{hfagtau@#1.gn}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1.td}{\ensuremath{#3}}%
  \@namedef{hfagtau@#1}{\ensuremath{#4}}%
  \@namedef{hfagtau@#1.v}{\ensuremath{#5}}%
  \@namedef{hfagtau@#1.e}{\ensuremath{#6}}%
}
\else
\newcommand{\htquantdef}[6]{%
  \ifx&#2&\else
  \@namedef{hfagtau@#1.gn}{\ensuremath{#2}}%
  \fi
  \ifx&#3&\else
  \@namedef{hfagtau@#1.td}{\ensuremath{#3}}%
  \fi
  \ifx&#6&%
    \@namedef{hfagtau@#1}{\ensuremath{#5}}%
  \else
    \ifthenelse{\equal{#6}{0}}{%
      \@namedef{hfagtau@#1}{\ensuremath{#5}}%
    }{%
      \@namedef{hfagtau@#1}{\ensuremath{#4}}%
      \@namedef{hfagtau@#1.v}{\ensuremath{#5}}%
      \@namedef{hfagtau@#1.e}{\ensuremath{#6}}%
    }%
  \fi
}
\fi

%
\newcommand{\htmeasdef}[8]{%
  \@namedef{hfagtau@#1,quant}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1,exp}{#3}%
  \@namedef{hfagtau@#1,ref}{\cite{#4}}%
  \@namedef{hfagtau@#1}{\ensuremath{#5}}%
  \@namedef{hfagtau@#1,val}{\ensuremath{#6}}%
  \@namedef{hfagtau@#1,stat}{\ensuremath{#7}}%
  \@namedef{hfagtau@#1,syst}{\ensuremath{#8}}%
}

%
\newcommand{\htconstrdef}[4]{%
  \@namedef{hfagtau@#1.left}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1.right}{\ensuremath{#3}}%
  \@namedef{hfagtau@#1.right.split}{\ensuremath{#4}}%
  \@namedef{hfagtau@#1.constr.eq}{\htuse{#1.left} ={}& \htuse{#1.right}}%
}

\newcommand{\htQuantLine}[3]{\ensuremath{\htuse{#1.td}}&\ensuremath{#2}\\}

\makeatother

\ifhevea
\input{tau-defs}
\input{hflav-2021}
\input{hflav-2018-babar-prelim-ichep2018.tex}
\input{hflav-2021-elab-vadirect}
%
\else
\input{tau/tau-defs}
\input{tau/hflav-2021}
\input{tau/hflav-2018-babar-prelim-ichep2018.tex}
\input{tau/hflav-2021-elab-vadirect}
%
\fi


==> tau/tau-sections.tex <==
This section reports a global fit of the available measurements of \mtau branching fractions and some elaborations of the fit results. In this edition, we do not include the combinations of upper limits on \mtau lepton-flavour-violating branching fractions, which were published in previous editions, since it was not possible to update this  contribution in due time.

Branching fractions averages are obtained with a fit of branching fractions
measurements so as to optimally exploit the available experimental
information. The fit is described in Section~\ref{sec:tau:br-fit}. The fit
results are used in
Section~\ref{sec:tau:leptonuniv} to test the lepton-flavour
universality of the charged-current weak interaction. A ``universality-improved''~\cite{Davier:2005xq}  branching fraction
$\BR_e=\BR(\tau \to e \nu \bar{\nu})$ and the ratio between the hadronic
branching fraction and $\BR_e$ are obtained in
Section~\ref{sec:tau:be-univ-rtau}.
The  value of the Cabibbo-Kobayashi-Maskawa
(CKM) matrix element \Vus obtained from \mtau decays
is given in Section~\ref{sec:tau:vus}.
\iffalse
Combinations of upper limits on lepton-flavour-violating \mtau branching
fractions are computed in Section~\ref{sec:tau:lfv-limits}.
All results are obtained from inputs available through March 2021.
\fi

%
\subsection{Branching fraction fit}
\cutname{br-fit.html}
\label{sec:tau:br-fit}

A fit of the available experimental measurements is used to
determine the \mtau branching fractions, together with their
uncertainties and correlations.
\iffalse
The \mtau branching fractions provide a test for theory predictions based
on the Standard Model (SM) EW and QCD interactions and can be further
elaborated to test the EW charged-current universality for leptons, and to
determine the CKM matrix coefficient \Vus and the QCD coupling constant
$\alpha_s$ at the \mtau mass.
\fi

All relevant published statistical and systematic correlations among the
measurements are used. In addition, for a selection of measurements,
particularly the most precise and the most recent ones, the documented
systematic uncertainty contributions are examined to consider systematic
dependence on external parameters.
\ifx\tauStandalone\undefined
We follow the procedures detailed in Section~\ref{sec:method:corrSysts} to
\else We use the standard HFLAV procedures to
\fi
account for the updated values and uncertainties of the external
parameters and for the correlations induced on different measurements
that have a systematic dependence on the same external parameter.

Both the measurements and the fitted quantities consist of either \mtau
decay branching fractions, labelled  $\BR_{i}$, or ratios of two \mtau
decay branching fractions, labelled  $\BR_{i}/\BR_{j}$. Some branching
fractions are sums of other branching fractions, for instance,
$\htuse{Gamma8.gn} = \BR(\tau^-\to\htuse{Gamma8.td})$, which is the sum of
$\htuse{Gamma9.gn} = \BR(\tau^-\to\htuse{Gamma9.td})$ and
$\htuse{Gamma10.gn} = \BR(\tau^-\to\htuse{Gamma10.td})$, with the symbol $h$
referring to a $\pi$ or a $K$. The fit \chisq is constructed following Eq.~(\ref{eq:averageEq}) and minimized subject to a list of constraints on the fitted quantities:
\begin{itemize}

\item the fitted quantity corresponding to the ratio $\BR_{i}/\BR_{j}$ must
  be equal to the ratio of the respective quantities $\BR_{i}$ and
  $\BR_{j}$;

\item the fitted quantity corresponding to a branching-fraction sum must be equal to the sum of the quantities
  corresponding to the summed branching fractions.

\end{itemize}
The constraints are implemented with Lagrange multipliers (see Sec.~\ref{sec:method}.
In some cases, constraints arise from approximate relations that
nevertheless hold within the present experimental precision and are treated as exact. For
instance, the constraint $\BR(\tau^-\to\htuse{Gamma96.td}) =
\BR(\tau^-\to\htuse{Gamma167.td}) \times \BR(\phi\to K^+K^-)$
is justified given the current experimental evidence.
Section~\ref{sec:tau:constraints} lists all constraint equations
relating the fitted quantities.

Following a convention established in the Review of Particle Physics, \mtau branching fractions are often labelled with the final state content of $\pi^\pm$, $\pi^0$, $K^\pm$, $\gamma$, implicitly including decay chains that involve intermediate particles, e.g., $K^0_S\to\pi^+\pi^-$, and $\eta$, $\omega$, $\phi$ decays. When measurements exclude the contribution of some or all the known intermediate particles, the branching fraction notation flags this information by adding, e.g., ``ex.$K^0$''.

\subsubsection{Fit results}
\label{sec:tau:fit}

We use a total of
\htuse{MeasNum} measurements to fit
\htuse{QuantNum} quantities subject to \htuse{ConstrNum} constraints.
%
The fit has $\chi^2/\text{d.o.f.} = \htuse{Chisq}/\htuse{Dof}$,
corresponding to a confidence level $\text{CL} = \htuse{ChisqProb}$.
%
The fitted quantity values and uncertainties are listed in
Table~\ref{tab:tau:br-fit}.
%
Although the fit treats all quantities in the same way, for the purpose of presenting correlations we select a set
of \htuse{BaseQuantNum} ``basis quantities'' from which all remaining
quantities can be calculated using the definitions listed in
Section~\ref{sec:tau:constraints}.
The off-diagonal correlation coefficients
between the basis quantities are listed
in Section~\ref{sec:tau:fitcorr}.

Table~\ref{tab:tau:br-fit} also reports
$\BR_{110}
= \BR(\tau^- \to X_s^- \nu_\tau)$
(see Section~\ref{sec:tau:constraints}), the total measured branching fraction for \mtau
decays to final states with strangeness 1.
Also reported is the unitarity residual
\htuse{Gamma998.gn} =  \htuse{Gamma998.td} = \htuse{Gamma998}, where $\htuse{Gamma998.td}$
is the sum of the \mtau branching fractions into all measured final states.
We find that $\BR_{998}$ is consistent with 0 to within the
experimental uncertainty.
A unitarity constraint forcing $\BR_{998}$ to be 0 is not applied.


\label{ref:tau:kkk-error-scale-factor}%
%
In performing the fit, a scale factor of 5.44 was applied
to the published uncertainties of the two severely inconsistent
measurements of \(\BR_{96} = \tau \to KKK\nu\) by \babar and
Belle. The scale-factor value was chosen using the PDG procedure,
\ie, it is such that $\chi^2/\text{d.o.f.}=1$
when fitting just the two \(\BR_{96}\) measurements.

%
\subsubsection{Changes with respect to the previous report}

In the previous HFLAV reports~\cite{Amhis:2012bh, Amhis:2014hma, Amhis:2016xyh, Amhis:2019ckw}, information from the ALEPH Collaboration~\cite{Schael:2005am} was used to compute inclusive \mtau branching fractions for final states with one or more hadron, where each hadron can be either a pion or a kaon. In the current report, we use Ref.~\cite{Schael:2005am}  for the branching fractions for exclusive final states containing one or more charged pions. The past choice granted some minor advantages, which are now dropped in the interest of simplicity. As a consequence, the \mtau branching fraction global fit reported here matches more closely the fit that we supply to the PDG, reported in Ref.~\cite{PDG_2020}.

A set of preliminary \babar results presented in 2018~\htuse{BaBar prelim. ICHEP2018.cite}, used in the \mtau branching fraction fit in the previous HFLAV report~\cite{Amhis:2019ckw}, are not used here since they have not yet been published. Therefore, we now use the older \babar measurement of $\htuse{Gamma16.gn} = \BR(\tau^-\to\htuse{Gamma16.td})$ in Ref.~\cite{Aubert:2007jh}. This revision of input measurements causes a significant shift of the value of $\BR(\tau^-\to\htuse{Gamma28.td})$, which is however consistent with the large uncertainty on the sole direct measurement of this mode by ALEPH.

Since this edition, we use new improved calculations of the radiative corrections for the theory predictions of the \mtau decays to pseudoscalar mesons~\cite{Arroyo-Urena:2021nil}. The estimated uncertainties are increased but more reliable in comparison to the previous estimations~\cite{Marciano:1993sh,Decker:1994dd,Decker:1994ea,Decker:1994kw}. There is a minor increase of the uncertainties on the lepton universality tests based on hadronic \mtau decays (section~\ref{sec:tau:leptonuniv}) and on \Vus (section~\ref{sec:tau:vus}).

\iffalse
We use new calculations of the radiative corrections for the theory predictions of $\BR(\pi\to\mu\nu)$ and $\BR(K\to\mu\nu)$~\cite{DiCarlo:2019thl} to produce alternative determinations of \Vus. There are negligible differences on the central values and uncertainties obtained using the previous estimations~\cite{Pich:2013lsa,Cirigliano:2011tm,Marciano:2004uf}.
\fi

The parameters used to update the measurements' systematic biases and
the parameters appearing in the constraint
equations in Section~\ref{sec:tau:constraints} have been updated to the
PDG 2020 update~\cite{PDG_2020}.

%
\subsubsection{Differences between the HFLAV 2021 fit and the PDG 2021
  fit}
\label{sec:tau:diffpdg}
Our branching-fraction fit is different from that of the PDG~\cite{PDG_2020} in several ways.

The PDG fit enforces the unitarity constraint $\BR_{998}=0$, while the HFLAV 2021 fit does not.

As in our previous report~\cite{Amhis:2019ckw}, we use the ALEPH~\cite{PDG_2020} estimate for
$\htuse{Gamma805.gn} =  \BR(\tau^-\to\htuse{Gamma805.td})$, which is not a direct
measurement.
By contrast, the PDG fit defines $\htuse{Gamma805.gn}
= \BR(a_1\to\pi\gamma)\times\BR(\tau \to 3\pi \nu)$, using the PDG average of
$\BR(a_1\to\pi\gamma)$ as a parameter in the fit. As a consequence, the PDG fit
procedure does not take into account the large uncertainty on $\BR(a_1\to\pi\gamma)$.
This results in an underestimated uncertainty on \htuse{Gamma805.gn}, which is then properly adjusted with respect to the fit result in the PDG listings.

%
\subsubsection{Branching fraction fit results and experimental inputs}
\label{sec:tau:br-fit-results}

Table~\ref{tab:tau:br-fit} reports the experimental inputs to the \mtau branching-fraction fit and the fit  results.

%
%
%
\begin{center}
\begin{envsmall}
\setlength{\LTcapwidth}{0.85\linewidth}
\renewcommand*{\arraystretch}{1.3}%
\ifhevea
\renewcommand{\bar}[1]{\textoverline{#1}}
\else
\begin{citenoleadsp}
\fi
\begin{longtable}{llll}
\caption{HFLAV \hfagTauTag branching fractions fit results.\label{tab:tau:br-fit}}%
\\
\toprule
\multicolumn{1}{l}{\bfseries \mtau lepton branching fraction} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{l}{\bfseries Reference} \\
\midrule
\endfirsthead
\multicolumn{4}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
\multicolumn{1}{l}{\bfseries \mtau lepton branching fraction} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{l}{\bfseries Reference} \\
\midrule
\endhead
\endfoot
\endlastfoot
\htuse{BrVal} \\
\bottomrule
\end{longtable}
\ifhevea\else
\end{citenoleadsp}
\fi
\end{envsmall}
\end{center}

\subsubsection{Correlation coefficients between basis branching fractions uncertainties}
\label{sec:tau:fitcorr}

The following tables report the correlation coefficients between basis
quantities that were obtained from the \mtau branching fractions fit,
in percent.

%
%
%
\htuse{BrCorr}

\subsubsection{Equality constraints}
\label{sec:tau:constraints}

The constraints on the \mtau branching-fractions fit quantities are
listed in the following equations.
When a quantity such as
$\BR_3/\BR_5$ appears on the left side of the equation it represents a
fitted quantity, while when it appears on the right side it represents the
ratio of two separate fitted quantities.


The  equations include coefficients that arise from  non-\mtau branching fractions, denoted, \eg, with the
self-describing notation $\BR_{K_S \to \pi^0\pi^0}$. Some coefficients
are probabilities corresponding to the squared moduli  of amplitudes
describing quantum
state mixtures, such as $K^0$, $\bar{K}^0$, $K_S$, $K_L$. These are denoted with,
\eg, $\BR_{<K^0|K_S>} = |{<}K^0|K_S{>}|^2$.
The values of all non-\mtau quantities are taken from the PDG 2021~\cite{PDG_2020}
averages. The fit procedure does not account for their
uncertainties, which are generally small with respect
to the uncertainties on the \mtau branching fractions.


\begin{envsmall}
  \setlength\abovedisplayskip{0pt}
  \setlength\belowdisplayshortskip{0pt}
  \ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
  %
  %
  %
  \htuse{ConstrEqs}
\end{envsmall}

\iffalse
%
%
%
The \mtau branching fractions are listed in Table~\ref{tab:tau:br-fit}.
The equations in the following permit the computation of the values and
uncertainties for branching fractions that are not listed in
Table~\ref{tab:tau:br-fit}, once they are expressed as function of the
quantities that are listed there.
\fi

%
\subsection{Tests of lepton universality}
\cutname{lepton-univ.html}
\label{sec:tau:leptonuniv}

Lepton universality tests probe the Standard-Model prediction that the
weak charged-current interaction has the same coupling for all lepton generations.
Starting with our 2014 report~\cite{Amhis:2014hma}, the precision of such tests was significantly improved due to use of the Belle \mtau lifetime
measurement~\cite{Belous:2013dba}, while improvements from the \mtau
branching fraction fit are negligible.
We perform the universality tests by using
ratios of the partial widths of a heavier lepton $\lepth$
decaying to a lighter lepton $\leptl$~\cite{Marciano:1988vm},
\begin{align}
  \Gamma(\lepth \to \nu_{\lepth} \leptl \nub_{\leptl} (\gamma)) =
  \frac{\BR(\lepth \to \nu_{\lepth} \leptl \nub_{\leptl})}{\tau_{\lepth}} =
  \frac {G_{\lepth} G_{\leptl} m^5_{\lepth}}{192 \pi^3}\, f\left(\frac {m^2_{\leptl}}{m^2_{\lepth}}\right)
  \radRatio^{\lepth\leptl}_W \radRatio^{\lepth}_\gamma~,
\end{align}
where
\begin{alignat}{3}
 G_{\leptl} &= \frac {g^2_{\leptl}}{4 \sqrt{2} M^2_W}~, &\quad&&
 f(x) &= 1 -8x +8x^3 -x^4 -12x^2 \text{ln}x~, \\
 \radRatio^{\lepth \leptl}_W &= 1 + \frac {3}{5} \frac {m^2_{\lepth}}{M^2_W} + \frac {9}{5} \frac {m^2_{\leptl}}{M^2_W}~
\cite{Pich:2013lsa, Ferroglia:2013dga, Fael:2013pja}, &\quad\quad&&
 \radRatio^{\lepth}_\gamma &= 1+\frac {\alpha(m_{\lepth})}{2\pi} \left(\frac {25}{4}-\pi^2\right)~.
\end{alignat}
The equation holds at leading perturbative order (with some corrections being computed at next-to-leading order) for branching fractions to final states that include a soft photon, as detailed in the notation. The inclusion of soft photons is not explicitly mentioned in the branching fractions notation used in this chapter, but ought to be implicitly assumed, since experimental measurements do include soft photons. For most measurements of \mtau branching fractions, soft photons are not experimentally reconstructed but accounted for in the simulations used to estimate the experimental efficiency. We use $\radRatio^\tau_\gamma=1-43.2\cdot 10^{-4}$ and
$\radRatio^\mu_\gamma=1-42.4\cdot 10^{-4}$~\cite{Marciano:1988vm} and $M_W$
from PDG 2021~\cite{PDG_2020}.
We use HFLAV 2021 averages and PDG 2021 for the other quantities.
Using pure leptonic processes we obtain the coupling ratios
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)_\tau = \htuse{gtaubygmu_tau}~,
  \\
  \left( \frac{g_\tau}{g_e} \right)_\tau  = \htuse{gtaubyge_tau}~,
  \\
  \left( \frac{g_\mu}{g_e} \right)_\tau  = \htuse{gmubyge_tau}~.
\end{align}
Using the expressions for the \mtau hadronic partial
widths, we obtain
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)^2_h =
  \frac{\BR({\tau \to h \nu_\tau})}{\BR({h \to \mu \bar{\nu}_\mu})}
  \frac{2m_h m^2_{\mu}\tau_h}{(1 + \dRradTauhHmu)m^3_{\tau}\tau_{\tau}}
  \left( \frac{1-m^2_{\mu}/m^2_h}{1-m^2_h/m^2_{\tau}} \right)^2~,
\end{align}
where $h$ = $\pi$ or $K$. The radiative corrections $\dRradTaupiPimu$ and $\dRradTaukKmu$ have been recently updated with an improved estimation of
their uncertainties and their values are $(\htuse{dRrad_taupi_by_pimu})\%$
and $(\htuse{dRrad_tauK_by_Kmu})\%$~\cite{Arroyo-Urena:2021nil}, respectively.
We obtain:
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)_\pi &= \htuse{gtaubygmu_pi}~,
  & \left( \frac{g_\tau}{g_\mu} \right)_K = \htuse{gtaubygmu_K}~.
\end{align}
The largest contributions to the uncertainties of the tests are the uncertainty on $\dRradTaupiPimu$  for $({g_\tau}/{g_\mu})_\pi$ and the uncertainty on the \mtau branching fraction for $({g_\tau}/{g_\mu})_K$.
Similar tests can be performed using measurements of decay modes with electrons, but are less precise because the meson decays to electrons are helicity suppressed and have less precise experimental measurements.
Averaging the three \(g_\tau/g_\mu\) ratios we obtain
\begin{align}
  \left( \frac{g_\tau}{g_\mu} \right)_{\tau{+}\pi{+}K} &= \htuse{gtaubygmu_fit}~,
\end{align}
accounting for correlations and assuming that the $\dRradTaupiPimu$ and $\dRradTaukKmu$ uncertainties are uncorrelated as they are estimated to be with good approximation~\cite{Arroyo-Urena:2021nil}.
Table~\ref{tab:tau:univ-fit-corr} reports the correlation coefficients for the fitted coupling ratios.
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Universality coupling ratios correlation coefficients (\%).\label{tab:tau:univ-fit-corr}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Universality coupling ratios correlation coefficients (\%).}\label{tab:tau:univ-fit-corr}%
\fi
\begin{center}
\renewcommand*{\arraystretch}{2}%
\begin{tabular}{lcccc}
\toprule
\htuse{couplingsCorr}
\\\bottomrule
\end{tabular}
\end{center}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
\noindent Since $(g_\tau/g_\mu)_\tau = (g_\tau/g_e)_\tau / (g_\mu/g_e)_\tau$, the correlation matrix is expected to be
positive semi-definite, with one eigenvalue equal to zero. Indeed, in the reported correlation matrix there is one eigenvalue that is consistent with zero within the numerical accuracy of the reported figures.

%
\subsection{\texorpdfstring{%
  Universality-improved $\BR(\tau \to e \nu \bar{\nu})$ and $\Rhad$}{%
  Universality-improved B(tau -> e nu nu\_bar) and Rhad}}
\cutname{Be_univ_and_Rtau.html}
\label{sec:tau:be-univ-rtau}

We compute two quantities that are used for further
tests involving the \mtau branching fractions:
\begin{itemize}

\item the ``universality-improved'' value $\BR_e^{\text{uni}}$ of $\BR_e = \BR(\tau \to e \nu \bar{\nu})$, determined with the assumption
  that the Standard Model and lepton universality hold;

\item the ratio \Rhad between the
total branching fraction of the \mtau to hadrons, $\BR_{\text{had}}$ and the universality-improved $\BR_e^{\text{uni}}$, which is a measure of the ratio $\Gamma(\tau \to \text{had}) / \Gamma(\tau\to e\nu\bar{\nu})$ of the respective
partial widths.
\end{itemize}

Following Ref.~\cite{Davier:2005xq}, we obtain the improved value $\BR_e^{\text{uni}}$ using the
\mtau branching fraction to $\mu \nu \bar{\nu}$, $\BR_\mu$, and the \mtau lifetime. We average:
\begin{itemize}

\item the $\BR_e$ fit value \htuse{Gamma5.gn},

\item
  the $\BR_e$ determination from the $\BR_\mu = \BR(\tau \to \mu \nu
  \bar{\nu})$ fit value \htuse{Gamma3.gn} assuming that $g_\mu/g_e = 1$,
  hence (see also Section~\ref{sec:tau:leptonuniv})
  \begin{align}
  \BR_e = \BR_\mu \cdot f(m^2_e/m^2_\tau)/f(m^2_\mu/m^2_\tau)~,
  \end{align}

\item
  the $\BR_e$ determination from the \mtau lifetime assuming that
  $g_\tau/g_\mu =1$, hence
  \begin{align}
  \BR_e = \BR(\mu \to e \bar{\nu}_e
  \nu_\mu)\cdot \frac{\tau_\tau}{\tau_\mu} \cdot \frac{m^5_\tau}{m^5_\mu} \cdot
  f(\frac{m^2_e}{m^2_\tau})/f(\frac{m^2_e}{m^2_\mu}) \cdot (\radRatio_\gamma^\tau
  \radRatio_W^\tau)/(\radRatio_\gamma^\mu \radRatio_W^\mu)~,
  \end{align}
  where $\BR(\mu \to e
  \bar{\nu}_e \nu_\mu) = 1$.

\end{itemize}
Accounting for correlations, we obtain
\begin{align}
  \BR_e^{\text{uni}} = (\htuse{Be_univ})\%.
\end{align}
%
We use $\BR_e^{\text{uni}}$ to obtain the ratio
\begin{align}
  \Rhad = \frac{\Gamma(\tau \to \text{hadrons})}{\Gamma(\tau\to
    e\nu\bar{\nu})} = \frac{\BR_{\text{had}}}{\BR_e^{\text{uni}}} =
  \htuse{R_tau}~,
\end{align}
where $\BR_{\text{had}}$ is the sum of all {\em measured}
branching fractions to hadrons.
\iffalse taken from the sum of all
branching fractions minus the leptonic branching fractions,
$\BR_{\text{had}} = \htuse{GammaAll.gn} - \BR_e - \BR_\mu =
(\htuse{B_tau_had_fit})\%$ (see
Section~\ref{sec:tau:br-fit} and Table~\ref{tab:tau:br-fit} for more details on the
definition of \htuse{GammaAll.gn}).
\fi
An alternative definition of $\BR_{\text{had}}$ uses the unitarity of
the sum of all branching fractions,
$\BR_{\text{had}}^{\text{uni}} = 1 - \BR_e - \BR_\mu =
(\htuse{B_tau_had_uni})\%$, and results in:
\begin{align}
  \Rhad^{\text{uni}} = \frac{1 - \BR_e - \BR_\mu}{\BR_e^{\text{uni}}} =
  \htuse{R_tau_uni}~.
\end{align}

A third definition of $\BR_{\text{had}}$ uses the unitarity of
the sum of all branching fractions, the Standard Model prediction
$\BR_\mu = \BR_e \cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau)$ and $ \BR_e^{\text{uni}}$ to define
$\BR_{\text{had}}^{\text{uni, SM}} = 1 -  \BR_e^{\text{uni}} -
\BR_e^{\text{uni}} \cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau) =
(\htuse{B_tau_had_uni_SM})\%$, yielding
\begin{align}
  \Rhad^{\text{uni, SM}} = \frac{1 - \BR_e^{\text{uni}} -
    \BR_e^{\text{uni}}\cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau)}{\BR_e^{\text{uni}}} =
  \htuse{R_tau_uni_SM}~.
\end{align}
Although $\BR_{\text{had}}^{\text{uni}}$ and
$\BR_{\text{had}}^{\text{uni, SM}}$ are more precise than
$\BR_{\text{had}}$, the precision of $\Rhad^{\text{uni}}$ and
$\Rhad^{\text{uni, SM}}$ is just slightly better than the one of \Rhad
because there are larger correlations between
$\BR_{\text{had}}^{\text{uni}}$, $\BR_{\text{had}}^{\text{uni, SM}}$ and
$\BR_e^{\text{uni}}$ than between $\BR_{\text{had}}$ and $\BR_e^{\text{uni}}$.

%
\subsection{\texorpdfstring{Measurements of $\Vus$}{Vus measurement}}
\cutname{vus.html}
\label{sec:tau:vus}

The CKM matrix element magnitude \Vus is most precisely determined from kaon
decays~\cite{Antonelli:2010yf} (see Figure~\ref{fig:tau:vus-summary}),
and its precision is limited by the
uncertainties of the lattice QCD estimates of the meson form factor $f_+^{K\pi}(0)$ and decay constant in $f_{K\pm}/f_{\pi\pm}$.
Using the \mtau branching fractions, it is possible to determine \Vus in an
alternative way~\cite{Gamiz:2002nu,Gamiz:2004ar} that does not depend on lattice QCD and
has small theory uncertainties (as discussed in Section~\ref{sec:tau:vus:incl}).
Moreover, \Vus can be determined using the \mtau branching fractions
similarly to the kaon case, using the lattice QCD predictions for the meson decay constants.

%
\subsubsection{\texorpdfstring{\Vus from $\BR(\tau \to X_s\nu)$}{Vus from B(tau -> X\_s nu)}}
\label{sec:tau:vus:incl}

The \mtau hadronic partial width is the sum of the \mtau partial widths to
strange and to non-strange hadronic final states, $\Gammahad =
\Gammastrange + \Gammanonstrange$.  The suffix ``VA'' traditionally denotes
the sum of the \mtau partial widths to non-strange final states, which proceed
through either vector or axial-vector currents.

Dividing any partial width $\Gamma_x$
by the electronic partial width, $\Gamma_e$, we obtain partial-width ratios
$R_x$,
%
which satisfy $\Rhad = \Rstrange + \Rnonstrange$. In terms of
such ratios, \Vus can be measured as~\cite{Gamiz:2002nu,Gamiz:2004ar}
\begin{align}
  \VusTauIncl &= \sqrt{\Rstrange/\left[\frac{\Rnonstrange}{\Vud^2} -  \delta R_{\text{theory}}\right]}~,\label{eq:Vus-tau-incl}
\end{align}
where $\delta R_{\text{theory}}$ can be determined using perturbative QCD and partly relying on experimental low energy scattering
data~\cite{Gamiz:2006xx,Gamiz:2007qs,Maltman:2010hb}.  The calculations in the first two references have been criticized for falling short in dealing with the biases and uncertainties in the low-energy regime of QCD~\cite{Hudspith:2017vew}, but are still supported by the authors.
In order to obtain smaller and more reliable QCD uncertainties, alternative procedures for computing \Vus using \mtau decays have been proposed,
which involve the \mtau spectral functions~\cite{Hudspith:2017vew}
and lattice QCD methods~\cite{Boyle:2018dwv}.

In the following, we compute \Vus using the \mtau branching fraction fit results according to eq.~\ref{eq:Vus-tau-incl}, since the complexity of the other
proposed procedures and the effort that is required to reproduce them exceed
the scope of this report. We use Ref.~\cite{Gamiz:2006xx} and the $s$-quark mass $m_s = \htuse{m_s}\,\mev$~\cite{PDG_2020} to calculate
$\delta R_{\text{theory}} = \htuse{deltaR_su3break}$, since that reference quotes uncertainties that are intermediate with respect to the other two assessments in the above mentioned existing literature.

We proceed following the same procedure of the 2012 HFLAV
report~\cite{Amhis:2012bh}. We sum the strange and non-strange hadronic \mtau branching
fractions $\BRstrange$ and $\BRnonstrange$, and  use the
universality-improved $\BR_e^{\text{uni}}$ (see
Section~\ref{sec:tau:be-univ-rtau}) to compute the  $\Rstrange$ and $\Rnonstrange$  ratios.
In past determinations of \Vus, such as the 2009 HFLAV
report~\cite{Asner:2010qj}, the total hadronic branching fraction
was computed using unitarity as $\BRhad^{\text{uni}} = 1 - \BR_e
-\BR_\mu$, and $\BRnonstrange$ was obtained from $\BRhad^{\text{uni}} -
\BRstrange$. Here we use the direct experimental determination
of $\BRnonstrange$ for two reasons.
First, both methods result in comparable uncertainties on \Vus,
since the better precision on  $\BRhad^{\text{uni}} = 1 - \BR_e
-\BR_\mu$ is offset by increased correlations in the
expressions $(1-\BR_e -\BR_\mu)/\BR_e^{\text{uni}}$ and
$\BRstrange/(\BRhad-\BRstrange)$ used in the \Vus calculation. Second, if
there are unobserved \mtau hadronic decay modes, they will affect
\BRnonstrange and \BRstrange in a more asymmetric way when using
unitarity.

Using the \mtau branching fraction fit results with their uncertainties
and correlations (Section~\ref{sec:tau:br-fit}), we compute $\BRstrange =
(\htuse{B_tau_s_fit})\%$ (see Table~\ref{tab:tau:vus}) and
$\BRnonstrange = \BR_{\text{had}} - \BRstrange=
(\htuse{B_tau_VA_fit})\%$. PDG 2021 averages~\cite{PDG_2020}
are used for quantities other than the results of the HFLAV \mtau branching fractions fit; $\Vud =
\htuse{Vud}$ is taken from a 2020 updated determination~\cite{Hardy:2020qwl}.
%
We obtain $\VusTauIncl = \htuse{Vus}$,
where the uncertainty includes a systematic error
contribution of \htuse{Vus_err_th} from the theory uncertainty on
$\delta R_{\text{theory}}$.
This value
is $\htuse{Vus_mism_sigma_abs}\sigma$ lower than the value $\VusUni = \htuse{Vus_uni}$ predicted from the CKM unitarity  relation $(\VusUni)^2 = 1 -
\Vud^2 - \Vub^2$. We also compute $(\Vus/\Vud)_{\tau s} = \htuse{Vus_by_Vud_tauXs}$.
\iffalse
The 2018 \babar preliminary results improved
the \Vus precision by about 10\% and reduced the discrepancy by about
6.5\%.
\fi

%
%
%
\begin{table}
\begin{center}
\renewcommand*{\arraystretch}{1.3}%
\caption{HFLAV \hfagTauTag \mtau branching fractions to strange final states.\label{tab:tau:vus}}%
\ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
\begin{envsmall}
\begin{center}
\begin{tabular}{lc}
\toprule
\multicolumn{1}{l}{\bfseries Branching fraction} &
\multicolumn{1}{c}{\bfseries HFLAV \hfagTauTag fit (\%)} \\
\midrule
\htuse{BrStrangeVal}
\midrule
\htuse{BrStrangeTotVal}
\bottomrule
\end{tabular}
\end{center}
\end{envsmall}
\end{center}
\end{table}

%
%
%
\subsubsection{\texorpdfstring{%
  \Vus from $\BR(\tau \to K\nu) / \BR(\tau \to \pi\nu)$}{%
  Vus from B(tau -> K nu) / B(tau -> pi nu)}}
\label{sec:tau:vus:taukpi}
%
%

We compute $\Vus/\Vud$ from
the ratio of branching fractions $\BR(\tau \to \htuse{Gamma10.td}) / \BR(\tau \to \htuse{Gamma9.td}) = \htuse{Gamma10by9}$
using the equation~\cite{Banerjee:2008hg}:
\begin{align}
  \frac{\BR(\tau^- \to \htuse{Gamma10.td})}{\BR(\tau^- \to \htuse{Gamma9.td})} & =
  \frac{f_{K\pm}^2 \Vus^2}{f_{\pi\pm}^2 \Vud^2} \frac{\left( m_\tau^2 - m_K^2 \right)^2}{\left( m_\tau^2 -  m_\pi^2 \right)^2}
  (1+\delta R_{\tau K/\tau\pi})~,
\end{align}
and we get $\Vus/\Vud = \htuse{Vus_by_Vud_tauKpi}$, using
the ratio of decay constants $f_{K\pm}/f_{\pi\pm} = \htuse{f_Kpm_by_f_pipm}$ from the FLAG 2019 lattice QCD averages with
$N_f=2+1+1$~\cite{Aoki:2019cca,Miller:2020xhy,Dowdall:2013rya,etm:2015lqcd,Bazavov:2017lyh} and $\delta R_{\tau K/\tau\pi} = (\htuse{dRrad_tauK_by_taupi})\%$~\cite{Arroyo-Urena:2021nil}.

By using \Vud~\cite{Hardy:2020qwl}
we compute $\VusTauKpi = \htuse{Vus_tauKpi}$,
$\htuse{Vus_tauKpi_mism_sigma_abs}\sigma$ below the CKM unitarity prediction.

%
%
%
\subsubsection{\texorpdfstring{%
    \Vus from $\BR(\tau \to K\nu)$}{%
    Vus from B(tau -> K nu)}}
\label{sec:tau:vus:tauk}
%
%

We determine \Vus from the branching fraction
$\BFtautoknu$ using
\begin{align}
  \BR(\tau^- \to K^-\nu_\tau) =
  \frac{G^2_F}{16\pi\hslash} f^2_{K\pm} \Vus^2 \tau_{\tau}  m_{\tau}^3 \left(1 - \frac{m_K^2}{m_\tau^2}\right)^2
  S_{EW}
  (1+\delta R_{\tau K})~.
\end{align}
We use $f_{K\pm} = \htuse{f_Kpm}\,\mev$ from the FLAG 2019 lattice QCD averages with
$N_f=2+1+1$~\cite{Aoki:2019cca,Dowdall:2013rya,Bazavov:2014wgs,etm:2015lqcd},
$S_{EW} = \htuse{S_EW}$~\cite{Erler:2002mv} and
$\delta R_{\tau K} =
(\htuse{dRrad_tauK})\%$~\cite{Arroyo-Urena:2021nil}.
We obtain $\VusTauKnu = \htuse{Vus_tauKnu}$,
which is $\htuse{Vus_tauKnu_mism_sigma_abs}\sigma$ below
the CKM unitarity prediction.
The physical constants $G_F$ and $\hslash$ are taken from CODATA 2018~\cite{Tiesinga:2021myr}.
This edition fixes a transcription error on the physical constants taken from PDG 2018 that caused an incorrect shift of the \VusTauKnu determination by about ${+}0.5\,\sigma$ in the previous HFLAV report~\cite{Amhis:2019ckw}.

%
%
%
\subsubsection{\texorpdfstring{Summary of \Vus from \mtau decays}{Summary of Vus from tau decays}}

\begin{figure}[tb]
  \begin{center}
   \ifhevea
    \begin{tabular}{@{}cc@{}}
      \larger\bfseries\ahref{vus-tau-hflav.png}{PNG format} &
      \larger\bfseries\ahref{vus-tau-hflav.pdf}{PDF format} \\
      \multicolumn{2}{c}{\ahref{vus-tau-hflav.png}{%
          \imgsrc[alt="Vus summary plot"]{vus-tau-hflav.png}}}
    \end{tabular}
    \else
    {\fboxsep=2pt\fbox{%
        \includegraphics[width=0.75\linewidth,clip]{figures/tau/vus-tau-hflav.pdf}}}
    \fi
    \caption{\Vus determinations. In the CKM-unitarity evaluation, \Vud is taken from a 2020 experimental update~\cite{Hardy:2020qwl}. The value $\Vus_{K\ell3}$ from $K^-\to \pi^0 \mu^-\bar\nu_\mu$ decays is taken from a 2021 update~\cite{Seng:2021nar}.
    The value $\Vus_{K\ell2}$ from $K^-\to  \mu^-\bar\nu_\mu$ decays is taken from Ref.~\cite{PDG_2020}.
    \label{fig:tau:vus-summary}%
    }
  \end{center}
\end{figure}

We summarize the \Vus results reporting the values, the discrepancy with
respect to the \Vus determination from CKM unitarity, and an illustration
of the measurement method:
\begin{alignat}{6}
  &\VusUni &&= \htuse{Vus_uni.v} &&\pm \htuse{Vus_uni.e} & \quad & \hphantom{{}-{}}0.0\sigma & \quad
  & [\sqrt{1 - \Vud^2 - \Vub^2} \quad\text{(CKM unitarity)}]~, \\
  %
  &\VusTauIncl &&= \htuse{Vus.v} &&\pm \htuse{Vus.e} & \quad & \htuse{Vus_mism_sigma}\sigma &
  & [\BR(\tau^- \to X_s^- \nut)]~, \\
  %
  &\VusTauKpi &&= \htuse{Vus_tauKpi.v} &&\pm \htuse{Vus_tauKpi.e} & \quad & \htuse{Vus_tauKpi_mism_sigma}\sigma &
  & [\BR(\tauknu)/\BR(\taupinu)]~, \label{eq:VusTauKpi} \\
  &\VusTauKnu &&= \htuse{Vus_tauKnu.v} &&\pm \htuse{Vus_tauKnu.e} & \quad & \htuse{Vus_tauKnu_mism_sigma}\sigma &
  & [\BR(\tauknu)]~.\label{eq:VusTauKnu}
\end{alignat}
%
Averaging the two \Vus determinations that rely on exclusive \mtau branching
fractions, we obtain:
\begin{alignat}{6}
  & \Vus_{\tau\text{ excl}} &&= \htuse{Vus_tau_excl} &\quad &\htuse{Vus_tau_excl_mism_sigma}\sigma \quad
  & [\text{average of \mtau exclusive measurements}]~.\label{eq:VusTauExcl}
\end{alignat}
%
Averaging the \mtau inclusive and exclusive \Vus determinations, we obtain:
\begin{alignat}{6}
  & \Vus_\tau &&= \htuse{Vus_tau} &\quad &\htuse{Vus_tau_mism_sigma}\sigma \quad
  & [\text{average of 3 \Vus \mtau measurements}]~.\label{eq:VusTau}
\end{alignat}
In calculating the averages, the correlation between $f_{K\pm}$ and $f_{K\pm}/f_{\pi\pm}$ is
taken to be zero, in absence of public information. Taking it to be $\pm 100\%$ varies the \Vus central value by about 8\% of its uncertainty and the \Vus uncertainty by about 1\% relative. From the purpose of estimating the correlations between $\delta R_{\tau K}$, $\delta R_{\tau\pi}$ and $\delta R_{\tau K/\tau\pi}$ we use the information~\cite{Arroyo-Urena:2021nil} that the uncertainties on $\delta R_{\tau K}$ and $\delta R_{\tau\pi}$ are uncorrelated to a good approximation and that $\delta R_{\tau K/\tau\pi} = \delta R_{\tau K} - \delta R_{\tau\pi}$.

All \Vus determinations based on measured \mtau branching fractions are
lower than both the kaon and the CKM-unitarity determinations. This is
correlated with the fact that the direct measurements of the
three largest \mtau branching fractions to kaons
[$\BR(\tau^-\to\htuse{Gamma10.td})$, $\BR(\tau^-\to\htuse{Gamma16.td})$ and
$\BR(\tau^-\to\htuse{Gamma35.td})$] yield lower values than their SM predictions based on the branching fractions of leptonic kaon decays~\cite{Pich:2013lsa, Jamin:2008qg, Antonelli:2013usa}.

Alternative determinations of \Vus from $\BR(\tau \to
X_s\nu)$~\cite{Hudspith:2017vew,Boyle:2018dwv}, based on partially
different sets of experimental inputs, report \Vus values consistent
with the unitarity determination.

Figure~\ref{fig:tau:vus-summary} reports our \Vus determinations
using the \mtau branching fractions, compared to two
determinations based on kaon data~\cite{PDG_2020} and to the value obtained
from \Vud with CKM-matrix unitarity~\cite{PDG_2020}.




==> tau/tau_all_common.tex <==
%

%
%
%

%
%
%

\ifhevea\else
\makeatletter
\let\citeSaveTau\cite
\let\bfseriesSaveTau\bfseries
\let\LT@makecaptionSaveTau\LT@makecaption
\makeatother

%
\renewcommand{\cite}[1]{\ifmmode\text{\citeSaveTau{#1}}\else\citeSaveTau{#1}\fi}

%
\makeatletter
\DeclareRobustCommand\bfseries{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont\boldmath}
\DeclareRobustCommand*{\bm}[1]{%
    \mathchoice{\bmbox{\displaystyle}{#1}}%
               {\bmbox{\textstyle}{#1}}%
               {\bmbox{\scriptstyle}{#1}}%
               {\bmbox{\scriptscriptstyle}{#1}}}
\DeclareRobustCommand*{\bmbox}[2]{\mbox{\bfseries$#1 #2$}}
\makeatother

%
\makeatletter
\def\LT@makecaption#1#2#3{%
  \LT@mcol\LT@cols c{\hbox to\z@{\hss\parbox[t]\LTcapwidth{%
    \sbox\@tempboxa{\normalsize#1{#2: }#3}%
    \ifdim\wd\@tempboxa>\hsize
      \normalsize#1{#2: }#3%
    \else
      \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
    \fi
    \endgraf\vskip\baselineskip}%
  \hss}}}
\makeatother

\begin{fleqn}
\fi
%
%
%
\ifhevea
\input{tau-sections}
%
%
%
\else
\input{tau/tau-sections}
%
%
%
\fi
%
%
%
\ifhevea\else
\end{fleqn}

\makeatletter
\let\cite\citeSaveTau
\let\bfseries\bfseriesSaveTau
\let\LT@makecaption\LT@makecaptionSaveTau
\makeatother
\fi

